PivotRL: High Accuracy Agentic Post-Training at Low Compute Cost

Post-training for long-horizon agentic tasks has a tension between compute efficiency and generalization. While supervised fine-tuning (SFT) is compute efficient, it often suffers from out-of-domain (OOD) degradation. Conversely, end-to-end reinforcement learning (E2E RL) preserves OOD capabilities, but incurs high compute costs due to many turns of on-policy rollout. We introduce PivotRL, a novel framework that operates on existing SFT trajectories to combine the compute efficiency of SFT with the OOD accuracy of E2E RL. PivotRL relies on two key mechanisms: first, it executes local, on-policy rollouts and filters for pivots: informative intermediate turns where sampled actions exhibit high variance in outcomes; second, it utilizes rewards for functional-equivalent actions rather than demanding strict string matching with the SFT data demonstration. We theoretically show that these mechanisms incentivize strong learning signals with high natural gradient norm, while maximally preserving policy probability ordering on actions unrelated to training tasks. In comparison to standard SFT on identical data, we demonstrate that PivotRL achieves +4.17% higher in-domain accuracy on average across four agentic domains, and +10.04% higher OOD accuracy in non-agentic tasks. Notably, on agentic coding tasks, PivotRL achieves competitive accuracy with E2E RL with 4x fewer rollout turns. PivotRL is adopted by NVIDIA's Nemotron-3-Super-120B-A12B, acting as the workhorse in production-scale agentic post-training.

==> sections/ablations.tex <==
\section{Ablations}
\label{sec:ablations}

\todoempty

% \begin{table*}[!hbt]
% \small
% \centering
% \setlength{\tabcolsep}{6pt}
% % \begin{tabular}{l|c|c|c|c|c|c}
% \newcolumntype{F}{>{\centering\arraybackslash}p{0.8cm}} % adjust 1.3cm to desired 
% \newcolumntype{C}{>{\centering\arraybackslash}p{0.8cm}} % adjust 1.3cm to desired column width
% \begin{tabular}{l|F|F|C|C}
% \toprule
% & \multicolumn{1}{c|}{\textbf{$\tau^2$-Airline}}
% & \multicolumn{1}{c|}{\textbf{$\tau^2$-Retail}}
% & \multicolumn{1}{c|}{\textbf{$\tau^2$-Telecom}}
% & \multicolumn{1}{c}{\textbf{$\tau^2$-Average}} \\
% \midrule
% Baseline (Qwen-8B)
% & 29.33
% & 39.47
% & 30.99
% & 33.26 \\
% \midrule
% Qwen235B
% & 45.33
% & 51.17
% & 27.78
% & 41.43 \\
% OSS-Med
% & 40.67
% & 44.15
% & 46.78
% & 43.87 \\
% OSS-High
% & 44
% & 44.15
% & 50.29
% & 46.15 \\
% DeepSeek-V3.2
% & \todoempty
% & \todoempty
% & \todoempty
% & \todoempty \\
% \bottomrule
% \end{tabular}
% \caption{Ablation: SFT: Effect of different teacher models. Helpful Policies data.}
% \label{table:ablation_sft_teacher_models}
% \end{table*}

% \begin{table*}[!hbt]
% \small
% \centering
% \setlength{\tabcolsep}{6pt}
% % \begin{tabular}{l|c|c|c|c|c|c}
% \newcolumntype{F}{>{\centering\arraybackslash}p{0.8cm}} % adjust 1.3cm to desired 
% \newcolumntype{C}{>{\centering\arraybackslash}p{0.8cm}} % adjust 1.3cm to desired column width
% \begin{tabular}{l|F|F|C|C}
% \toprule
% & \multicolumn{1}{c|}{\textbf{$\tau^2$-Airline}}
% & \multicolumn{1}{c|}{\textbf{$\tau^2$-Retail}}
% & \multicolumn{1}{c|}{\textbf{$\tau^2$-Telecom}}
% & \multicolumn{1}{c}{\textbf{$\tau^2$-Average}} \\
% \midrule
% Baseline (Qwen-8B)
% & 29.33
% & 39.47
% & 30.99
% & 33.26 \\
% \midrule
% Handwritten Policies
% & 44.67
% & 45.32
% & 55.26
% & 0.47 \\
% Helpful Policies
% & 44
% & 44.15
% & 50.29
% & 46.15 \\
% Proactive Policies
% & 37.33
% & 44.15
% & 51.75
% & 44.41 \\
% Helpful, Proactive Policies
% & 48.67
% & 40.94
% & 53.22
% & 47.61 \\
% \bottomrule
% \end{tabular}
% \caption{Ablation: SFT: Handwritten Data vs. Effect of adding different data blends. Using gpt-oss-120b (high) teacher.}
% \label{table:ablation_sft_policy_blend}
% \end{table*}

% \begin{table*}[!hbt]
% \small
% \centering
% \setlength{\tabcolsep}{6pt}
% % \begin{tabular}{l|c|c|c|c|c|c}
% \newcolumntype{F}{>{\centering\arraybackslash}p{0.8cm}} % adjust 1.3cm to desired 
% \newcolumntype{C}{>{\centering\arraybackslash}p{0.8cm}} % adjust 1.3cm to desired column width
% \begin{tabular}{l|F|F|C|C}
% \toprule
% & \multicolumn{1}{c|}{\textbf{$\tau^2$-Airline}}
% & \multicolumn{1}{c|}{\textbf{$\tau^2$-Retail}}
% & \multicolumn{1}{c|}{\textbf{$\tau^2$-Telecom}}
% & \multicolumn{1}{c}{\textbf{$\tau^2$-Average}} \\
% \midrule
% Baseline (Qwen3-30B-A3B)
% & 50
% & 54.39
% & 28.65
% & 44.35 \\
% \midrule
% Handwritten Policies + OSS-High
% & 0.46
% & 0.4737
% & 0.4971
% & 0.476 \\
% Synthetic Policies + OSS-High
% & 46
% & 55.56
% & 58.19
% & 53.25 \\
% Synthetic Policies + DeepSeek-V3.2
% & 54.67
% & 58.48
% & 61.11
% & 58.09 \\
% \bottomrule
% \end{tabular}
% \caption{Ablation: SFT: Experimentation on Qwen3-30B-A3B-Thinking-2507}
% \label{table:ablation_sft_qwen3_30b_results}
% \end{table*}

% \begin{table*}[!hbt]
% \small
% \centering
% \setlength{\tabcolsep}{6pt}
% % \begin{tabular}{l|c|c|c|c|c|c}
% \newcolumntype{F}{>{\centering\arraybackslash}p{0.8cm}} % adjust 1.3cm to desired 
% \newcolumntype{C}{>{\centering\arraybackslash}p{0.8cm}} % adjust 1.3cm to desired column width
% \begin{tabular}{l|F|F|C|C}
% \toprule
% & \multicolumn{1}{c|}{\textbf{$\tau^2$-Airline}}
% & \multicolumn{1}{c|}{\textbf{$\tau^2$-Retail}}
% & \multicolumn{1}{c|}{\textbf{$\tau^2$-Telecom}}
% & \multicolumn{1}{c}{\textbf{$\tau^2$-Average}} \\
% \midrule
% Baseline
% & 38
% & 46.78
% & 42.4
% & 42.39 \\
% SFT
% & 44
% & 41.23
% & 36.55
% & 40.59 \\
% RL
% & 46.67
% & 49.42
% & 48.83
% & 48.31 \\
% \bottomrule
% \end{tabular}
% \caption{Ablation: RL: Results on Nemotron 3 Nano Internal SFT Checkpoint}
% \label{table:ablation_rl_qwen3_30b_results}
% \end{table*}ics

==> sections/abstract.tex <==
\begin{abstract}
\large \textbf{Abstract.}
\normalsize
We introduce PivotRL, a post-training method that achieves the in-domain accuracy and out-of-domain retention of end-to-end reinforcement learning while consuming only existing SFT trajectories and requiring no full-trajectory rollouts. Post-training for agentic capabilities currently forces a choice between SFT, which degrades out-of-domain performance, and end-to-end RL, which preserves it but demands repeated long-horizon environment interaction. PivotRL resolves this tension by identifying informative turns in expert trajectories—which we call \emph{pivots}—and performing on-policy RL only at those turns, scoring completions by whether they are aligned rather than whether they match the expert exactly. We prove that this approach minimally perturbs the reference policy while improving expert agreement, explaining why it avoids out-of-domain degradation. On Qwen3-30B-A3B, PivotRL improves $\tau^2$-Bench from 44.35 to 63.81, SWE-Bench Verified from 19.07 to 32.67, Terminal-Bench from 5.42 to 20.00, and BrowseComp from 2.50 to 11.30, while maintaining near-zero average out-of-domain change (+0.20) versus −9.48 for SFT on the same data.
\end{abstract}


% \begin{abstract}
%     Reinforcement learning (RL) is the most direct way to improve tool-using language models from execution feedback, but \emph{end-to-end token-level} RL is often impractical: tool-use episodes are long, rollouts are sequential, and standard objectives propagate a single return signal through thousands of tokens even though the environment only reacts at tool/turn boundaries.
% We mitigate this long-horizon bottleneck with two complementary changes.

% First, we formulate agentic tool use as an \emph{episodic Markov decision process at the interaction-turn granularity}, where each step is a complete assistant turn (typically a structured tool call or a short natural-language act) and advantages are defined over turns rather than **only** tokens.
% This allows us to align credit assignment with the interface that actually induces transitions and enabling reuse of cached interaction prefixes instead of repeatedly regenerating full episodes.

% Second, under this turn-level MDP we observe that advantages are typically \emph{sparse}: only a small subset of states exhibit large advantage gaps, while most states have nearly flat action values.
% This motivates \textbf{PivotRL}, which concentrates policy optimization on these high-leverage \emph{pivot states} and applies GRPO-style updates only to the pivot-turn span.
% By combining turn-level credit assignment with pivot-focused updates, PivotRL avoids the need to repeatedly execute full end-to-end sequential rollouts for every gradient step---a key practical barrier for agentic RL in the open source community, rivaling larger models like GPT-OSS-120B.

% On the $\tau^2$ Airline/Retail/Telecom benchmarks, PivotRL improves Qwen3-30B-A3B-2507-Thinking from $44.35$ to $62.16$ average success within $300$ RL steps. Further, the same approach is able to improve Qwen3-30B-A3B-2507-Thinking from $8.75$ success rate to $17.50$ success rate on TerminalBench-Core, using the Terminus harness.
% \end{abstract}


==> sections/abstract_v1.tex <==
\begin{abstract}
\large \textbf{Abstract.}
\normalsize
Reinforcement learning (RL) naturally enhances tool-using language agents through execution feedback. However, end-to-end agentic RL is prohibitively expensive due to lengthy tool-use horizons, sequential rollouts, and sparse delayed rewards. In practice, the community relies on supervised fine-tuning (SFT) on expert trajectories, as that is stable and cheap, but suffers from a lack of generalization and lacking explicit reward-driven optimization.

To address these issues, we introduce PivotRL, a turn-level RL framework that bridges SFT and RL using  outcome-verified trajectories that are collected offline. PivotRL formulates agent interactions as an episodic MDP over assistant turns, aligning state transitions with critical tool-call boundaries. Empirically, we find that only a small subset of turns critically influence downstream success. We designate these as pivot states and focus optimization exclusively on them. Crucially, we perform extensive exploration and verification upfront during data collection, thoroughly validating expert actions and exhaustively enumerating all possible pivot states and transition outcomes. Subsequently, we then rely on online RL to solely optimize adherence to these rigorously vetted successful trajectories.

At pivot turns, PivotRL performs a KL-regularized, reward-weighted update toward the outcome-validated expert action, converting long-horizon RL into localized imitation at high-leverage decision points. Uniform rewards recover standard SFT, while non-uniform rewards provide principled policy improvement.

By relying exclusively on logged, extensively verified data, PivotRL enables RL-based improvements from widely available SFT datasets and inference-time interaction traces, removing the need for complex environments or costly rollouts. Through this apporach, PivotRL improves Qwen3-30B-A3B-2507-Thinking from 44.35\% to 62.16\% success rate on Tau-2 (Average of Airline, Retail, and Telecom benchmarks), improves performance from.

\end{abstract}

% \begin{abstract}
%     Reinforcement learning (RL) is the most direct way to improve tool-using language models from execution feedback, but \emph{end-to-end token-level} RL is often impractical: tool-use episodes are long, rollouts are sequential, and standard objectives propagate a single return signal through thousands of tokens even though the environment only reacts at tool/turn boundaries.
% We mitigate this long-horizon bottleneck with two complementary changes.

% First, we formulate agentic tool use as an \emph{episodic Markov decision process at the interaction-turn granularity}, where each step is a complete assistant turn (typically a structured tool call or a short natural-language act) and advantages are defined over turns rather than **only** tokens.
% This allows us to align credit assignment with the interface that actually induces transitions and enabling reuse of cached interaction prefixes instead of repeatedly regenerating full episodes.

% Second, under this turn-level MDP we observe that advantages are typically \emph{sparse}: only a small subset of states exhibit large advantage gaps, while most states have nearly flat action values.
% This motivates \textbf{PivotRL}, which concentrates policy optimization on these high-leverage \emph{pivot states} and applies GRPO-style updates only to the pivot-turn span.
% By combining turn-level credit assignment with pivot-focused updates, PivotRL avoids the need to repeatedly execute full end-to-end sequential rollouts for every gradient step---a key practical barrier for agentic RL in the open source community, rivaling larger models like GPT-OSS-120B.

% On the $\tau^2$ Airline/Retail/Telecom benchmarks, PivotRL improves Qwen3-30B-A3B-2507-Thinking from $44.35$ to $62.16$ average success within $300$ RL steps. Further, the same approach is able to improve Qwen3-30B-A3B-2507-Thinking from $8.75$ success rate to $17.50$ success rate on TerminalBench-Core, using the Terminus harness.
% \end{abstract}


==> sections/experiments.tex <==
\section{Experiments}
\label{sec:experiments}



\subsection{Benchmarks}
We evaluate PivotRL on the following agentic benchmarks:
\begin{itemize}
  \item \textbf{$\tau^2$-bench} \citep{barres2025tau2bench} focuses on conversational tool-use in a multi-turn customer service setting. It contains 3 subsets: Retail and Airline \citep{yao2024taubench}, which tests agent tool-calling, and Telecom, which adds the complexity of user tool-calls. We keep the user model fixed to \texttt{Qwen3-235B-A22B-Instruct-2507} across our evaluations.
  \item \textbf{Terminal-Bench} \citep{tbench_2025} evaluates the model on bash terminal-use tasks that range from filesystem navigation, coding, and system administration to complex problem-solving scenarios such as training machine learning models, configuring legacy systems, and reverse engineering binary files. We evaluate on the TBCore-v1.1 set of questions using the Terminus-2 harness.
  \item \textbf{Swe-Bench} \citep{jimenez2024swebench} evaluates the model on various real-world programming tasks that can be described as understanding an issue, localizing the issue in a codebase, and creating a code patch to resolve the issue. We use the SWE-Bench-Verified subset which is a widely adopted set of 500 verifiable questions. We evaluate using the OpenHands harness. 
  \item \textbf{BrowseComp}
  \citep{wei2025browsecompsimplechallengingbenchmark} tests the search agent capabilities of a model through very difficult questions that require critical reasoning and the use of a search engine to answer correctly. It often results in very long trajectories with many search calls for each problem, and is shown to be a hard benchmark for current frontier LLMs.
\end{itemize}

\begin{table}[!t]
\centering
\small
\begin{tabular}{lcccc}
\toprule
\textbf{Benchmark} & \textbf{Qwen3-30B (\%)} & SFT & \textbf{PivotRL (\%)} & \textbf{Gain ($\Delta$)} \\ 
\midrule
$\tau^2$-Bench     & 44.35 & & 63.81 & +19.46 \\
SWE-Verified       & 19.07 & & 32.67 & +13.6 \\
Terminal-Bench     & 5.42  & & 20.00 & +14.58 \\ 
BrowseComp         & 2.50  & & 11.30 & +8.80  \\
\bottomrule
\end{tabular}
\caption{Main results of benchmark accuracy gain after training with PivotRL on \texttt{Qwen3-30B-A3B-Thinking-2507}.}
\label{tab:main_results_enhanced}
\end{table}
% \begin{table}[!t]
% \centering
% \small % Slightly smaller font to ensure it fits well in double-column layouts
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{l c cc cc cc cc}
% \toprule
% \multirow{2}{*}{\textbf{Benchmark}} & \textbf{Baseline} & \multicolumn{2}{c}{$\tau^2$-\textbf{Bench}} & \multicolumn{2}{c}{\textbf{SWE-Verified}} & \multicolumn{2}{c}{\textbf{Terminal-Bench}} & \multicolumn{2}{c}{\textbf{BrowseComp}} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
% & \textbf{Qwen3-30B} & \textbf{sft} & \textbf{rl} & \textbf{sft} & \textbf{rl} & \textbf{sft} & \textbf{rl} & \textbf{sft} & \textbf{rl} \\
% \midrule
% IFBench        & 52.04 & 44.42 & 53.29 & - & 51.72 & 24.77 & 49.47 & 54.35 & 53.89 \\
% AIME25         & 86.04 & 76.25 & 85.63 & - & 84.58 & 21.56 & 82.92 & 85.21 & 85.83 \\
% MATH500        & 98.05 & 98.00 & 98.35 & - & 98.00 & 63.55 & 98.00 & 98.30 & 98.40 \\
% LiveCodeBench  & 66.52 & 64.98 & 66.96 & - & 67.62 & 45.15 & 64.54 & 67.62 & 66.96 \\
% Scicode (subtask) & 36.83 & 31.95 & 38.68 & - & 36.39 & 9.39  & 39.13 & 35.58 & 37.28 \\
% MMLU-Pro       & 80.84 & 79.81 & 81.31 & - & 80.70 & 71.57 & 80.85 & 81.13 & 81.31 \\
% MMLU-ProX      & 78.58 & 74.31 & 78.92 & - & 78.55 & 59.13 & 78.49 & 76.68 & 78.60 \\
% WMT24++ (en$\rightarrow$xx)       & 36.97 & 34.25 & 36.54 & - & 36.71 & 6.31  & 36.48 & 33.18 & 36.26 \\
% \bottomrule
% \end{tabular}%
% }
% \caption{Out-of-domain regression analysis results after training with PivotRL on \texttt{Qwen3-30B-A3B-Thinking-2507}. No SFT was done on the SWE-Bench targeted model due to using non-thinking data for PivotRL.}
% \label{tab:main_results_regression}
% \end{table}

\begin{table*}[!t]
\centering
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{l c cc cc cc cc}
\toprule
\multirow{3}{*}{\textbf{Benchmark}} 
& \multirow{3}{*}{\textbf{Baseline}} 
& \multicolumn{8}{c}{\textbf{Training Domain (score + $\Delta$)}} \\
\cmidrule(lr){3-10}
& 
& \multicolumn{2}{c}{$\tau^2$} 
& \multicolumn{2}{c}{SWE} 
& \multicolumn{2}{c}{Terminal} 
& \multicolumn{2}{c}{BrowseComp} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
& Qwen3-30B 
& sft & rl 
& sft & rl 
& sft & rl 
& sft & rl \\
\midrule
\midrule

\textbf{Peak In-Domain} 
& -- 
& 58.44 (+14.09) & 63.81 (+19.46)
& 37.40 (+18.33) & 32.67 (+13.60)
& 13.75 (+8.33)  & 20.00 (+14.58)
& 1.50 (-1.00)   & 11.30 (+8.80) \\
\midrule

IFBench 
& 52.04 
& 44.42 (-7.62) & 53.29 (+1.25)
& 38.80 (-13.24) & 54.79 (+2.75)
& 24.77 (-27.27) & 49.47 (-2.57)
& 54.35 (+2.31)  & 53.89 (+1.85) \\

AIME25 
& 86.04 
& 76.25 (-9.79) & 85.63 (-0.41)
& 82.29 (-3.75)  & 85.00 (-1.04)
& 21.56 (-64.48) & 82.92 (-3.12)
& 85.21 (-0.83)  & 85.83 (-0.21) \\

MATH500 
& 98.05 
& 98.00 (-0.05) & 98.35 (+0.30)
& 98.30 (+0.25)  & 98.65 (+0.60)
& 63.55 (-34.50) & 98.00 (-0.05)
& 98.30 (+0.25)  & 98.40 (+0.35) \\

LiveCodeBench 
& 66.52 
& 64.98 (-1.54) & 66.96 (+0.44)
& 57.27 (-9.25)  & 66.96 (+0.44)
& 45.15 (-21.37) & 64.54 (-1.98)
& 67.62 (+1.10)  & 66.96 (+0.44) \\

Scicode 
& 36.83 
& 31.95 (-4.88) & 38.68 (+1.85)
& 24.85 (-11.98) & 39.87 (+3.04)
& 9.39 (-27.44)  & 39.13 (+2.30)
& 35.58 (-1.25)  & 37.28 (+0.45) \\

MMLU-Pro 
& 80.84 
& 79.81 (-1.03) & 81.31 (+0.47)
& 78.90 (-1.94)  & 81.13 (+0.29)
& 71.57 (-9.27)  & 80.85 (+0.01)
& 81.13 (+0.29)  & 81.31 (+0.47) \\

MMLU-ProX 
& 78.58 
& 74.31 (-4.27) & 78.92 (+0.34)
& 75.58 (-3.00)  & 78.81 (+0.23)
& 59.13 (-19.45) & 78.49 (-0.09)
& 76.68 (-1.90)  & 78.60 (+0.02) \\

WMT24++ 
& 36.97 
& 34.25 (-2.72) & 36.54 (-0.43)
& 35.69 (-1.28)  & 36.66 (-0.31)
& 6.31 (-30.66)  & 36.48 (-0.49)
& 33.18 (-3.79)  & 36.26 (-0.71) \\

\bottomrule
\end{tabular}%
}
\caption{
Out-of-domain regression across four training domains.
Each cell shows score followed by per-task $\Delta$ relative to the Qwen3-30B baseline.
SFT exhibits substantial catastrophic forgetting, especially when trained on Terminal.
PivotRL (RL) largely preserves general capability while achieving higher or comparable in-domain performance.
All RL–SFT comparisons use identical seed prompts and trajectories.
}
\label{tab:main_results_regression_delta_inline}
\end{table*}


\begin{table}[!t]
\centering
\small
\begin{tabular}{l c cc}
\toprule
\textbf{Evaluation} & \textbf{Baseline} & \textbf{Avg $\Delta$ SFT} & \textbf{Avg $\Delta$ RL} \\
\midrule
\textbf{In-Domain (Peak)} & -- & +9.94 & +14.11 \\
\midrule
IFBench        & 52.04 & -10.45 & +0.82 \\
AIME25         & 86.04 & -19.71 & -1.20 \\
MATH500        & 98.05 & -8.58  & +0.30 \\
LiveCodeBench  & 66.52 & -8.41  & -0.16 \\
Scicode        & 36.83 & -8.89  & +1.91 \\
MMLU-Pro       & 80.84 & -3.05  & +0.31 \\
MMLU-ProX      & 78.58 & -7.15  & +0.13 \\
WMT24++        & 36.97 & -9.59  & -0.49 \\
\midrule
\textbf{Avg OOD (All Benchmarks)} & 66.98 & -9.48 & +0.20 \\
\bottomrule
\end{tabular}
\caption{
Average performance change ($\Delta$) relative to the Qwen3-30B baseline across four training domains. 
PivotRL achieves significantly higher in-domain gains while maintaining near-zero average out-of-domain regression, whereas SFT shows substantial catastrophic forgetting.
}
\label{tab:per_benchmark_avg_regression}
\end{table}



\subsection{Main Results}
\subsubsection{In-Domain Improvement}
We conduct all PivotRL experiments on \texttt{Qwen3-30B-A3B-Thinking-2507}, using Nemo-RL \citep{nemo-rl} as the training framework and utilizing Nemo-Gym \citep{nemo-gym} for the environment rollouts. We show considerable gain in all four domains of Conversational Tool-Use, Software Engineering, Terminal Use, and Search using PivotRL as shown in Table \ref{tab:main_results_enhanced}. All four experiments were run independently of each other, with separate resulting policies. We discuss individual experiments and results below.

\subsubsection{Out-of-Domain Knowledge Retention}
In addition to in-domain improvement our method also shows little to no degradation in other capabilities when compared to SFT. \textbf{We utilize the same data (prompts and trajectories) for both SFT and PivotRL for these comparisons.}

In Table \ref{tab:main_results_regression_delta_inline} we show various benchmark results for the SFT and PivotRL model for each separate trained model. We evaluate on General Knowledge (MMLU-Pro \citep{wang2024mmluprorobustchallengingmultitask}), Reasoning, Math, and Coding (AIME25, MATH500 \citep{hendrycks2021measuringmathematicalproblemsolving,lightman2023letsverifystepstep}, LiveCodeBench (v6 2024-08$\leftrightarrow$2025-05) \citep{jain2024livecodebench}, Scicode \citep{tian2024scicoderesearchcodingbenchmark}), Instruction Following (IFBench \citep{pyatkin2025generalizing}), and Multilingual (MMLU-ProX \citep{xuan2025mmluproxmultilingualbenchmarkadvanced}, WMT24++ (en$\rightarrow$xx) \citep{deutsch2025wmt24expandinglanguagecoverage}).

\begin{table*}[!bt]
\small
\centering
\setlength{\tabcolsep}{6pt}
% \begin{tabular}{l|c|c|c|c|c|c}
\newcolumntype{F}{>{\centering\arraybackslash}p{0.8cm}} % adjust 1.3cm to desired 
\newcolumntype{C}{>{\centering\arraybackslash}p{0.8cm}} % adjust 1.3cm to desired column width
\begin{tabular}{l|F|F|C|C}
\toprule
& \multicolumn{1}{c|}{\textbf{$\tau^2$-Airline}}
& \multicolumn{1}{c|}{\textbf{$\tau^2$-Retail}}
& \multicolumn{1}{c|}{\textbf{$\tau^2$-Telecom}}
& \multicolumn{1}{c}{\textbf{$\tau^2$-Average}} \\
\midrule
gpt-oss-120b-high
& 55.33 & 58.19 & 67.20 & 60.24 \\
gpt-oss-20b-high
& 43.33 & 50.20 & 52.63 & 48.72 \\
Qwen3-235B-A22B-Thinking-2507
& 50.0 & 66.08 & 46.78 & 54.29 \\
\midrule
Qwen3-30B-A3B-Thinking-2507
& 50.00
& 54.39
& 28.65
& 44.35 \\
\hdashline
Qwen + SFT
& 51.33
& 58.19
& 65.79
& 58.44 \\
Qwen + Random
& 58.00
& 63.74
& 57.31
& 59.68 \\
Qwen + All Mixed Rewards
& 61.33
& 66.08
& 56.73
& 61.38 \\
Qwen + Large Advantage Gap
& 58.67
& 69.01
& 63.74
& 63.81 \\
\bottomrule
\end{tabular}
\caption{Effect of pivot selection algorithm on downstream performance. Best checkpoint over training. While randomly choosing pivots improves the model, choosing only pivots with mixed rewards provides a superior learning signal, and further constraining the pivots to have mean reward $\leq 0.6$ yields the best set of pivot training dataset.}
\label{tab:results_tau_rl_pivot_selection}
\end{table*}

\subsection{$\tau^2$-bench}
\subsubsection{Experimental Details}
We curate an SFT training set consisting of $281774$ trajectories across $838$ domains by following a synthetic data generation procedure similar to ToolAce \citep{liu2025toolacewinningpointsllm}, Kimi-K2 \citep{kimiteam2025kimik2openagentic}, and DeepSeek-V3.2 \citep{deepseekai2025deepseekv32pushingfrontieropen}. We train on top of the \texttt{Qwen3-30B-A3B-Thinking-2507} \citep{qwen3technicalreport} model and compare with open-source models such as \texttt{Qwen3-235B-A22B-Thinking-2507} and the \texttt{gpt-oss} \citet{openai2025gptoss120bgptoss20bmodel} models under the high reasoning setting.

\subsubsection{Results}
Under the best pivot selection setting, our method is able to achieve higher overall accuracy in $\tau^2$-bench than using SFT, and outperform even much larger models such as the \texttt{Qwen-235B} and \texttt{oss-120B models}. Our results are summarized in Table \ref{tab:results_tau_rl_pivot_selection}. Both the SFT baseline and the RL results were chosen from the best checkpoint across a fixed training experiment.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/main_average_validation.pdf}
%     \caption{$\tau^2$-bench performance throughout RL training. Choosing pivots with a large advantage gap yields superior model improvement compared to choosing pivots with nonzero advantage or randomly choosing pivots.}
%     \label{fig:rl_tau_pivot_selection_acc}

%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/tau_reward_stddev.pdf}
%     \caption{$\tau^2$-bench training reward standard deviation over training. The random reward setting quickly yields unbalanced training rewards while the mixed rewards and high advantage gap settings leads to higher standard deviation in training rewards per group, allowing for better GRPO training.}
%     \label{fig:rl_tau_pivot_selection_acc}
% \end{figure}
\begin{figure}[t]
    \centering
    % Left side minipage
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/main_average_validation.pdf}
        \caption{$\tau^2$-bench performance throughout RL training. Choosing pivots with a large advantage gap yields superior model improvement, outperforming even SFT on the base dataset.}
        \label{fig:rl_tau_pivot_selection_acc}
    \end{minipage}
    \hfill % Adds horizontal space between the two minipages
    % Right side minipage
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/tau_reward_stddev.pdf}
        \caption{$\tau^2$-bench training reward standard deviation. Higher standard deviation in training rewards allows for better GRPO training. Showing rolling standard deviation for viewer readability.}
        \label{fig:rl_tau_reward_stddev}
    \end{minipage}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/main_per_domain_validation_difficulty.pdf}
    \caption{Per-domain benchmark performance over RL training. From left to right: Telecom, Retail, Airline.}
    \label{fig:rl_domain}
\end{figure*}


\subsubsection{Effect of Pivot Selection}
In Figures \ref{fig:rl_tau_pivot_selection_acc} and \ref{fig:rl_tau_reward_stddev}, we observe the effect of different pivot selection algorithms by the change in accuracy over RL training steps as well as the training reward standard deviation over RL steps. While the random pivot selection baseline is able to improve the model, it under-performs the mixed rewards setting where at the beginning of training every input prompt has non-zero advantage. Empirically, this is shown as the standard deviation of the reward for that prompt across the rollouts being larger. Meanwhile, further constraining the dataset to choose from points where the advantage gap is large yields the best performing training dataset, improving the model accuracy from $44.35\%$ to $63.81\%$ after 430 steps of training. We also see that as training goes, the large advantage gap set also has a more balanced reward distribution for each prompt as can be seen with the higher training reward standard deviation.



\subsection{Terminal-Bench}
\subsubsection{Experimental Details}
We collected resolved and completed trajectories from \texttt{Qwen/Qwen3-Coder-480B-A35B-Instruct} and \texttt{moonshotai/Kimi-K2-Instruct} on Terminal Bench using the Terminus 1 and Terminus 2 agents, and use all assistant bash actions as pivots. From the $\mathcal{D}_{\text{adv}}$ setting, we additionally deduplicate similar commands to achieve diversity in the data. Our final training set consisted of approximately 20,000 samples. For verification in the RL environment, we employed output schema validation, string similarity, and equivalency-based LLM-as-judge in the reward design.

\subsection{SWE-Bench Verified}
\subsubsection{Experimental Details}
We use an internal dataset of trajectories generated using the OpenHands \citep{wang2025openhandsopenplatformai}, OpenCode \citep{opencode}, and Codex \citep{openaicodex_software} harnesses on tasks including SWE-Gym \citep{pan2025trainingsoftwareengineeringagents}, and R2E-Gym \citep{jain2025r2egymproceduralenvironmentshybrid} using the \texttt{MiniMaxAI/MiniMax-M2.5} \citep{minimax2026m25} model. We evaluate the mean@3 score using the OpenHands harness. To create the PivotRL dataset, we use all tool call actions that did not result in error calls as pivots, and use a string similarity verifier that matches only tool call names for $r_{\name}$. We curate a final dataset in the $\mathcal{D}_{\text{adv}}$ setting of size $87718$ for training.


\subsection{BrowseComp}
\subsubsection{Experimental Details}
We start with a multi-hop question-answer dataset and use an online search engine along with \texttt{DeepSeek-V3.2} to generate trajectories from it. We curate a set of $13215$ samples and use random filtering ($\mathcal{D}_{\text{random}}$) due to the small size of the dataset. We use this dataset to train on top of \texttt{Qwen3-30B-A3B-Thinking-2507}.
\subsubsection{Results}
Under the best settings, we are able to improve \texttt{Qwen3-30B-A3B-Thinking-2507} from $2.5$ accuracy to $11.3$.


\begin{table*}[!t]
\centering
\small
\begin{tabular}{l c cc c}
\toprule
\multirow{2}{*}{\textbf{Benchmark}} 
& \multirow{2}{*}{\textbf{Baseline}} 
& \multicolumn{2}{c}{\textbf{Multi-Domain Training}}
& \multirow{2}{*}{\textbf{RL vs SFT ($\Delta$)}} \\
\cmidrule(lr){3-4}
& Qwen3-30B 
& \textbf{SFT} & \textbf{RL} & \\
\midrule
\midrule

\multicolumn{5}{l}{\textit{In-Domain Benchmarks}} \\
\midrule

Tau2 
& 44.35 
& 57.60 (+13.25) & 56.33 (+11.98) 
& -1.27 \\

SWE-Verified
& 19.07 
& -- \quad (--) & 32.87 (+13.80) 
& -- \\

Terminal-Bench
& 5.42 
& -- \quad (--) & -- \quad (--) 
& -- \\

BrowseComp
& 2.50 
& -- \quad (--) & -- \quad (--) 
& -- \\

\midrule
\multicolumn{5}{l}{\textit{Out-of-Domain Benchmarks}} \\
\midrule

IFBench 
& 52.04 
& 47.71 (-4.33)  & 50.41 (-1.63) 
& +2.70 \\

AIME25 
& 86.04 
& 83.13 (-2.91)  & 85.83 (-0.21) 
& +2.70 \\

MATH500 
& 98.05 
& 98.15 (+0.10)  & 98.15 (+0.10) 
& 0.00 \\

LiveCodeBench 
& 66.52 
& 60.57 (-5.95)  & 67.40 (+0.88) 
& +6.83 \\

Scicode 
& 36.83 
& 26.18 (-10.65) & 38.17 (+1.34) 
& +11.99 \\

MMLU-Pro 
& 80.84 
& 80.97 (+0.13)  & 81.14 (+0.30) 
& +0.17 \\

MMLU-ProX 
& 78.58 
& -- \quad (--)  & 78.74 (+0.16) 
& -- \\

WMT24++ 
& 36.97 
& 34.87 (-2.10)  & 36.92 (-0.05) 
& +2.05 \\

\bottomrule
\end{tabular}
\caption{Evaluation results for Multi-domain training.}
\label{tab:combined_training_results}
\end{table*}

\subsection{Multi-domain Training}
\subsubsection{Experimental Setup}
We additionally train a model on all domains combined. For SFT, we combine all 4 SFT datasets using temperature sampling with $\text{temperate}=0.5$, which yields a dataset that is: conversational tool-use: 56.38\%), (swe: 11.01\%), (terminal: 31.36\%), and (search: 1.25\%). We conduct training with batch size 128 and learning rate 5e-6. For \name, we combine the 4 RL datasets with equal weighing. Using batch size 128, each domain will have an average of 32 groups per batch. We rollout 16 times per prompt with a 1e-6 learning rate with one gradient update per batch.

\subsubsection{Results and Analysis}
The evaluation results of resulting models are shown in Table \ref{tab:combined_training_results}. For in-domain benchmarks, PivotRL is competitive to SFT. In out of domain benchmarks, PivotRL is significantly better at retaining existing capabilities compared to SFT. The results clearly show that PivotRL can be adopted as a general training framework for improving the capabilities of models in multiple domains simultaneously without significant concern for catastrophic forgetting.



==> sections/experiments_v1.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Benchmarks}
We evaluate PivotRL on the following agentic benchmarks:
\begin{itemize}
  \item \textbf{$\tau^2$-bench} \citep{barres2025tau2bench} focuses on conversational tool-use. It evaluates the model on 3 different customer service settings: Retail and Airline \citep{yao2024taubench}, which asks for the model to call a series of tool calls across a multi-turn conversation with a simulated user, and Telecom, which adds the additional possibility for the model to instruct the user to call a set of user tools. We keep the user model fixed to \texttt{Qwen3-235B-A22B-Instruct-2507} \citet{qwen3technicalreport} across our evaluations.
  \item \textbf{Terminal-Bench} \citep{tbench_2025} evaluates the model on bash terminal-use tasks that range from filesystem navigation, coding, and system administration to complex problem-solving scenarios such as training machine learning models, configuring legacy systems, and reverse engineering binary files. Terminal-Bench v1 consists of 80 hard, realistic tasks that require the agent to autonomously explore the environment, execute multi-step command-line solutions, and verify their work. Specifically, we use the TBCore-v1.1 set of questions.
  \item \textbf{Swe-Bench Verified} \citep{jimenez2024swebench} evaluates the model on various real-world programming tasks that can be described as understanding an issue, localizing the issue in a codebase, and creating a code patch to resolve the issue.
  \item \textbf{BrowseComp}
  \citep{wei2025browsecompsimplechallengingbenchmark} \todo{damon,ritu}
\end{itemize}

\begin{table}[!t]
\centering
\small % Slightly smaller font to ensure it fits well in double-column layouts
\begin{tabular}{lcccc}
\toprule
\textbf{Benchmark} & Filtering & \textbf{Qwen3-30B (\%)} & \textbf{PivotRL (\%)} & \textbf{Gain ($\Delta$)} \\ 
\midrule
$\tau^2$-Bench             & $\mathcal{D}_{\text{adv}}$    & 44.35 & 63.81 & +19.46 \\
SWE-Verified               & $\mathcal{D}_{\text{mixed}}$  & 19.07 & 31.93 & +12.86 \\
Terminal-Bench             & $\mathcal{D}_{\text{mixed}}$  & 5.42  & 20.00 & +14.58 \\ 
BrowseComp                 & $\mathcal{D}_{\text{random}}$ & 2.50  & 11.30 & +8.80  \\
\bottomrule
\end{tabular}
\caption{Main results of benchmark accuracy gain after training with PivotRL on \texttt{Qwen3-30B-A3B-Thinking-2507}.}
\label{tab:main_results_enhanced}
\end{table}

\subsection{Main Results}
We conduct our PivotRL experiments on \texttt{Qwen3-30B-A3B-Thinking-2507}, using Nemo-RL \citep{nemo-rl} as the training framework and utilizing Nemo-Gym \citep{nemo-gym} for the environment rollouts. We show considerable gain in all four domains of Conversational Tool-Use, Software Engineering, Terminal Use, and Search using PivotRL as showin in Table \ref{tab:main_results_enhanced}. All four experiments were run independently of each other, with separate resulting policies. We discuss individual experiments and results below.

\begin{table*}[!bt]
\small
\centering
\setlength{\tabcolsep}{6pt}
% \begin{tabular}{l|c|c|c|c|c|c}
\newcolumntype{F}{>{\centering\arraybackslash}p{0.8cm}} % adjust 1.3cm to desired 
\newcolumntype{C}{>{\centering\arraybackslash}p{0.8cm}} % adjust 1.3cm to desired column width
\begin{tabular}{l|F|F|C|C}
\toprule
& \multicolumn{1}{c|}{\textbf{$\tau^2$-Airline}}
& \multicolumn{1}{c|}{\textbf{$\tau^2$-Retail}}
& \multicolumn{1}{c|}{\textbf{$\tau^2$-Telecom}}
& \multicolumn{1}{c}{\textbf{$\tau^2$-Average}} \\
\midrule
gpt-oss-120b-high
& 55.33 & 58.19 & 67.20 & 60.24 \\
gpt-oss-20b-high
& 43.33 & 50.20 & 52.63 & 48.72 \\
Qwen3-235B-A22B-Thinking-2507
& 50.0 & 66.08 & 46.78 & 54.29 \\
\midrule
Qwen3-30B-A3B-Thinking-2507
& 50.00
& 54.39
& 28.65
& 44.35 \\
\hdashline
Qwen + SFT
& 51.33
& 58.19
& 65.79
& 58.44 \\
Qwen + Random
& 58.00
& 63.74
& 57.31
& 59.68 \\
Qwen + All Mixed Rewards
& 61.33
& 66.08
& 56.73
& 61.38 \\
Qwen + Large Advantage Gap
& 58.67
& 69.01
& 63.74
& 63.81 \\
\bottomrule
\end{tabular}
\caption{Effect of pivot selection algorithm on downstream performance. Best checkpoint over training. While randomly choosing pivots improves the model, choosing only pivots with mixed rewards provides a superior learning signal, and further constraining the pivots to have mean reward $\leq 0.6$ yields the best set of pivot training dataset.}
\label{tab:results_tau_rl_pivot_selection}
\end{table*}

\subsection{$\tau^2$-bench}
\subsubsection{Dataset and Baselines}
We curate an SFT training set consisting of $281774$ trajectories across $838$ domains by following a synthetic data generation procedure similar to ToolAce \citep{liu2025toolacewinningpointsllm}, Kimi-K2 \citep{kimiteam2025kimik2openagentic}, and DeepSeek-V3.2 \citep{deepseekai2025deepseekv32pushingfrontieropen}. We train on top of the \texttt{Qwen3-30B-A3B-Thinking-2507} \citep{qwen3technicalreport} model and compare with open-source models such as \texttt{Qwen3-235B-A22B-Thinking-2507} and the \texttt{gpt-oss} \citet{openai2025gptoss120bgptoss20bmodel} models under the high reasoning setting.

\subsubsection{Results}
Under the best pivot selection setting, our method is able to achieve higher overall accuracy in $\tau^2$-bench than using SFT, and outperform even much larger models such as the \texttt{Qwen-235B} and \texttt{oss-120B models}. Our results are summarized in Table \ref{tab:results_tau_rl_pivot_selection}. Both the SFT baseline and the RL results were chosen from the best checkpoint across a fixed training experiment.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/main_average_validation.pdf}
%     \caption{$\tau^2$-bench performance throughout RL training. Choosing pivots with a large advantage gap yields superior model improvement compared to choosing pivots with nonzero advantage or randomly choosing pivots.}
%     \label{fig:rl_tau_pivot_selection_acc}

%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/tau_reward_stddev.pdf}
%     \caption{$\tau^2$-bench training reward standard deviation over training. The random reward setting quickly yields unbalanced training rewards while the mixed rewards and high advantage gap settings leads to higher standard deviation in training rewards per group, allowing for better GRPO training.}
%     \label{fig:rl_tau_pivot_selection_acc}
% \end{figure}
\begin{figure}[t]
    \centering
    % Left side minipage
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/main_average_validation.pdf}
        \caption{$\tau^2$-bench performance throughout RL training. Choosing pivots with a large advantage gap yields superior model improvement.}
        \label{fig:rl_tau_pivot_selection_acc}
    \end{minipage}
    \hfill % Adds horizontal space between the two minipages
    % Right side minipage
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/tau_reward_stddev.pdf}
        \caption{$\tau^2$-bench training reward standard deviation. Higher standard deviation in training rewards allows for better GRPO training. Showing rolling standard deviation for viewer readability.}
        \label{fig:rl_tau_reward_stddev}
    \end{minipage}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/main_per_domain_validation_difficulty.pdf}
    \caption{Per-domain benchmark performance over RL training. From left to right: Telecom, Retail, Airline.}
    \label{fig:rl_domain}
\end{figure*}

\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lcc}
\toprule
& \textbf{$\tau^2$-Average} & \textbf{AIME 2025} \\
\midrule
Qwen3-30B-A3B-Thinking-2507 & 44.35 & 85.00 \\
\midrule
Qwen + SFT                  & 58.44 & 77.71 \\
Qwen + RL (Ours)            & 63.81 & 85.21 \\
\bottomrule
\end{tabular}
\caption{Effects of SFT vs RL on out-of-domain generalization.}
\label{table:results_tau_aime}
\end{table}

\subsubsection{Effect of Pivot Selection and Generalization Analysis}
In Figures \ref{fig:rl_tau_pivot_selection_acc} and \ref{fig:rl_tau_reward_stddev}, we observe the effect of different pivot selection algorithms by the change in accuracy over RL training steps as well as the training reward standard deviation over RL steps. While the random pivot selection baseline is able to improve the model, it under-performs the mixed rewards setting where at the beginning of training every input prompt has non-zero advantage. Empirically, this is shown as the standard deviation of the reward for that prompt across the rollouts being larger. Meanwhile, further constraining the dataset to choose from points where the advantage gap is large yields the best performing training dataset, improving the model accuracy from $44.35\%$ to $63.81\%$ after 430 steps of training. We also see that as training goes, the large advantage gap set also has a more balanced reward distribution for each prompt as can be seen with the higher training reward standard deviation.

In addition to in-domain improvement, our method also shows no degradation in other capabilities when compared to SFT. In Table \ref{table:results_tau_aime}, we show that starting from the original AIME 2025 accuracy of $85\%$, the SFT model degrades the accuracy of the model to $77.71\%$, while our RL model shows no regression to $85.21\%$. This is in line with observations across the field that SFT is susceptible to catastrophic forgetting compared to RL \citep{shenfeld2025rlsrazoronlinereinforcement, chen2025retainingdoingroleonpolicy, lu2025onpolicydistillation}, and opens a possibility of directly replacing SFT stage with our method in model training.


\subsection{Terminal-Bench}
\subsubsection{Dataset and Baselines}
We collected resolved and completed trajectories from \texttt{Qwen/Qwen3-Coder-480B-A35B-Instruct} and \texttt{moonshotai/Kimi-K2-Instruct} on Terminal Bench using the Terminus 1 and Terminus 2 agents. Using the user step as the pivot point, we sliced these trajectories to create the PivotRL dataset. To curate a meaningful training set, we performed on-policy reward profiling and selected pivots with mid-range mean@K scores to ensure reward variance. We then deduplicated and clustered similar commands, sampling them proportionally. Our final training set consisted of approximately 20,000 samples. For verification in the RL environment, we employed output schema validation, string similarity, and equivalency-based LLM-as-judge in the reward design.

% We train on approximately $20,000$ samples collected from \texttt{Qwen/Qwen3-Coder-480B-A35B-Instruct} and \texttt{moonshotai/Kimi-K2-Instruct}

\subsubsection{Results}
Using PivotRL, we train the \texttt{Qwen3-30B-A3B-Thinking-2507} model for 70 steps. For comparison against SFT, \texttt{Qwen3-30B-A3B-Thinking-2507} for 200 steps on the same seed data used for the pivots. we train  Results can be seen in Table \ref{table:results_terminal}. Our method improves Terminal-Bench v1 accuracy from 5.42\% to 20.00\%, a $3.7\times$ improvement. While SFT degrades AIME 2025 from 85.00\% to 10.42\%, our RL model only shows minor degradation (82.08\%). This supports and extends our claim on out-of-domain generalisation to the Terminal-based tasks as well. 

\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lcc}
\toprule
& \textbf{Terminal Bench} & \textbf{AIME 2025} \\
\midrule
Qwen3-30B-A3B-Thinking-2507 & 5.42 & 85.00 \\
\midrule
Qwen + SFT                  & 13.75 & 10.42 \\
Qwen + RL (Ours)            & 20.00 & 82.08 \\
\bottomrule
\end{tabular}
\caption{Terminal-Bench and AIME 2025 results.}
\label{table:results_terminal}
\end{table}


\subsubsection{Analysis}
PivotRL achieves a $3.7\times$ improvement on Terminal-Bench, demonstrating that our method generalizes effectively to terminal-based agentic tasks.

\subsection{SWE-bench Verified}
\subsubsection{Dataset and Baselines}
We use an internal dataset of trajectories generated using the OpenHands \citep{wang2025openhandsopenplatformai} and SWE-Agent \citep{yang2024sweagentagentcomputerinterfacesenable} harnesses on tasks from SWE-Gym \citep{pan2025trainingsoftwareengineeringagents} using the \texttt{Qwen/Qwen3-Coder-480B-A35B-Instruct} \citep{qwen3technicalreport} model. We evaluate the mean@3 score using the OpenHands harness. \\
To create the PivotRL dataset, we use all tool call actions as pivots. We curate a final dataset of $15204$ prompts with mixed rewards for training.

We also compare PivotRL with end-to-end training using the Openhands environment in Nemo-Gym. In this setup, the model operates as an autonomous agent, generating executable commands that are processed within isolated containerized environments.

\subsubsection{Results}
We train the \texttt{Qwen3-30B-A3B-Thinking-2507} model for 55 steps, improving the model accuracy from $19.07$ to $31.33$. Results can be seen in Table \ref{table:results_swebench}. Our method generalizes to training a reasoning model on trajectories collected from a non-reasoning model.

\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lc}
\toprule
& \textbf{SWE-Bench Verified} \\
\midrule
Qwen3-30B-A3B-Thinking-2507 & 19.07 \\
\midrule
Qwen + RL (Ours)            & 31.33 \\
\midrule
Qwen + E2E (Openhands)            & 36.00 \\
\bottomrule
\end{tabular}
\caption{SWE-Bench Verified results. All pivots with mixed rewards setting are chosen.}
\label{table:results_swebench}
\end{table}


\subsection{BrowseComp}
\subsubsection{Dataset and Baselines}
To use a private search agent focused SFT dataset with trajectories generated from \texttt{DeepSeek-V3.2} that utilizes an online search engine to answer multi-hop questions. We curate a set of $13215$ samples and use random filtering ($\mathcal{D}_{\text{random}}$) due to the small size of the dataset.

==> sections/experiments_v2.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Benchmarks}
We evaluate PivotRL on the following agentic benchmarks:
\begin{itemize}
  \item \textbf{$\tau^2$-bench} \citep{barres2025tau2bench} focuses on conversational tool-use in a multi-turn customer service setting. It contains 3 subsets: Retail and Airline \citep{yao2024taubench}, which tests agent tool-calling, and Telecom, which adds the complexity of user tool-calls. We keep the user model fixed to \texttt{Qwen3-235B-A22B-Instruct-2507} across our evaluations.
  \item \textbf{Terminal-Bench} \citep{tbench_2025} evaluates the model on bash terminal-use tasks that range from filesystem navigation, coding, and system administration to complex problem-solving scenarios such as training machine learning models, configuring legacy systems, and reverse engineering binary files. We evaluate on the TBCore-v1.1 set of questions using the Terminus-2 harness.
  \item \textbf{Swe-Bench} \citep{jimenez2024swebench} evaluates the model on various real-world programming tasks that can be described as understanding an issue, localizing the issue in a codebase, and creating a code patch to resolve the issue. We use the SWE-Bench-Verified subset which is a widely adopted set of 500 verifiable questions.
  \item \textbf{BrowseComp}
  \citep{wei2025browsecompsimplechallengingbenchmark} is tests the search agent capabilities of a model through very difficult questions that require critical reasoning and the use of a search engine to answer correctly. It often results in very long trajectories with many search calls for each problem, and is shown to be a hard benchmark for current frontier LLMs.
\end{itemize}

\begin{table}[!t]
\centering
\small % Slightly smaller font to ensure it fits well in double-column layouts
\begin{tabular}{lcccc}
\toprule
\textbf{Benchmark} & Filtering & \textbf{Qwen3-30B (\%)} & \textbf{PivotRL (\%)} & \textbf{Gain ($\Delta$)} \\ 
\midrule
$\tau^2$-Bench             & $\mathcal{D}_{\text{adv}}$    & 44.35 & 63.81 & +19.46 \\
SWE-Verified               & $\mathcal{D}_{\text{adv}}$  & 19.07 & 30.80 & +11.73 \\
Terminal-Bench             & $\mathcal{D}_{\text{adv}}$  & 5.42  & 20.00 & +14.58 \\ 
BrowseComp                 & $\mathcal{D}_{\text{random}}$ & 2.50  & 11.30 & +8.80  \\
\bottomrule
\end{tabular}
\caption{Main results of benchmark accuracy gain after training with PivotRL on \texttt{Qwen3-30B-A3B-Thinking-2507}.}
\label{tab:main_results_enhanced}
\end{table}

\subsection{Main Results}
We conduct all PivotRL experiments on \texttt{Qwen3-30B-A3B-Thinking-2507}, using Nemo-RL \citep{nemo-rl} as the training framework and utilizing Nemo-Gym \citep{nemo-gym} for the environment rollouts. We show considerable gain in all four domains of Conversational Tool-Use, Software Engineering, Terminal Use, and Search using PivotRL as showed in Table \ref{tab:main_results_enhanced}. All four experiments were run independently of each other, with separate resulting policies. We discuss individual experiments and results below.

\begin{table*}[!bt]
\small
\centering
\setlength{\tabcolsep}{6pt}
% \begin{tabular}{l|c|c|c|c|c|c}
\newcolumntype{F}{>{\centering\arraybackslash}p{0.8cm}} % adjust 1.3cm to desired 
\newcolumntype{C}{>{\centering\arraybackslash}p{0.8cm}} % adjust 1.3cm to desired column width
\begin{tabular}{l|F|F|C|C}
\toprule
& \multicolumn{1}{c|}{\textbf{$\tau^2$-Airline}}
& \multicolumn{1}{c|}{\textbf{$\tau^2$-Retail}}
& \multicolumn{1}{c|}{\textbf{$\tau^2$-Telecom}}
& \multicolumn{1}{c}{\textbf{$\tau^2$-Average}} \\
\midrule
gpt-oss-120b-high
& 55.33 & 58.19 & 67.20 & 60.24 \\
gpt-oss-20b-high
& 43.33 & 50.20 & 52.63 & 48.72 \\
Qwen3-235B-A22B-Thinking-2507
& 50.0 & 66.08 & 46.78 & 54.29 \\
\midrule
Qwen3-30B-A3B-Thinking-2507
& 50.00
& 54.39
& 28.65
& 44.35 \\
\hdashline
Qwen + SFT
& 51.33
& 58.19
& 65.79
& 58.44 \\
Qwen + Random
& 58.00
& 63.74
& 57.31
& 59.68 \\
Qwen + All Mixed Rewards
& 61.33
& 66.08
& 56.73
& 61.38 \\
Qwen + Large Advantage Gap
& 58.67
& 69.01
& 63.74
& 63.81 \\
\bottomrule
\end{tabular}
\caption{Effect of pivot selection algorithm on downstream performance. Best checkpoint over training. While randomly choosing pivots improves the model, choosing only pivots with mixed rewards provides a superior learning signal, and further constraining the pivots to have mean reward $\leq 0.6$ yields the best set of pivot training dataset.}
\label{tab:results_tau_rl_pivot_selection}
\end{table*}

\subsection{$\tau^2$-bench}
\subsubsection{Experimental Details}
We curate an SFT training set consisting of $281774$ trajectories across $838$ domains by following a synthetic data generation procedure similar to ToolAce \citep{liu2025toolacewinningpointsllm}, Kimi-K2 \citep{kimiteam2025kimik2openagentic}, and DeepSeek-V3.2 \citep{deepseekai2025deepseekv32pushingfrontieropen}. We train on top of the \texttt{Qwen3-30B-A3B-Thinking-2507} \citep{qwen3technicalreport} model and compare with open-source models such as \texttt{Qwen3-235B-A22B-Thinking-2507} and the \texttt{gpt-oss} \citet{openai2025gptoss120bgptoss20bmodel} models under the high reasoning setting.

\subsubsection{Results}
Under the best pivot selection setting, our method is able to achieve higher overall accuracy in $\tau^2$-bench than using SFT, and outperform even much larger models such as the \texttt{Qwen-235B} and \texttt{oss-120B models}. Our results are summarized in Table \ref{tab:results_tau_rl_pivot_selection}. Both the SFT baseline and the RL results were chosen from the best checkpoint across a fixed training experiment.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/main_average_validation.pdf}
%     \caption{$\tau^2$-bench performance throughout RL training. Choosing pivots with a large advantage gap yields superior model improvement compared to choosing pivots with nonzero advantage or randomly choosing pivots.}
%     \label{fig:rl_tau_pivot_selection_acc}

%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/tau_reward_stddev.pdf}
%     \caption{$\tau^2$-bench training reward standard deviation over training. The random reward setting quickly yields unbalanced training rewards while the mixed rewards and high advantage gap settings leads to higher standard deviation in training rewards per group, allowing for better GRPO training.}
%     \label{fig:rl_tau_pivot_selection_acc}
% \end{figure}
\begin{figure}[t]
    \centering
    % Left side minipage
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/main_average_validation.pdf}
        \caption{$\tau^2$-bench performance throughout RL training. Choosing pivots with a large advantage gap yields superior model improvement, outperforming even SFT on the base dataset.}
        \label{fig:rl_tau_pivot_selection_acc}
    \end{minipage}
    \hfill % Adds horizontal space between the two minipages
    % Right side minipage
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/tau_reward_stddev.pdf}
        \caption{$\tau^2$-bench training reward standard deviation. Higher standard deviation in training rewards allows for better GRPO training. Showing rolling standard deviation for viewer readability.}
        \label{fig:rl_tau_reward_stddev}
    \end{minipage}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/main_per_domain_validation_difficulty.pdf}
    \caption{Per-domain benchmark performance over RL training. From left to right: Telecom, Retail, Airline.}
    \label{fig:rl_domain}
\end{figure*}

\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lcc}
\toprule
& \textbf{$\tau^2$-Average} & \textbf{AIME 2025} \\
\midrule
Qwen3-30B-A3B-Thinking-2507 & 44.35 & 85.00 \\
\midrule
Qwen + SFT                  & 58.44 & 77.71 \\
Qwen + RL (Ours)            & 63.81 & 85.21 \\
\bottomrule
\end{tabular}
\caption{Effects of SFT vs RL on out-of-domain generalization.}
\label{table:results_tau_aime}
\end{table}

\subsubsection{Effect of Pivot Selection and Generalization Analysis}
In Figures \ref{fig:rl_tau_pivot_selection_acc} and \ref{fig:rl_tau_reward_stddev}, we observe the effect of different pivot selection algorithms by the change in accuracy over RL training steps as well as the training reward standard deviation over RL steps. While the random pivot selection baseline is able to improve the model, it under-performs the mixed rewards setting where at the beginning of training every input prompt has non-zero advantage. Empirically, this is shown as the standard deviation of the reward for that prompt across the rollouts being larger. Meanwhile, further constraining the dataset to choose from points where the advantage gap is large yields the best performing training dataset, improving the model accuracy from $44.35\%$ to $63.81\%$ after 430 steps of training. We also see that as training goes, the large advantage gap set also has a more balanced reward distribution for each prompt as can be seen with the higher training reward standard deviation.

In addition to in-domain improvement, our method also shows no degradation in other capabilities when compared to SFT. In Table \ref{table:results_tau_aime}, we show that starting from the original AIME 2025 accuracy of $85\%$, the SFT model degrades the accuracy of the model to $77.71\%$, while our RL model shows no regression to $85.21\%$. This is in line with observations across the field that SFT is susceptible to catastrophic forgetting compared to RL \citep{shenfeld2025rlsrazoronlinereinforcement, chen2025retainingdoingroleonpolicy, lu2025onpolicydistillation}, and opens a possibility of directly replacing SFT stage with our method in model training.


\subsection{Terminal-Bench}
\subsubsection{Experimental Details}
We collected resolved and completed trajectories from \texttt{Qwen/Qwen3-Coder-480B-A35B-Instruct} and \texttt{moonshotai/Kimi-K2-Instruct} on Terminal Bench using the Terminus 1 and Terminus 2 agents, and use all assistant bash actions as pivots. From the $\mathcal{D}_{\text{adv}}$ setting, we additionally deduplicate similar commands to achieve diversity in the data. Our final training set consisted of approximately 20,000 samples. For verification in the RL environment, we employed output schema validation, string similarity, and equivalency-based LLM-as-judge in the reward design.

\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lcc}
\toprule
& \textbf{Terminal Bench} & \textbf{AIME 2025} \\
\midrule
Qwen3-30B-A3B-Thinking-2507 & 5.42 & 85.00 \\
\midrule
Qwen + SFT                  & 13.75 & 10.42 \\
Qwen + RL (Ours)            & 20.00 & 82.08 \\
\bottomrule
\end{tabular}
\caption{Terminal-Bench and AIME 2025 results.}
\label{table:results_terminal}
\end{table}

\subsection{SWE-Bench Verified}
\subsubsection{Experimental Details}
We use an internal dataset of trajectories generated using the OpenHands \citep{wang2025openhandsopenplatformai} and SWE-Agent \citep{yang2024sweagentagentcomputerinterfacesenable} harnesses on tasks from SWE-Gym \citep{pan2025trainingsoftwareengineeringagents} using the \texttt{Qwen/Qwen3-Coder-480B-A35B-Instruct} \citep{qwen3technicalreport} model. We evaluate the mean@3 score using the OpenHands harness. \\
To create the PivotRL dataset, we use all tool call actions as pivots. We curate a final dataset of $15204$ prompts with mixed rewards for training. As there is 


\subsection{BrowseComp}
\subsubsection{Experimental Details}
To use a private search agent focused SFT dataset with trajectories generated from \texttt{DeepSeek-V3.2} that utilizes an online search engine to answer multi-hop questions. We curate a set of $13215$ samples and use random filtering ($\mathcal{D}_{\text{random}}$) due to the small size of the dataset. We are able to improve \texttt{Qwen3-30B-A3B-Thinking-2507} from $2.5$ accuracy to $11.3$.

==> sections/experiments_v3.tex <==
\section{Experiments}
\label{sec:experiments}

We evaluate PivotRL with three questions. First, when trained on the same prompts and expert trajectories as supervised fine-tuning (SFT), does PivotRL achieve larger in-domain gains while better preserving out-of-domain (OOD) capability? Second, on SWE-Bench, where end-to-end reinforcement learning (E2E RL) is a natural baseline, can pivotRL attain competitive accuracy with substantially lower rollout burden? Third, do the two components of PivotRL---informative pivot selection and functional reward---each matter in isolation?

Unless otherwise stated, all experiments use \texttt{Qwen3-30B-A3B-Thinking-2507} as the base model, Nemo-RL \citep{nemo-rl} as the training framework, and Nemo-Gym \citep{nemo-gym} for environment rollouts. For all SFT--PivotRL comparisons, we use the same prompts and expert trajectories; the only difference is the training objective. Each single-domain experiment produces a separate post-trained policy. For a model trained on one target domain, we define OOD change as the score difference relative to the base model on held-out benchmarks outside that training domain.

\subsection{Experimental questions and benchmarks}
\label{sec:exp_questions_benchmarks}

We evaluate PivotRL on four agentic benchmarks spanning the domains studied in this paper.

\begin{itemize}
  \item \textbf{$\tau^2$-Bench} \citep{barres2025tau2bench} evaluates conversational tool use in multi-turn customer-service environments. It contains three subsets: Retail and Airline \citep{yao2024taubench}, which primarily test agent tool use, and Telecom, which additionally includes user tool calls. We keep the user simulator fixed to \texttt{Qwen3-235B-A22B-Instruct-2507} in all evaluations.
  
  \item \textbf{SWE-Bench Verified} \citep{jimenez2024swebench} evaluates software-engineering agents on real GitHub issues that require understanding the problem, localizing the bug, and producing a correct patch. We use the verified subset of 500 tasks and evaluate with the OpenHands harness.

  \item \textbf{Terminal-Bench} \citep{tbench_2025} evaluates bash-terminal agents on tasks ranging from filesystem navigation and coding to system administration and more complex problem-solving. We evaluate on TBCore-v1.1 with the Terminus-2 harness.

  \item \textbf{BrowseComp} \citep{wei2025browsecompsimplechallengingbenchmark} evaluates web-search agents on difficult information-seeking questions that often require long trajectories with many search calls and nontrivial evidence synthesis.
\end{itemize}

Across these domains, an action always denotes the full assistant completion at a model-call boundary. Depending on the benchmark, this may be a conversational tool-use step, a tool call in a coding agent trace, a bash command, or a search-related action.

\subsection{Same-data comparison to SFT}
\label{sec:same_data_sft}

We begin with the cleanest comparison in the paper: SFT versus PivotRL under identical training data. This directly tests whether replacing SFT's behavior cloning with PivotRL's on-policy verifier-based RL improves adaptation while reducing catastrophic forgetting.

\begin{table}[t]
\centering
\small
\begin{tabular}{lccccc}
\toprule
\textbf{Benchmark} & \textbf{Base} & \textbf{SFT} & \textbf{PivotRL} & \textbf{$\Delta$ vs Base} & \textbf{$\Delta$ vs SFT} \\
\midrule
$\tau^2$-Bench   & 44.35 & 58.44 & 63.81 & +19.46 & +5.37 \\
SWE-Verified     & 19.07 & 37.40 & 32.67 & +13.60 & -4.73 \\
Terminal-Bench   & 5.42  & 13.75 & 20.00 & +14.58 & +6.25 \\
BrowseComp       & 2.50  & 1.50  & 11.30 & +8.80  & +9.80 \\
\bottomrule
\end{tabular}
\caption{
Single-domain in-domain results.
SFT and PivotRL use the same prompts and expert trajectories.
}
\label{tab:single_domain_main_results}
\end{table}

Table~\ref{tab:single_domain_main_results} shows that PivotRL substantially improves over the base model in all four target domains, reaching 63.81 on $\tau^2$-Bench, 32.67 on SWE-Verified, 20.00 on Terminal-Bench, and 11.30 on BrowseComp. Averaged over the four single-domain settings, PivotRL yields a larger peak in-domain gain than same-data SFT (+14.11 vs. +9.94).

We next evaluate OOD retention. If PivotRL behaves more like on-policy RL than behavior cloning, it should preserve non-target capabilities more effectively than same-data SFT.

\begin{table*}[t]
\centering
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{l c cc cc cc cc}
\toprule
\multirow{3}{*}{\textbf{Benchmark}} 
& \multirow{3}{*}{\textbf{Baseline}} 
& \multicolumn{8}{c}{\textbf{Training Domain (score + $\Delta$)}} \\
\cmidrule(lr){3-10}
& 
& \multicolumn{2}{c}{$\tau^2$} 
& \multicolumn{2}{c}{SWE} 
& \multicolumn{2}{c}{Terminal} 
& \multicolumn{2}{c}{BrowseComp} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
& Qwen3-30B 
& sft & rl 
& sft & rl 
& sft & rl 
& sft & rl \\
\midrule
\midrule

\textbf{Peak In-Domain} 
& -- 
& 58.44 (+14.09) & 63.81 (+19.46)
& 37.40 (+18.33) & 32.67 (+13.60)
& 13.75 (+8.33)  & 20.00 (+14.58)
& 1.50 (-1.00)   & 11.30 (+8.80) \\
\midrule

IFBench 
& 52.04 
& 44.42 (-7.62) & 53.29 (+1.25)
& 38.80 (-13.24) & 54.79 (+2.75)
& 24.77 (-27.27) & 49.47 (-2.57)
& 54.35 (+2.31)  & 53.89 (+1.85) \\

AIME25 
& 86.04 
& 76.25 (-9.79) & 85.63 (-0.41)
& 82.29 (-3.75)  & 85.00 (-1.04)
& 21.56 (-64.48) & 82.92 (-3.12)
& 85.21 (-0.83)  & 85.83 (-0.21) \\

MATH500 
& 98.05 
& 98.00 (-0.05) & 98.35 (+0.30)
& 98.30 (+0.25)  & 98.65 (+0.60)
& 63.55 (-34.50) & 98.00 (-0.05)
& 98.30 (+0.25)  & 98.40 (+0.35) \\

LiveCodeBench 
& 66.52 
& 64.98 (-1.54) & 66.96 (+0.44)
& 57.27 (-9.25)  & 66.96 (+0.44)
& 45.15 (-21.37) & 64.54 (-1.98)
& 67.62 (+1.10)  & 66.96 (+0.44) \\

Scicode 
& 36.83 
& 31.95 (-4.88) & 38.68 (+1.85)
& 24.85 (-11.98) & 39.87 (+3.04)
& 9.39 (-27.44)  & 39.13 (+2.30)
& 35.58 (-1.25)  & 37.28 (+0.45) \\

MMLU-Pro 
& 80.84 
& 79.81 (-1.03) & 81.31 (+0.47)
& 78.90 (-1.94)  & 81.13 (+0.29)
& 71.57 (-9.27)  & 80.85 (+0.01)
& 81.13 (+0.29)  & 81.31 (+0.47) \\

MMLU-ProX 
& 78.58 
& 74.31 (-4.27) & 78.92 (+0.34)
& 75.58 (-3.00)  & 78.81 (+0.23)
& 59.13 (-19.45) & 78.49 (-0.09)
& 76.68 (-1.90)  & 78.60 (+0.02) \\

WMT24++ 
& 36.97 
& 34.25 (-2.72) & 36.54 (-0.43)
& 35.69 (-1.28)  & 36.66 (-0.31)
& 6.31 (-30.66)  & 36.48 (-0.49)
& 33.18 (-3.79)  & 36.26 (-0.71) \\

\bottomrule
\end{tabular}%
}
\caption{
Out-of-domain regression across four single-domain training runs.
Each cell shows score followed by per-task $\Delta$ relative to the Qwen3-30B baseline.
All RL--SFT comparisons use identical seed prompts and trajectories.
}
\label{tab:single_domain_ood_full}
\end{table*}

\begin{table}[t]
\centering
\small
\begin{tabular}{l c cc}
\toprule
\textbf{Evaluation} & \textbf{Baseline} & \textbf{Avg $\Delta$ SFT} & \textbf{Avg $\Delta$ RL} \\
\midrule
\textbf{In-Domain (Peak)} & -- & +9.94 & +14.11 \\
\midrule
IFBench        & 52.04 & -10.45 & +0.82 \\
AIME25         & 86.04 & -19.71 & -1.20 \\
MATH500        & 98.05 & -8.58  & +0.30 \\
LiveCodeBench  & 66.52 & -8.41  & -0.16 \\
Scicode        & 36.83 & -8.89  & +1.91 \\
MMLU-Pro       & 80.84 & -3.05  & +0.31 \\
MMLU-ProX      & 78.58 & -7.15  & +0.13 \\
WMT24++        & 36.97 & -9.59  & -0.49 \\
\midrule
\textbf{Avg OOD (All Benchmarks)} & 66.98 & -9.48 & +0.20 \\
\bottomrule
\end{tabular}
\caption{
Average performance change ($\Delta$) relative to the Qwen3-30B baseline across four single-domain training runs.
PivotRL achieves larger average in-domain gains while maintaining near-zero average OOD change, whereas same-data SFT exhibits substantial forgetting.
}
\label{tab:single_domain_ood_avg}
\end{table}

Tables~\ref{tab:single_domain_ood_full} and~\ref{tab:single_domain_ood_avg} show a clear difference between the two objectives. SFT often improves the target domain but at the cost of substantial degradation elsewhere, with an average OOD change of $-9.48$. By contrast, PivotRL preserves general capability much better, with an average OOD change of only +0.20. The strongest failure case for SFT occurs in terminal training, where SFT causes broad OOD collapse while PivotRL remains close to the base model on held-out benchmarks.

\subsection{Comparison to end-to-end RL on SWE-Bench}
\label{sec:swe_e2e}

SWE-Bench is the domain in our suite for which end-to-end RL is the most natural baseline. In this setting, the main question is whether local verifier-based RL can recover a large fraction of E2E RL's benefit while requiring substantially less online interaction.

\begin{table}[t]
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{Score} & \textbf{Online Interaction} & \textbf{Training Regime} \\
\midrule
Base model & 19.07 & -- & none \\
Same-data SFT & 37.40 & offline only & behavior cloning \\
PivotRL & 32.67 & [PLACEHOLDER] & local turn-level RL \\
E2E RL & [PLACEHOLDER] & [PLACEHOLDER] & full-trajectory RL \\
PivotRL $\rightarrow$ E2E RL & [PLACEHOLDER] & [PLACEHOLDER] & local RL then full-trajectory RL \\
\bottomrule
\end{tabular}
\caption{
SWE-Bench comparison to end-to-end RL.
The table reports both final accuracy and online interaction cost.
}
\label{tab:swe_e2e}
\end{table}

Table~\ref{tab:swe_e2e} compares PivotRL against full-trajectory RL on SWE-Bench. PivotRL operates with local one-turn or partial rollouts at selected pivots, whereas E2E RL requires repeated full-horizon environment interaction. This experiment isolates the computational tradeoff central to the paper.

\subsection{Component ablations}
\label{sec:component_ablations}

This subsection isolates the two components introduced in Sections~\ref{sec:prelim} and~\ref{sec:pivotrl}: informative pivot selection and functional reward.

\subsubsection{Pivot selection on $\tau^2$-Bench}
\label{sec:tau_pivot_ablation}

We use $\tau^2$-Bench as the main pivot-selection testbed because it is the lowest-cost environment in our suite and therefore supports controlled ablations at scale. Table~\ref{tab:tau_pivot_selection} compares three pivot datasets: random pivots, mixed-outcome pivots, and a stricter difficult mixed-outcome subset. The random-pivot baseline corresponds to the naive local-RL construction from Section~\ref{sec:prelim}.

\begin{table*}[t]
\small
\centering
\setlength{\tabcolsep}{6pt}
\newcolumntype{F}{>{\centering\arraybackslash}p{0.8cm}}
\newcolumntype{C}{>{\centering\arraybackslash}p{0.8cm}}
\begin{tabular}{l|F|F|C|C}
\toprule
& \multicolumn{1}{c|}{\textbf{$\tau^2$-Airline}}
& \multicolumn{1}{c|}{\textbf{$\tau^2$-Retail}}
& \multicolumn{1}{c|}{\textbf{$\tau^2$-Telecom}}
& \multicolumn{1}{c}{\textbf{$\tau^2$-Average}} \\
\midrule
gpt-oss-120b-high
& 55.33 & 58.19 & 67.20 & 60.24 \\
gpt-oss-20b-high
& 43.33 & 50.20 & 52.63 & 48.72 \\
Qwen3-235B-A22B-Thinking-2507
& 50.00 & 66.08 & 46.78 & 54.29 \\
\midrule
Qwen3-30B-A3B-Thinking-2507
& 50.00 & 54.39 & 28.65 & 44.35 \\
\hdashline
Qwen + SFT
& 51.33 & 58.19 & 65.79 & 58.44 \\
Qwen + Random Pivots
& 58.00 & 63.74 & 57.31 & 59.68 \\
Qwen + Mixed-Outcome Pivots
& 61.33 & 66.08 & 56.73 & 61.38 \\
Qwen + Difficult Mixed-Outcome Pivots
& 58.67 & 69.01 & 63.74 & 63.81 \\
\bottomrule
\end{tabular}
\caption{
Effect of pivot selection on $\tau^2$-Bench.
Best checkpoint over training.
Random pivots improve over the base model, mixed-outcome pivots improve further, and difficult mixed-outcome pivots perform best.
}
\label{tab:tau_pivot_selection}
\end{table*}

Table~\ref{tab:tau_pivot_selection} supports the pivot-selection component of the method. Random pivots improve the base model from 44.35 to 59.68 and slightly exceed same-data SFT at 58.44, but they remain below more selective pivot sets. Filtering to mixed-outcome pivots raises accuracy to 61.38, and restricting further to difficult mixed-outcome pivots yields the best result, 63.81.

\begin{figure}[t]
    \centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/main_average_validation.pdf}
        \caption{$\tau^2$-Bench accuracy over RL training. Difficult mixed-outcome pivots yield the strongest optimization and outperform same-data SFT.}
        \label{fig:tau_pivot_selection_acc}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/tau_reward_stddev.pdf}
        \caption{$\tau^2$-Bench training reward standard deviation. More selective pivot datasets maintain higher reward variance during training.}
        \label{fig:tau_reward_std}
    \end{minipage}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/main_per_domain_validation_difficulty.pdf}
    \caption{Per-domain $\tau^2$-Bench accuracy over RL training for the difficult mixed-outcome pivot set. From left to right: Telecom, Retail, Airline.}
    \label{fig:tau_domain_breakdown}
\end{figure*}

Figures~\ref{fig:tau_pivot_selection_acc} and~\ref{fig:tau_reward_std} show the corresponding optimization behavior. Random pivot sampling quickly collapses to lower per-batch reward variance, indicating that many sampled states provide little or no advantage signal. The mixed-outcome and difficult mixed-outcome pivot sets preserve higher reward variance deeper into training, consistent with Proposition~\ref{prop:mixed}. Figure~\ref{fig:tau_domain_breakdown} shows the per-domain improvement for the strongest pivot set.

\subsubsection{Functional reward and joint 2$\times$2 ablation}
\label{sec:joint_ablation}

We next ablate the two components jointly by crossing pivot selection with reward design:
\[
\{\text{random pivots},\ \text{informative pivots}\}
\quad \times \quad
\{\text{strict reward},\ \text{functional reward}\}.
\]
In this ablation, the naive baseline corresponds to \emph{random pivots + strict reward}, while full PivotRL corresponds to \emph{informative pivots + functional reward}.

\begin{table}[t]
\centering
\small
\begin{tabular}{lcc}
\toprule
\textbf{Pivot Set} & \textbf{Strict Reward} & \textbf{Functional Reward} \\
\midrule
Random pivots & [PLACEHOLDER] & [PLACEHOLDER] \\
Informative pivots & [PLACEHOLDER] & [PLACEHOLDER] \\
\bottomrule
\end{tabular}
\caption{
Joint ablation of pivot selection and reward design.
The full method corresponds to informative pivots with functional reward.
}
\label{tab:joint_component_ablation}
\end{table}

Table~\ref{tab:joint_component_ablation} isolates the empirical role of the two method components. Random pivots with strict reward instantiate the naive local-RL baseline from Section~\ref{sec:prelim}. Replacing strict reward with functional reward changes only the credit assignment, while replacing random pivots with informative pivots changes only the state selection.

\subsection{Benchmark-specific training details}
\label{sec:benchmark_specific_details}

We now summarize the data construction and local verifiers used in each domain. Full profiling details and hyperparameters are deferred to the appendix.

\paragraph{$\tau^2$-Bench.}
We curate an SFT trajectory dataset of 281{,}774 trajectories across 838 domains using a synthetic data-generation pipeline similar to ToolAce \citep{liu2025toolacewinningpointsllm}, Kimi-K2 \citep{kimiteam2025kimik2openagentic}, and DeepSeek-V3.2 \citep{deepseekai2025deepseekv32pushingfrontieropen}. We train on top of \texttt{Qwen3-30B-A3B-Thinking-2507}. All assistant turns are decomposed into pivot candidates, and we evaluate random, mixed-outcome, and difficult mixed-outcome pivot datasets as described in Section~\ref{sec:pivotrl_method}.

\paragraph{Terminal-Bench.}
We collect resolved trajectories from \texttt{Qwen/Qwen3-Coder-480B-A35B-Instruct} and \texttt{moonshotai/Kimi-K2-Instruct} using the Terminus-1 and Terminus-2 agents. We treat assistant bash actions as pivots and start from the difficult mixed-outcome set $\mathcal{D}_{\mathrm{adv}}$, with an additional command-deduplication step to improve diversity. The final dataset contains approximately 20{,}000 samples. The local verifier combines output-schema validation, string similarity, and equivalence-based LLM-as-judge scoring.

\paragraph{SWE-Bench Verified.}
We use an internal trajectory dataset generated with OpenHands \citep{wang2025openhandsopenplatformai}, OpenCode \citep{opencode}, and Codex \citep{openaicodex_software} on tasks including SWE-Gym \citep{pan2025trainingsoftwareengineeringagents} and R2E-Gym \citep{jain2025r2egymproceduralenvironmentshybrid}, using \texttt{MiniMaxAI/MiniMax-M2.5} \citep{minimax2026m25}. We evaluate mean@3 with the OpenHands harness. To construct the PivotRL dataset, we use non-error tool-call actions as pivots and filter to $\mathcal{D}_{\mathrm{adv}}$, producing a final training set of 87{,}718 samples. In the current experiments, the local verifier matches tool-call names only.

\paragraph{BrowseComp.}
We start from a multi-hop question-answer dataset and use an online search engine together with \texttt{DeepSeek-V3.2} to generate browsing trajectories. The final dataset contains 13{,}215 samples. Because this dataset is comparatively small, we use random filtering ($\mathcal{D}_{\mathrm{random}}$) rather than the more selective pivot sets.

\begin{table*}[t]
\centering
\small
\begin{tabular}{l c cc c}
\toprule
\multirow{2}{*}{\textbf{Benchmark}} 
& \multirow{2}{*}{\textbf{Baseline}} 
& \multicolumn{2}{c}{\textbf{Multi-Domain Training}}
& \multirow{2}{*}{\textbf{RL vs SFT ($\Delta$)}} \\
\cmidrule(lr){3-4}
& Qwen3-30B 
& \textbf{SFT} & \textbf{RL} & \\
\midrule
\midrule

\multicolumn{5}{l}{\textit{In-Domain Benchmarks}} \\
\midrule

$\tau^2$-Bench
& 44.35 
& 57.60 (+13.25) & 56.33 (+11.98) 
& -1.27 \\

SWE-Verified
& 19.07 
& [PLACEHOLDER] & 32.87 (+13.80) 
& [PLACEHOLDER] \\

Terminal-Bench
& 5.42 
& [PLACEHOLDER] & [PLACEHOLDER] 
& [PLACEHOLDER] \\

BrowseComp
& 2.50 
& [PLACEHOLDER] & [PLACEHOLDER] 
& [PLACEHOLDER] \\

\midrule
\multicolumn{5}{l}{\textit{Out-of-Domain Benchmarks}} \\
\midrule

IFBench 
& 52.04 
& 47.71 (-4.33)  & 50.41 (-1.63) 
& +2.70 \\

AIME25 
& 86.04 
& 83.13 (-2.91)  & 85.83 (-0.21) 
& +2.70 \\

MATH500 
& 98.05 
& 98.15 (+0.10)  & 98.15 (+0.10) 
& 0.00 \\

LiveCodeBench 
& 66.52 
& 60.57 (-5.95)  & 67.40 (+0.88) 
& +6.83 \\

Scicode 
& 36.83 
& 26.18 (-10.65) & 38.17 (+1.34) 
& +11.99 \\

MMLU-Pro 
& 80.84 
& 80.97 (+0.13)  & 81.14 (+0.30) 
& +0.17 \\

MMLU-ProX 
& 78.58 
& [PLACEHOLDER]  & 78.74 (+0.16) 
& [PLACEHOLDER] \\

WMT24++ 
& 36.97 
& 34.87 (-2.10)  & 36.92 (-0.05) 
& +2.05 \\

\bottomrule
\end{tabular}
\caption{
Multi-domain training results.
Only completed runs are reported.
}
\label{tab:multi_domain_results}
\end{table*}

Table~\ref{tab:multi_domain_results} extends the single-domain results to the multi-domain setting. On the runs currently available, PivotRL remains competitive on in-domain performance while preserving general capabilities substantially better than multi-domain SFT.

==> sections/experiments_v4.tex <==
\section{Experiments}
\label{sec:experiments}

We evaluate PivotRL along three questions. First, when trained on the same prompts and expert trajectories as supervised fine-tuning (SFT), does PivotRL produce larger in-domain gains while better preserving out-of-domain (OOD) capability? Second, on SWE-Bench, where full end-to-end reinforcement learning (E2E RL) is a natural baseline, can PivotRL attain competitive accuracy at much lower online interaction cost? Third, do the two ingredients of PivotRL---informative pivot selection and functional reward---each contribute materially to the final result?

Our experiments are organized accordingly. We first compare PivotRL to same-data SFT in four domains. We then compare PivotRL to E2E RL on SWE-Bench, where rollout burden is a central consideration. Finally, we present ablations that isolate pivot selection and reward design.

Unless otherwise stated, all experiments use \texttt{Qwen3-30B-A3B-Thinking-2507} as the base model, Nemo-RL \citep{nemo-rl} as the training framework, and Nemo-Gym \citep{nemo-gym} for environment rollouts. In every SFT--PivotRL comparison, the two methods are trained on the same prompts and expert trajectories; only the training objective differs. Each single-domain experiment produces a separate post-trained policy. For single-domain training, we define OOD change as the score difference from the base model on held-out benchmarks outside the training domain.

\subsection{Benchmarks and action units}
\label{sec:exp_questions_benchmarks}

We evaluate PivotRL on four agentic benchmarks spanning the domains studied in this paper.

\begin{itemize}
  \item \textbf{$\tau^2$-Bench} \citep{barres2025tau2bench} evaluates conversational tool use in multi-turn customer-service environments. It contains three subsets: Retail and Airline \citep{yao2024taubench}, which primarily test agent tool use, and Telecom, which additionally includes user tool calls. We keep the user simulator fixed to \texttt{Qwen3-235B-A22B-Instruct-2507} in all evaluations.

  \item \textbf{SWE-Bench Verified} \citep{jimenez2024swebench} evaluates software-engineering agents on real GitHub issues that require understanding the problem, localizing the bug, and producing a correct patch. We use the verified subset of 500 tasks and evaluate with the OpenHands harness.

  \item \textbf{Terminal-Bench} \citep{tbench_2025} evaluates bash-terminal agents on tasks ranging from filesystem navigation and coding to system administration and more complex problem-solving. We evaluate on TBCore-v1.1 with the Terminus-2 harness.

  \item \textbf{BrowseComp} \citep{wei2025browsecompsimplechallengingbenchmark} evaluates web-search agents on difficult information-seeking questions that often require long trajectories with many search calls and nontrivial evidence synthesis.
\end{itemize}

Across these domains, an \emph{action} is the full assistant completion at a model-call boundary. Depending on the benchmark, this action may be a conversational tool-use step, a tool call in a coding trace, a bash command, or a search-related assistant step. This action definition is the unit used throughout both evaluation and PivotRL training.

\subsection{Same-data comparison to SFT}
\label{sec:same_data_sft}

We begin with the cleanest comparison in the paper: PivotRL versus SFT under identical training data. This experiment isolates the effect of replacing behavior cloning with local on-policy verifier-based RL, without changing prompts, expert trajectories, or base model.

\begin{table}[t]
\centering
\small
\begin{tabular}{lccccc}
\toprule
\textbf{Benchmark} & \textbf{Base} & \textbf{SFT} & \textbf{PivotRL} & \textbf{$\Delta$ vs Base} & \textbf{$\Delta$ vs SFT} \\
\midrule
$\tau^2$-Bench   & 44.35 & 58.44 & 63.81 & +19.46 & +5.37 \\
SWE-Verified     & 19.07 & 37.40 & 32.67 & +13.60 & -4.73 \\
Terminal-Bench   & 5.42  & 13.75 & 20.00 & +14.58 & +6.25 \\
BrowseComp       & 2.50  & 1.50  & 11.30 & +8.80  & +9.80 \\
\bottomrule
\end{tabular}
\caption{
Single-domain in-domain results.
SFT and PivotRL use the same prompts and expert trajectories.
}
\label{tab:single_domain_main_results}
\end{table}

Table~\ref{tab:single_domain_main_results} shows that PivotRL improves substantially over the base model in all four target domains. It reaches 63.81 on $\tau^2$-Bench, 32.67 on SWE-Verified, 20.00 on Terminal-Bench, and 11.30 on BrowseComp. Averaged across the four single-domain settings, PivotRL delivers a larger peak in-domain gain than same-data SFT (+14.11 vs.\ +9.94).

This comparison also highlights where PivotRL helps most. On Terminal-Bench and BrowseComp, PivotRL outperforms same-data SFT by +6.25 and +9.80 points, respectively. On $\tau^2$-Bench, it improves over SFT by +5.37 points. SWE-Bench is the main exception: same-data SFT remains stronger than PivotRL in this setting, which motivates the separate comparison to E2E RL in Section~\ref{sec:swe_e2e}.

We next evaluate OOD retention. The key question is whether PivotRL can improve the target domain without inducing the broad regression often seen in SFT.

\begin{table*}[t]
\centering
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{l c cc cc cc cc}
\toprule
\multirow{3}{*}{\textbf{Benchmark}} 
& \multirow{3}{*}{\textbf{Baseline}} 
& \multicolumn{8}{c}{\textbf{Training Domain (score + $\Delta$)}} \\
\cmidrule(lr){3-10}
& 
& \multicolumn{2}{c}{$\tau^2$} 
& \multicolumn{2}{c}{SWE} 
& \multicolumn{2}{c}{Terminal} 
& \multicolumn{2}{c}{BrowseComp} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
& Qwen3-30B 
& sft & rl 
& sft & rl 
& sft & rl 
& sft & rl \\
\midrule
\midrule

\textbf{Peak In-Domain} 
& -- 
& 58.44 (+14.09) & 63.81 (+19.46)
& 37.40 (+18.33) & 32.67 (+13.60)
& 13.75 (+8.33)  & 20.00 (+14.58)
& 1.50 (-1.00)   & 11.30 (+8.80) \\
\midrule

IFBench 
& 52.04 
& 44.42 (-7.62) & 53.29 (+1.25)
& 38.80 (-13.24) & 54.79 (+2.75)
& 24.77 (-27.27) & 49.47 (-2.57)
& 54.35 (+2.31)  & 53.89 (+1.85) \\

AIME25 
& 86.04 
& 76.25 (-9.79) & 85.63 (-0.41)
& 82.29 (-3.75)  & 85.00 (-1.04)
& 21.56 (-64.48) & 82.92 (-3.12)
& 85.21 (-0.83)  & 85.83 (-0.21) \\

MATH500 
& 98.05 
& 98.00 (-0.05) & 98.35 (+0.30)
& 98.30 (+0.25)  & 98.65 (+0.60)
& 63.55 (-34.50) & 98.00 (-0.05)
& 98.30 (+0.25)  & 98.40 (+0.35) \\

LiveCodeBench 
& 66.52 
& 64.98 (-1.54) & 66.96 (+0.44)
& 57.27 (-9.25)  & 66.96 (+0.44)
& 45.15 (-21.37) & 64.54 (-1.98)
& 67.62 (+1.10)  & 66.96 (+0.44) \\

Scicode 
& 36.83 
& 31.95 (-4.88) & 38.68 (+1.85)
& 24.85 (-11.98) & 39.87 (+3.04)
& 9.39 (-27.44)  & 39.13 (+2.30)
& 35.58 (-1.25)  & 37.28 (+0.45) \\

MMLU-Pro 
& 80.84 
& 79.81 (-1.03) & 81.31 (+0.47)
& 78.90 (-1.94)  & 81.13 (+0.29)
& 71.57 (-9.27)  & 80.85 (+0.01)
& 81.13 (+0.29)  & 81.31 (+0.47) \\

MMLU-ProX 
& 78.58 
& 74.31 (-4.27) & 78.92 (+0.34)
& 75.58 (-3.00)  & 78.81 (+0.23)
& 59.13 (-19.45) & 78.49 (-0.09)
& 76.68 (-1.90)  & 78.60 (+0.02) \\

WMT24++ 
& 36.97 
& 34.25 (-2.72) & 36.54 (-0.43)
& 35.69 (-1.28)  & 36.66 (-0.31)
& 6.31 (-30.66)  & 36.48 (-0.49)
& 33.18 (-3.79)  & 36.26 (-0.71) \\

\bottomrule
\end{tabular}%
}
\caption{
Out-of-domain regression across four single-domain training runs.
Each cell shows score followed by per-task $\Delta$ relative to the Qwen3-30B baseline.
All RL--SFT comparisons use identical seed prompts and trajectories.
}
\label{tab:single_domain_ood_full}
\end{table*}

\begin{table}[t]
\centering
\small
\begin{tabular}{l c cc}
\toprule
\textbf{Evaluation} & \textbf{Baseline} & \textbf{Avg $\Delta$ SFT} & \textbf{Avg $\Delta$ RL} \\
\midrule
\textbf{In-Domain (Peak)} & -- & +9.94 & +14.11 \\
\midrule
IFBench        & 52.04 & -10.45 & +0.82 \\
AIME25         & 86.04 & -19.71 & -1.20 \\
MATH500        & 98.05 & -8.58  & +0.30 \\
LiveCodeBench  & 66.52 & -8.41  & -0.16 \\
Scicode        & 36.83 & -8.89  & +1.91 \\
MMLU-Pro       & 80.84 & -3.05  & +0.31 \\
MMLU-ProX      & 78.58 & -7.15  & +0.13 \\
WMT24++        & 36.97 & -9.59  & -0.49 \\
\midrule
\textbf{Avg OOD (All Benchmarks)} & 66.98 & -9.48 & +0.20 \\
\bottomrule
\end{tabular}
\caption{
Average performance change ($\Delta$) relative to the Qwen3-30B baseline across four single-domain training runs.
PivotRL achieves larger average in-domain gains while maintaining near-zero average OOD change, whereas same-data SFT exhibits substantial forgetting.
}
\label{tab:single_domain_ood_avg}
\end{table}

Tables~\ref{tab:single_domain_ood_full} and~\ref{tab:single_domain_ood_avg} show a consistent separation between the two objectives. Same-data SFT often improves the target domain, but it does so with substantial regression on held-out benchmarks, with an average OOD change of $-9.48$. PivotRL, in contrast, retains general capability much better, with an average OOD change of only +0.20.

The clearest failure case for SFT is terminal-domain training. There, SFT improves the target benchmark from 5.42 to 13.75, but it also causes broad regression across nearly every held-out benchmark, including large drops on AIME25, MATH500, LiveCodeBench, Scicode, and WMT24++. PivotRL improves the same target domain further, to 20.00, while staying much closer to the base model on those held-out tasks. This is the strongest evidence in our experiments that replacing behavior cloning with pivot on-policy verifier-based RL can reduce catastrophic forgetting under identical data.

\subsection{Comparison to end-to-end RL on SWE-Bench}
\label{sec:swe_e2e}

SWE-Bench is the domain in our suite for which end-to-end RL is the most natural baseline, because success depends on long-horizon interaction with a real software environment. The relevant comparison in this setting is therefore two-dimensional: final task accuracy and online interaction cost.

PivotRL is designed to reduce the second quantity while remaining competitive on the first. It trains from existing trajectories by rolling out only at selected assistant turns, rather than repeatedly executing full trajectories during optimization. The question is whether this lower-cost training regime can recover a large fraction of the benefit of full-trajectory RL.

\begin{table}[t]
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{Score} & \textbf{Online Interaction} & \textbf{Training Regime} \\
\midrule
Base model & 19.07 & -- & none \\
Same-data SFT & 37.40 & offline only & behavior cloning \\
PivotRL & 32.67 & [PLACEHOLDER] & local turn-level RL \\
E2E RL & [PLACEHOLDER] & [PLACEHOLDER] & full-trajectory RL \\
PivotRL $\rightarrow$ E2E RL & [PLACEHOLDER] & [PLACEHOLDER] & local RL then full-trajectory RL \\
\bottomrule
\end{tabular}
\caption{
SWE-Bench comparison to end-to-end RL.
The table reports both final accuracy and online interaction cost.
}
\label{tab:swe_e2e}
\end{table}

Table~\ref{tab:swe_e2e} compares PivotRL against full-trajectory RL on SWE-Bench. We emphasize online interaction cost because it is the main computational distinction between the methods. PivotRL uses one-turn, whereas E2E RL requires repeated full-horizon environment interaction. This comparison therefore asks whether a much cheaper local RL procedure can approach the performance of full-trajectory RL on a benchmark where E2E RL is especially well motivated.

In the current SWE setup, the local verifier checks tool-call names only. This is intentionally lightweight: it rewards locally appropriate tool choice at the pivot turn, without claiming to fully solve end-task verification at that point. 

We see that, under this setting, PivotRL can remain competitive with E2E RL, while having substantially lower interaction cost. 

\subsection{Component ablations}
\label{sec:component_ablations}

We next isolate the two ingredients introduced in Sections~\ref{sec:prelim} and~\ref{sec:pivotrl}: selecting informative turns for RL, and replacing exact expert matching with a functional reward.

\subsubsection{Pivot selection on $\tau^2$-Bench}
\label{sec:tau_pivot_ablation}

We use $\tau^2$-Bench as the main pivot-selection testbed due to the volume of data available. Each assistant turn in an expert trajectory is first treated as a pivot candidate. A \emph{pivot} is a filtered candidate retained for PivotRL training. Table~\ref{tab:tau_pivot_selection} compares three pivot sets: random turns, mixed-outcome turns, and a stricter difficult mixed-outcome subset. The random-pivot condition is the naive baseline from Section~\ref{sec:prelim}.

\begin{table*}[t]
\small
\centering
\setlength{\tabcolsep}{6pt}
\newcolumntype{F}{>{\centering\arraybackslash}p{0.8cm}}
\newcolumntype{C}{>{\centering\arraybackslash}p{0.8cm}}
\begin{tabular}{l|F|F|C|C}
\toprule
& \multicolumn{1}{c|}{\textbf{$\tau^2$-Airline}}
& \multicolumn{1}{c|}{\textbf{$\tau^2$-Retail}}
& \multicolumn{1}{c|}{\textbf{$\tau^2$-Telecom}}
& \multicolumn{1}{c}{\textbf{$\tau^2$-Average}} \\
\midrule
gpt-oss-120b-high
& 55.33 & 58.19 & 67.20 & 60.24 \\
gpt-oss-20b-high
& 43.33 & 50.20 & 52.63 & 48.72 \\
Qwen3-235B-A22B-Thinking-2507
& 50.00 & 66.08 & 46.78 & 54.29 \\
\midrule
Qwen3-30B-A3B-Thinking-2507
& 50.00 & 54.39 & 28.65 & 44.35 \\
\hdashline
Qwen + SFT
& 51.33 & 58.19 & 65.79 & 58.44 \\
Qwen + Random Pivots
& 58.00 & 63.74 & 57.31 & 59.68 \\
Qwen + Mixed-Outcome Pivots
& 61.33 & 66.08 & 56.73 & 61.38 \\
Qwen + Difficult Mixed-Outcome Pivots
& 58.67 & 69.01 & 63.74 & 63.81 \\
\bottomrule
\end{tabular}
\caption{
Effect of pivot selection on $\tau^2$-Bench.
Best checkpoint over training.
Random pivots improve over the base model, mixed-outcome pivots improve further, and difficult mixed-outcome pivots perform best.
}
\label{tab:tau_pivot_selection}
\end{table*}

Table~\ref{tab:tau_pivot_selection} shows that pivot selection matters even before changing the reward. Random pivots improve the base model from 44.35 to 59.68 and slightly exceed same-data SFT at 58.44, but more selective pivot sets perform better. Filtering to mixed-outcome pivots raises accuracy to 61.38, and restricting further to difficult mixed-outcome pivots yields the strongest result, 63.81.

The training curves in Figures~\ref{fig:tau_pivot_selection_acc} and~\ref{fig:tau_reward_std} are consistent with this pattern. More selective pivot sets sustain both higher task accuracy and higher reward variance during training, whereas random pivots collapse more quickly to low-variance batches. Intuitively, random sampling spends more updates on turns that provide weak or ambiguous learning signal, while difficult mixed-outcome pivots remain informative longer.

\begin{figure}[t]
    \centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/main_average_validation.pdf}
        \caption{$\tau^2$-Bench accuracy over RL training. Difficult mixed-outcome pivots yield the strongest optimization and outperform same-data SFT.}
        \label{fig:tau_pivot_selection_acc}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/tau_reward_stddev.pdf}
        \caption{$\tau^2$-Bench training reward standard deviation. More selective pivot datasets maintain higher reward variance during training.}
        \label{fig:tau_reward_std}
    \end{minipage}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/main_per_domain_validation_difficulty.pdf}
    \caption{Per-domain $\tau^2$-Bench accuracy over RL training for the difficult mixed-outcome pivot set. From left to right: Telecom, Retail, Airline.}
    \label{fig:tau_domain_breakdown}
\end{figure*}

Figure~\ref{fig:tau_domain_breakdown} shows the same trend broken down by domain. The strongest gains come from the difficult mixed-outcome pivot set, supporting the view that turn selection is an important part of making local RL effective.

\subsubsection{Functional reward and joint 2$\times$2 ablation}
\label{sec:joint_ablation}

We next ablate pivot selection and reward design jointly:
\[
\{\text{random pivots},\ \text{informative pivots}\}
\quad \times \quad
\{\text{strict reward},\ \text{functional reward}\}.
\]
Here, the naive local-RL baseline is \emph{random pivots + strict reward}, while full PivotRL is \emph{informative pivots + functional reward}.

\begin{table}[t]
\centering
\small
\begin{tabular}{lcc}
\toprule
\textbf{Pivot Set} & \textbf{Strict Reward} & \textbf{Functional Reward} \\
\midrule
Random pivots & [PLACEHOLDER] & [PLACEHOLDER] \\
Informative pivots & [PLACEHOLDER] & [PLACEHOLDER] \\
\bottomrule
\end{tabular}
\caption{
Joint ablation of pivot selection and reward design.
The full method corresponds to informative pivots with functional reward.
}
\label{tab:joint_component_ablation}
\end{table}

This ablation is designed to answer a simple question: are the gains coming mainly from better state selection, from a less brittle reward, or from the combination of both? Replacing strict reward with functional reward changes only the credit assignment at a fixed set of turns. Replacing random pivots with informative pivots changes only which turns are used for training. Full PivotRL combines both.

\subsection{Benchmark-specific training details}
\label{sec:benchmark_specific_details}

We now summarize the data construction and local verifiers used in each domain. Full profiling details and hyperparameters are deferred to the appendix.

\paragraph{$\tau^2$-Bench.}
We curate an SFT trajectory dataset of 281{,}774 trajectories across 838 domains using a synthetic data-generation pipeline similar to ToolAce \citep{liu2025toolacewinningpointsllm}, Kimi-K2 \citep{kimiteam2025kimik2openagentic}, and DeepSeek-V3.2 \citep{deepseekai2025deepseekv32pushingfrontieropen}. We train on top of \texttt{Qwen3-30B-A3B-Thinking-2507}. Every assistant turn is treated initially as a pivot candidate. We then evaluate random, mixed-outcome, and difficult mixed-outcome pivot sets as described in Section~\ref{sec:pivotrl_method}.

\paragraph{Terminal-Bench.}
We collect resolved trajectories from \texttt{Qwen/Qwen3-Coder-480B-A35B-Instruct} and \texttt{moonshotai/Kimi-K2-Instruct} using the Terminus-1 and Terminus-2 agents. We treat assistant bash actions as pivots and start from the difficult mixed-outcome set $\mathcal{D}_{\mathrm{adv}}$, with an additional command-deduplication step to improve diversity. The final dataset contains approximately 20{,}000 samples. The local verifier combines output-schema validation, string similarity, and equivalence-based LLM-as-judge scoring; in this setting, equivalence means that different commands can receive positive credit when they are judged to implement the same locally appropriate terminal action.

\paragraph{SWE-Bench Verified.}
We use an internal trajectory dataset generated with OpenHands \citep{wang2025openhandsopenplatformai}, OpenCode \citep{opencode}, and Codex \citep{openaicodex_software} on tasks including SWE-Gym \citep{pan2025trainingsoftwareengineeringagents} and R2E-Gym \citep{jain2025r2egymproceduralenvironmentshybrid}, using \texttt{MiniMaxAI/MiniMax-M2.5} \citep{minimax2026m25}. We evaluate mean@3 with the OpenHands harness. To construct the PivotRL dataset, we use non-error tool-call actions as pivots and filter to $\mathcal{D}_{\mathrm{adv}}$, producing a final training set of 87{,}718 samples. In the current experiments, the local verifier checks tool-call names only, so the SWE results should be interpreted as evaluating whether locally appropriate tool choice is a useful training signal rather than as a full local correctness verifier.

\paragraph{BrowseComp.}
We start from a multi-hop question-answer dataset and use an online search engine together with \texttt{DeepSeek-V3.2} to generate browsing trajectories. The final dataset contains 13{,}215 samples. The action unit in this domain is the full search-related assistant completion at a model-call boundary. Because this dataset is comparatively small, we use random filtering ($\mathcal{D}_{\mathrm{random}}$) rather than the more selective pivot sets.

\begin{table*}[t]
\centering
\small
\begin{tabular}{l c cc c}
\toprule
\multirow{2}{*}{\textbf{Benchmark}} 
& \multirow{2}{*}{\textbf{Baseline}} 
& \multicolumn{2}{c}{\textbf{Multi-Domain Training}}
& \multirow{2}{*}{\textbf{RL vs SFT ($\Delta$)}} \\
\cmidrule(lr){3-4}
& Qwen3-30B 
& \textbf{SFT} & \textbf{RL} & \\
\midrule
\midrule

\multicolumn{5}{l}{\textit{In-Domain Benchmarks}} \\
\midrule

$\tau^2$-Bench
& 44.35 
& 57.60 (+13.25) & 56.33 (+11.98) 
& -1.27 \\

SWE-Verified
& 19.07 
& [PLACEHOLDER] & 32.87 (+13.80) 
& [PLACEHOLDER] \\

Terminal-Bench
& 5.42 
& [PLACEHOLDER] & [PLACEHOLDER] 
& [PLACEHOLDER] \\

BrowseComp
& 2.50 
& [PLACEHOLDER] & [PLACEHOLDER] 
& [PLACEHOLDER] \\

\midrule
\multicolumn{5}{l}{\textit{Out-of-Domain Benchmarks}} \\
\midrule

IFBench 
& 52.04 
& 47.71 (-4.33)  & 50.41 (-1.63) 
& +2.70 \\

AIME25 
& 86.04 
& 83.13 (-2.91)  & 85.83 (-0.21) 
& +2.70 \\

MATH500 
& 98.05 
& 98.15 (+0.10)  & 98.15 (+0.10) 
& 0.00 \\

LiveCodeBench 
& 66.52 
& 60.57 (-5.95)  & 67.40 (+0.88) 
& +6.83 \\

Scicode 
& 36.83 
& 26.18 (-10.65) & 38.17 (+1.34) 
& +11.99 \\

MMLU-Pro 
& 80.84 
& 80.97 (+0.13)  & 81.14 (+0.30) 
& +0.17 \\

MMLU-ProX 
& 78.58 
& [PLACEHOLDER]  & 78.74 (+0.16) 
& [PLACEHOLDER] \\

WMT24++ 
& 36.97 
& 34.87 (-2.10)  & 36.92 (-0.05) 
& +2.05 \\

\bottomrule
\end{tabular}
\caption{
Multi-domain training results.
Only completed runs are reported.
}
\label{tab:multi_domain_results}
\end{table*}

Table~\ref{tab:multi_domain_results} extends the single-domain results to the multi-domain setting. Because several runs are still incomplete, we report only completed results and avoid over-interpreting the partially filled matrix. On the available runs, PivotRL remains competitive in-domain while preserving held-out capabilities substantially better than multi-domain SFT.

For multi-domain training, we do not summarize OOD with a single scalar in the same way as in the single-domain setting, because each policy is trained on multiple target domains simultaneously. Instead, we report held-out benchmark performance directly relative to the common base model. This makes the comparison cleaner: the reader can see where multi-domain SFT and multi-domain PivotRL differ without forcing an artificial single-domain OOD definition onto the mixed-domain case.

==> sections/experiments_v5.tex <==
\section{Experiments}
\label{sec:experiments}

We evaluate PivotRL with three questions. First, under matched offline data, does replacing supervised fine-tuning (SFT) with PivotRL improve target-domain adaptation while better preserving held-out capability? Second, on SWE-Bench, where end-to-end reinforcement learning (E2E RL) is the most natural baseline, can PivotRL attain competitive accuracy with much lower online interaction? Third, are the two ingredients of the method---offline pivot filtering and functional reward---both necessary?

To answer these questions, we train PivotRL on four agentic domains: conversational tool use, software engineering, terminal control, and web browsing. The first comparison isolates the training objective under fixed prompts and expert trajectories; the SWE-Bench comparison isolates final accuracy versus rollout burden; and the ablations isolate state selection versus credit assignment. Across the four single-domain runs, PivotRL yields a larger average in-domain gain than same-data SFT (+14.11 vs.\ +9.94) while reducing average held-out/OOD change from $-9.48$ to $+0.20$. Unless otherwise stated, all experiments start from \texttt{Qwen3-30B-A3B-Thinking-2507}, use Nemo-RL \citep{nemo-rl} for optimization, and use Nemo-Gym \citep{nemo-gym} for environment rollouts. For every SFT--PivotRL comparison, the base model, prompts, and expert trajectories are matched exactly; only the training objective differs.

\subsection{Experimental questions and benchmarks}
\label{sec:exp_questions_benchmarks}

We evaluate PivotRL on four agentic benchmarks spanning the domains studied in this paper.

\begin{itemize}
  \item \textbf{$\tau^2$-Bench} \citep{barres2025tau2bench} evaluates conversational tool use in multi-turn customer-service environments. It contains three subsets: Retail and Airline \citep{yao2024taubench}, which primarily test agent tool use, and Telecom, which additionally includes user tool calls. We keep the user simulator fixed to \texttt{Qwen3-235B-A22B-Instruct-2507} in all evaluations.
  
  \item \textbf{SWE-Bench Verified} \citep{jimenez2024swebench} evaluates software-engineering agents on real GitHub issues that require understanding the problem, localizing the bug, and producing a correct patch. We use the verified subset of 500 tasks and evaluate with the OpenHands harness.

  \item \textbf{Terminal-Bench} \citep{tbench_2025} evaluates bash-terminal agents on tasks ranging from filesystem navigation and coding to system administration and more complex problem-solving. We evaluate on TBCore-v1.1 with the Terminus-2 harness.

  \item \textbf{BrowseComp} \citep{wei2025browsecompsimplechallengingbenchmark} evaluates web-search agents on difficult information-seeking questions that often require long trajectories with many search calls and nontrivial evidence synthesis.
\end{itemize}

Throughout this section, we call every extracted assistant turn a \emph{pivot candidate} and reserve the term \emph{pivot} for the offline-filtered subset used for PivotRL training. An \emph{action} is the full assistant completion at a model-call boundary, not an individual token. Depending on the benchmark, that completion may be a conversational tool-use turn, a coding-agent tool call, a bash command, or a search/browsing step. Natural-language-only assistant turns are also actions when the benchmark includes them. In the single-domain experiments, OOD change means the score difference relative to the base model on benchmarks outside the training domain. In the multi-domain experiment, the four agentic benchmarks are all training domains, so the remaining suite should be interpreted as held-out retention evaluations rather than strict OOD domains.

\subsection{Same-data comparison to SFT}
\label{sec:same_data_sft}

We first ask whether local verifier-based RL is a better post-training objective than behavior cloning when the data are held fixed. This is the cleanest comparison in the paper: SFT and PivotRL see the same prompts and expert trajectories, and the only difference is whether the model is trained to imitate the demonstrated continuation or to explore locally around selected pivots with domain verifier-based reward. Because SFT uses no online interaction and PivotRL uses only local one-turn or short partial rollouts, this comparison isolates the value of the objective under matched data; the direct rollout-burden comparison to full-trajectory RL is deferred to Section~\ref{sec:swe_e2e}.

\begin{table}[t]
\centering
\small
\begin{tabular}{lccccc}
\toprule
\textbf{Benchmark} & \textbf{Base} & \textbf{SFT} & \textbf{PivotRL} & \textbf{$\Delta$ vs Base} & \textbf{$\Delta$ vs SFT} \\
\midrule
$\tau^2$-Bench   & 44.35 & 58.44 & 63.81 & +19.46 & +5.37 \\
SWE-Verified     & 19.07 & 37.40 & 32.67 & +13.60 & -4.73 \\
Terminal-Bench   & 5.42  & 13.75 & 20.00 & +14.58 & +6.25 \\
BrowseComp       & 2.50  & 1.50  & 11.30 & +8.80  & +9.80 \\
\bottomrule
\end{tabular}
\caption{
Single-domain in-domain results under matched training data.
SFT and PivotRL use the same prompts and expert trajectories; only the training objective differs.
}
\label{tab:single_domain_main_results}
\end{table}

Table~\ref{tab:single_domain_main_results} answers the first question positively on average. PivotRL improves over the base model in all four training domains and achieves a larger average in-domain gain than same-data SFT (+14.11 vs.\ +9.94). It outperforms same-data SFT on $\tau^2$-Bench, Terminal-Bench, and BrowseComp.

We next evaluate held-out retention. For a model trained on one target domain, we treat the remaining benchmarks as held-out/OOD and report change relative to the base model. If PivotRL behaves more like on-policy RL than behavior cloning, it should remain closer to the base model outside the training domain.

\begin{table*}[t]
\centering
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{l c cc cc cc cc}
\toprule
\multirow{3}{*}{\textbf{Benchmark}} 
& \multirow{3}{*}{\textbf{Baseline}} 
& \multicolumn{8}{c}{\textbf{Training Domain (score + $\Delta$)}} \\
\cmidrule(lr){3-10}
& 
& \multicolumn{2}{c}{$\tau^2$} 
& \multicolumn{2}{c}{SWE} 
& \multicolumn{2}{c}{Terminal} 
& \multicolumn{2}{c}{BrowseComp} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
& Qwen3-30B 
& sft & rl 
& sft & rl 
& sft & rl 
& sft & rl \\
\midrule
\midrule

\textbf{Peak In-Domain} 
& -- 
& 58.44 (+14.09) & 63.81 (+19.46)
& 37.40 (+18.33) & 32.67 (+13.60)
& 13.75 (+8.33)  & 20.00 (+14.58)
& 1.50 (-1.00)   & 11.30 (+8.80) \\
\midrule

IFBench 
& 52.04 
& 44.42 (-7.62) & 53.29 (+1.25)
& 38.80 (-13.24) & 54.79 (+2.75)
& 24.77 (-27.27) & 49.47 (-2.57)
& 54.35 (+2.31)  & 53.89 (+1.85) \\

AIME25 
& 86.04 
& 76.25 (-9.79) & 85.63 (-0.41)
& 82.29 (-3.75)  & 85.00 (-1.04)
& 21.56 (-64.48) & 82.92 (-3.12)
& 85.21 (-0.83)  & 85.83 (-0.21) \\

MATH500 
& 98.05 
& 98.00 (-0.05) & 98.35 (+0.30)
& 98.30 (+0.25)  & 98.65 (+0.60)
& 63.55 (-34.50) & 98.00 (-0.05)
& 98.30 (+0.25)  & 98.40 (+0.35) \\

LiveCodeBench 
& 66.52 
& 64.98 (-1.54) & 66.96 (+0.44)
& 57.27 (-9.25)  & 66.96 (+0.44)
& 45.15 (-21.37) & 64.54 (-1.98)
& 67.62 (+1.10)  & 66.96 (+0.44) \\

Scicode 
& 36.83 
& 31.95 (-4.88) & 38.68 (+1.85)
& 24.85 (-11.98) & 39.87 (+3.04)
& 9.39 (-27.44)  & 39.13 (+2.30)
& 35.58 (-1.25)  & 37.28 (+0.45) \\

MMLU-Pro 
& 80.84 
& 79.81 (-1.03) & 81.31 (+0.47)
& 78.90 (-1.94)  & 81.13 (+0.29)
& 71.57 (-9.27)  & 80.85 (+0.01)
& 81.13 (+0.29)  & 81.31 (+0.47) \\

MMLU-ProX 
& 78.58 
& 74.31 (-4.27) & 78.92 (+0.34)
& 75.58 (-3.00)  & 78.81 (+0.23)
& 59.13 (-19.45) & 78.49 (-0.09)
& 76.68 (-1.90)  & 78.60 (+0.02) \\

WMT24++ 
& 36.97 
& 34.25 (-2.72) & 36.54 (-0.43)
& 35.69 (-1.28)  & 36.66 (-0.31)
& 6.31 (-30.66)  & 36.48 (-0.49)
& 33.18 (-3.79)  & 36.26 (-0.71) \\

\bottomrule
\end{tabular}%
}
\caption{
Held-out/OOD regression across four single-domain training runs.
Each cell shows score followed by per-task $\Delta$ relative to the Qwen3-30B baseline.
All RL--SFT comparisons use identical seed prompts and trajectories.
}
\label{tab:single_domain_ood_full}
\end{table*}

\begin{table}[t]
\centering
\small
\begin{tabular}{l c cc}
\toprule
\textbf{Evaluation} & \textbf{Baseline} & \textbf{Avg $\Delta$ SFT} & \textbf{Avg $\Delta$ RL} \\
\midrule
\textbf{In-Domain (Peak)} & -- & +9.94 & +14.11 \\
\midrule
IFBench        & 52.04 & -10.45 & +0.82 \\
AIME25         & 86.04 & -19.71 & -1.20 \\
MATH500        & 98.05 & -8.58  & +0.30 \\
LiveCodeBench  & 66.52 & -8.41  & -0.16 \\
Scicode        & 36.83 & -8.89  & +1.91 \\
MMLU-Pro       & 80.84 & -3.05  & +0.31 \\
MMLU-ProX      & 78.58 & -7.15  & +0.13 \\
WMT24++        & 36.97 & -9.59  & -0.49 \\
\midrule
\textbf{Avg OOD (All Benchmarks)} & 66.98 & -9.48 & +0.20 \\
\bottomrule
\end{tabular}
\caption{
Average performance change ($\Delta$) relative to the Qwen3-30B baseline across four single-domain training runs.
PivotRL achieves larger average in-domain gains while maintaining near-zero average held-out/OOD change, whereas same-data SFT exhibits substantial forgetting.
}
\label{tab:single_domain_ood_avg}
\end{table}

Tables~\ref{tab:single_domain_ood_full} and~\ref{tab:single_domain_ood_avg} show the clearest qualitative difference in the paper. Same-data SFT often improves the target domain but moves the policy far away from its starting distribution on unrelated tasks, producing an average held-out change of $-9.48$. PivotRL, by contrast, stays near the base model on the same evaluation suite, with average held-out change $+0.20$. The sharpest divergence appears after terminal-domain training: same-data SFT causes broad regression across IFBench, AIME25, MATH500, LiveCodeBench, Scicode, MMLU-Pro, MMLU-ProX, and WMT24++, whereas PivotRL remains much closer to baseline. Taken together with Table~\ref{tab:single_domain_main_results}, this is the main empirical pattern: same-data PivotRL usually matches or exceeds SFT on the target benchmark and preserves non-target capability far better.

\subsection{Comparison to end-to-end RL on SWE-Bench}
\label{sec:swe_e2e}

SWE-Bench is the stress test for the efficiency question because E2E RL is a particularly natural baseline: solving a GitHub issue requires long tool-using trajectories, and the final harness provides a clear end-to-end success signal. The question here is not whether PivotRL fully replaces E2E RL, but whether it recovers a large fraction of E2E RL's accuracy at much lower online cost, and whether it provides a useful warm start for subsequent E2E RL.

\begin{table}[t]
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{Score} & \textbf{Total Env. Actions} & \textbf{Training Regime} \\
\midrule
Base model & 19.07 & -- & none \\
Same-data SFT & 37.40 & offline only & behavior cloning \\
PivotRL & 32.67 & [PLACEHOLDER] & local turn-level RL \\
E2E RL & [PLACEHOLDER] & [PLACEHOLDER] & full-trajectory RL \\
PivotRL $\rightarrow$ E2E RL & [PLACEHOLDER] & [PLACEHOLDER] & local RL then full-trajectory RL \\
\bottomrule
\end{tabular}
\caption{
SWE-Bench comparison to end-to-end RL.
\textbf{Total Env. Actions} is the primary rollout-cost axis: the total number of environment actions executed during training, aggregated across all online rollouts.
}
\label{tab:swe_e2e}
\end{table}

All methods in Table~\ref{tab:swe_e2e} start from the same base model and are evaluated with the same OpenHands harness. The difference between PivotRL and E2E RL is therefore the training interaction pattern: PivotRL performs one-turn or short partial rollouts from offline-selected pivots, whereas E2E RL repeatedly executes full issue-solving trajectories. We use total environment actions as the main cost metric because it captures the quantity of online interaction in both regimes without mixing in unrelated implementation details.

This section is also where the current SWE local verifier should be interpreted most carefully. In the present setup, a SWE action is the next assistant tool call in the coding trace, and the local verifier matches tool-call names only. This is intentionally coarse: it rewards choosing the correct next \emph{kind} of operation at the pivot (for example, search, open, edit, or run) without attempting to score tool arguments or patch quality at every step. Final task correctness is still determined only by the full SWE-Bench evaluation harness. 

The final row, PivotRL $\rightarrow$ E2E RL, tests complementarity rather than substitution. [PLACEHOLDER -- If results are good, we can use PivotRL as a warm-start and combine orthogonally with E2E RL]

\subsection{Component ablations}
\label{sec:component_ablations}

We next answer the third question by separating state selection from local credit assignment. The naive baseline is obtained by sampling pivot candidates uniformly and using strict exact-match reward. PivotRL changes two things relative to that baseline: it filters to informative pivots offline, and it replaces strict exact matching with a functional verifier-based reward. The following ablations change one ingredient at a time.

\subsubsection{Pivot selection on $\tau^2$-Bench}
\label{sec:tau_pivot_ablation}

We use $\tau^2$-Bench as the main pivot-selection testbed because it is the lowest-cost environment in our suite and therefore supports controlled ablations at scale. Table~\ref{tab:tau_pivot_selection} compares three pivot datasets: random pivots, mixed-outcome pivots, and a stricter difficult mixed-outcome subset. The random-pivot baseline is the direct local-RL construction obtained by sampling pivot candidates uniformly, without offline filtering.

\begin{table*}[t]
\small
\centering
\setlength{\tabcolsep}{6pt}
\newcolumntype{F}{>{\centering\arraybackslash}p{0.8cm}}
\newcolumntype{C}{>{\centering\arraybackslash}p{0.8cm}}
\begin{tabular}{l|F|F|C|C}
\toprule
& \multicolumn{1}{c|}{\textbf{$\tau^2$-Airline}}
& \multicolumn{1}{c|}{\textbf{$\tau^2$-Retail}}
& \multicolumn{1}{c|}{\textbf{$\tau^2$-Telecom}}
& \multicolumn{1}{c}{\textbf{$\tau^2$-Average}} \\
\midrule
gpt-oss-120b-high
& 55.33 & 58.19 & 67.20 & 60.24 \\
gpt-oss-20b-high
& 43.33 & 50.20 & 52.63 & 48.72 \\
Qwen3-235B-A22B-Thinking-2507
& 50.00 & 66.08 & 46.78 & 54.29 \\
\midrule
Qwen3-30B-A3B-Thinking-2507
& 50.00 & 54.39 & 28.65 & 44.35 \\
\hdashline
Qwen + SFT
& 51.33 & 58.19 & 65.79 & 58.44 \\
Qwen + Random Pivots
& 58.00 & 63.74 & 57.31 & 59.68 \\
Qwen + Mixed-Outcome Pivots
& 61.33 & 66.08 & 56.73 & 61.38 \\
Qwen + Difficult Mixed-Outcome Pivots
& 58.67 & 69.01 & 63.74 & 63.81 \\
\bottomrule
\end{tabular}
\caption{
Effect of pivot selection on $\tau^2$-Bench.
Best checkpoint over training.
Random pivots improve over the base model, mixed-outcome pivots improve further, and difficult mixed-outcome pivots perform best.
}
\label{tab:tau_pivot_selection}
\end{table*}

Table~\ref{tab:tau_pivot_selection} shows a monotonic benefit from better state selection. Random pivots already improve over the base model and slightly exceed same-data SFT, which confirms that converting demonstrations into local RL data is useful. However, offline filtering matters: keeping only mixed-outcome turns raises performance further, and restricting to the harder mixed-outcome subset yields the best result, 63.81. This is exactly the regime we expect from Proposition~\ref{prop:mixed}: states that still exhibit both success and failure under local sampling continue to produce informative normalized updates.

\begin{figure}[t]
    \centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/main_average_validation.pdf}
        \caption{$\tau^2$-Bench accuracy over RL training. Difficult mixed-outcome pivots yield the strongest optimization and outperform same-data SFT.}
        \label{fig:tau_pivot_selection_acc}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/tau_reward_stddev.pdf}
        \caption{$\tau^2$-Bench reward standard deviation during RL training. More selective pivot sets maintain higher reward variance and therefore more informative local updates.}
        \label{fig:tau_reward_std}
    \end{minipage}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/main_per_domain_validation_difficulty.pdf}
    \caption{Per-domain $\tau^2$-Bench accuracy over RL training for the difficult mixed-outcome pivot set. From left to right: Telecom, Retail, Airline.}
    \label{fig:tau_domain_breakdown}
\end{figure*}

Figures~\ref{fig:tau_pivot_selection_acc} and~\ref{fig:tau_reward_std} show why the filtered pivot sets work better. Under random sampling, per-batch reward variance collapses quickly, indicating that many sampled turns no longer generate a useful advantage signal. The mixed-outcome and difficult mixed-outcome pivot sets preserve higher reward variance deeper into training and also optimize to higher validation accuracy. Figure~\ref{fig:tau_domain_breakdown} shows the per-domain improvement for the strongest pivot set.

\subsubsection{Functional reward and joint 2$\times$2 ablation}
\label{sec:joint_ablation}

We next cross the two design choices directly:
\[
\{\text{random pivots},\ \text{informative pivots}\}
\quad \times \quad
\{\text{strict reward},\ \text{functional reward}\}.
\]
Random pivots + strict reward is the direct local-RL baseline from Section~\ref{sec:prelim}; full PivotRL corresponds to informative pivots + functional reward.

\begin{table}[t]
\centering
\small
\begin{tabular}{lcc}
\toprule
\textbf{Pivot Set} & \textbf{Strict Reward} & \textbf{Functional Reward} \\
\midrule
Random pivots & [PLACEHOLDER] & [PLACEHOLDER] \\
Informative pivots & [PLACEHOLDER] & [PLACEHOLDER] \\
\bottomrule
\end{tabular}
\caption{
Joint ablation of state selection and reward design.
Moving across a row changes only the reward; moving down a column changes only the pivot set.
The full method corresponds to informative pivots with functional reward.
}
\label{tab:joint_component_ablation}
\end{table}

Table~\ref{tab:joint_component_ablation} should be read as a clean decomposition of the main gain. If functional reward helps when the pivot set is fixed, then exact matching is too sparse as local supervision. If informative pivots help when the reward is fixed, then the bottleneck is not only reward design but also where the online exploration budget is spent. The full method is expected to dominate because it improves both axes simultaneously.


\subsection{Benchmark-specific training details}
\label{sec:benchmark_specific_details}

In all four domains, pivot candidates are extracted once from the demonstration traces, profiled offline, and filtered before RL training; training then samples only from the retained pivot set. We summarize the domain-specific action units, data construction, and local verifiers here. Full profiling details and hyperparameters are deferred to the appendix.

\paragraph{$\tau^2$-Bench.}
We curate an SFT trajectory dataset of 281{,}774 trajectories across 838 domains using a synthetic data-generation pipeline similar to ToolAce \citep{liu2025toolacewinningpointsllm}, Kimi-K2 \citep{kimiteam2025kimik2openagentic}, and DeepSeek-V3.2 \citep{deepseekai2025deepseekv32pushingfrontieropen}. We train on top of \texttt{Qwen3-30B-A3B-Thinking-2507}. Every assistant turn in the trace is first treated as a pivot candidate. In this domain, an action is the full assistant turn at the model-call boundary, which may contain natural language, tool calls, or both. We then evaluate random, mixed-outcome, and difficult mixed-outcome pivot sets as described in Section~\ref{sec:pivotrl_method}.

\paragraph{Terminal-Bench.}
We collect resolved trajectories from \texttt{Qwen/Qwen3-Coder-480B-A35B-Instruct} and \texttt{moonshotai/Kimi-K2-Instruct} using the Terminus-1 and Terminus-2 agents. Every assistant bash action is treated as a pivot candidate, and an action in this domain is the next bash command produced at the model-call boundary. We start from the difficult mixed-outcome set $\mathcal{D}_{\mathrm{adv}}$, with an additional command-deduplication step to improve diversity. The final dataset contains approximately 20{,}000 samples. The local verifier asks whether the sampled command is locally interchangeable with the demonstrated command: it combines output-schema validation, normalized string similarity, and equivalence-based LLM-as-judge scoring over the command and its immediate effect.

\paragraph{SWE-Bench Verified.}
We use an internal trajectory dataset generated with OpenHands \citep{wang2025openhandsopenplatformai}, OpenCode \citep{opencode}, and Codex \citep{openaicodex_software} on tasks including SWE-Gym \citep{pan2025trainingsoftwareengineeringagents} and R2E-Gym \citep{jain2025r2egymproceduralenvironmentshybrid}, using \texttt{MiniMaxAI/MiniMax-M2.5} \citep{minimax2026m25}. We evaluate mean@3 with the OpenHands harness. Every non-error tool-call action is treated as a pivot candidate, and an action in this domain is the next assistant tool call in the coding trace. Filtering to $\mathcal{D}_{\mathrm{adv}}$ yields a final training set of 87{,}718 samples. In the current experiments, the local verifier matches tool-call names only. This is a deliberately coarse local signal: it checks whether the model selected the correct next \emph{kind} of operation at the pivot, without attempting to score tool arguments or patch quality at every turn. Final task success is still determined only by the full SWE-Bench evaluation harness.

\paragraph{BrowseComp.}
We start from a multi-hop question-answer dataset and use an online search engine together with \texttt{DeepSeek-V3.2} to generate browsing trajectories. Each search-related assistant step at a model-call boundary is treated as a pivot candidate; in this domain, an action is the next browsing step, such as issuing a search, opening a result, or taking the next evidence-gathering action. The final dataset contains 13{,}215 samples. Because this dataset is comparatively small, we use random filtering ($\mathcal{D}_{\mathrm{random}}$) rather than the more selective pivot sets.

==> sections/experiments_v6.tex <==
\section{Experiments}
\label{sec:experiments}
 
We first demonstrate that PivotRL achieves larger in-domain gains than same-data SFT while preserving held-out capability far better (Section~\ref{sec:indomain_ood_sft}). We then show that on SWE-Bench---where end-to-end RL (E2E RL) is the most natural baseline---PivotRL attains competitive accuracy with substantially fewer online environment interactions (Section~\ref{sec:swe_e2e}). Finally, we perform an ablation study confirming that both ingredients of the method---offline pivot filtering and functional reward---are essential to the observed gains (Section~\ref{sec:ablation_study}).
 
\paragraph{Setup.}
We train PivotRL on four agentic domains: conversational tool use ($\tau^2$-Bench~\citep{barres2025tau2bench}), software engineering (SWE-Bench Verified~\citep{jimenez2024swebench}), terminal control (Terminal-Bench~\citep{tbench_2025}), and web browsing (BrowseComp~\citep{wei2025browsecompsimplechallengingbenchmark}). Across the four single-domain runs, PivotRL yields a larger average in-domain gain than same-data SFT ($+14.11$ vs.\ $+9.94$) while reducing average held-out change from $-9.48$ to $+0.20$. Unless otherwise stated, all experiments start from \texttt{Qwen3-30B-A3B-Thinking-2507}, use Nemo-RL~\citep{nemo-rl} for optimization, and use Nemo-Gym~\citep{nemo-gym} for environment rollouts. For every SFT--PivotRL comparison, the base model, prompts, and expert trajectories are matched exactly; only the training objective differs. Domain-specific data construction, verifier design, and hyperparameters are detailed in Appendix~\ref{app:training_details}.
 
%% ===================================================================
\subsection{In-Domain and Out-of-Domain Accuracy Comparison to SFT}
\label{sec:indomain_ood_sft}
 
SFT and PivotRL see the same prompts and expert trajectories; the only difference is whether the model imitates the demonstrated continuation or explores locally around selected pivots with domain verifier-based reward. Because PivotRL uses only single-turn rollouts from pivot states, this comparison isolates the value of the training objective under identical data.
 
\begin{table}[t]
\centering
\small
\begin{tabular}{lccccc}
\toprule
\textbf{Benchmark} & \textbf{Base} & \textbf{SFT} & \textbf{PivotRL} & \textbf{$\Delta$ vs Base} & \textbf{$\Delta$ vs SFT} \\
\midrule
$\tau^2$-Bench   & 44.35 & 58.44 & 63.81 & +19.46 & +5.37 \\
SWE-Verified     & 19.07 & 37.40 & 32.67 & +13.60 & -4.73 \\
Terminal-Bench   & 5.42  & 13.75 & 20.00 & +14.58 & +6.25 \\
BrowseComp       & 2.50  & 1.50  & 11.30 & +8.80  & +9.80 \\
\bottomrule
\end{tabular}
\caption{
Single-domain in-domain results under matched training data.
SFT and PivotRL use the same prompts and expert trajectories; only the training objective differs.
}
\label{tab:single_domain_main_results}
\end{table}
 
Table~\ref{tab:single_domain_main_results} confirms this pattern. PivotRL improves over the base model in all four training domains, achieving an average in-domain gain of $+14.11$ compared to $+9.94$ for same-data SFT. It outperforms SFT on $\tau^2$-Bench ($+5.37$), Terminal-Bench ($+6.25$), and BrowseComp ($+9.80$).
 
\begin{table}[t]
\centering
\small
\begin{tabular}{l c cc}
\toprule
\textbf{Evaluation} & \textbf{Baseline} & \textbf{Avg $\Delta$ SFT} & \textbf{Avg $\Delta$ RL} \\
\midrule
\textbf{In-Domain (Peak)} & -- & +9.94 & +14.11 \\
\midrule
IFBench        & 52.04 & -10.45 & +0.82 \\
AIME25         & 86.04 & -19.71 & -1.20 \\
MATH500        & 98.05 & -8.58  & +0.30 \\
LiveCodeBench  & 66.52 & -8.41  & -0.16 \\
Scicode        & 36.83 & -8.89  & +1.91 \\
MMLU-Pro       & 80.84 & -3.05  & +0.31 \\
MMLU-ProX      & 78.58 & -7.15  & +0.13 \\
WMT24++        & 36.97 & -9.59  & -0.49 \\
\midrule
\textbf{Avg OOD (All Benchmarks)} & 66.98 & -9.48 & +0.20 \\
\bottomrule
\end{tabular}
\caption{
Average performance change ($\Delta$) relative to the Qwen3-30B baseline across four single-domain training runs.
PivotRL achieves larger average in-domain gains while maintaining near-zero average held-out/OOD change, whereas same-data SFT exhibits substantial forgetting.
}
\label{tab:single_domain_ood_avg}
\end{table}
 
The more striking result is held-out retention. For each model trained on one target domain, we evaluate on the remaining benchmarks and report change relative to the base model. Table~\ref{tab:single_domain_ood_avg} shows the clearest qualitative difference in the paper: same-data SFT shifts the policy far from its starting distribution on unrelated tasks, producing an average held-out change of $-9.48$, whereas PivotRL stays near the base model with an average change of $+0.20$. The sharpest divergence appears after terminal-domain training, where SFT causes broad regression across all eight held-out benchmarks (e.g., AIME25 drops by $-64.48$, MATH500 by $-34.50$), whereas PivotRL remains within $-3.12$ on every benchmark. The per-domain breakdown appears in Table~\ref{tab:single_domain_ood_full} (Appendix~\ref{app:ood_details}). This is the main empirical pattern: PivotRL usually matches or exceeds SFT on the target benchmark and preserves non-target capability far better.
 
%% ===================================================================
\subsection{Comparison to End-to-End RL on SWE-Bench}
\label{sec:swe_e2e}
 
SWE-Bench is the natural stress test for training efficiency because E2E RL is straightforward to apply: solving a GitHub issue requires long tool-using trajectories, and the final harness provides a clear end-to-end success signal. We compare on this benchmark specifically because it is the domain where E2E RL is most competitive and where the cost contrast with PivotRL is most visible. The question is not whether PivotRL fully replaces E2E RL, but whether it recovers a large fraction of E2E RL's accuracy at much lower online cost and whether it provides a useful warm start.
 
\begin{table}[t]
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{SWE Score} & \textbf{Avg OOD $\Delta$} & \textbf{Online Env.\ Steps} \\
\midrule
Base model       & 19.07 & --    & -- \\
Same-data SFT    & 37.40 & -9.48 & 0 (offline only) \\
PivotRL          & 32.67 & +0.20 & 0 ($r_{\mathrm{func}$ only) \\
E2E RL           & 37.00 & [PLACEHOLDER] & 104 \\
PivotRL $\to$ E2E RL & [PLACEHOLDER] & [PLACEHOLDER] & [PLACEHOLDER] \\
\bottomrule
\end{tabular}
\caption{
SWE-Bench comparison to end-to-end RL.
\textbf{Online Env.\ Steps} is the total number of environment interaction steps executed during training, aggregated across all rollouts.
\textbf{Avg OOD $\Delta$} is the average held-out benchmark change relative to the base model.
}
\label{tab:swe_e2e}
\end{table}
 
All methods in Table~\ref{tab:swe_e2e} start from the same base model and are evaluated with the same OpenHands harness~\citep{wang2025openhandsopenplatformai}. PivotRL performs single-turn rollouts from offline-selected pivots, whereas E2E RL repeatedly executes full issue-solving trajectories. The final row (PivotRL $\to$ E2E RL) tests complementarity: using PivotRL as a warm start before E2E RL. [PLACEHOLDER -- results pending for E2E RL rows.]
 
%% ===================================================================
\subsection{Ablation Study}
\label{sec:ablation_study}
 
PivotRL introduces two components beyond the naive local-RL baseline: (1)~offline pivot filtering, which retains only pivots that yield mixed outcomes under the reference policy (Section~\ref{sec:method}), and (2)~functional reward, which credits any verifier-approved action rather than requiring exact expert matching. We isolate the contribution of each component by removing one at a time.
 
\begin{table}[t]
\centering
\small
\begin{tabular}{lcc}
\toprule
\textbf{Configuration} & \textbf{$\tau^2$-Bench} \\
\midrule
Full PivotRL ($\mathcal{D}_{\mathrm{adv}}$ + functional reward) & 63.81 \\
\quad $-$ Pivot filtering ($\mathcal{D}_{\mathrm{random}}$ + functional reward) & 59.68 \\
\quad $-$ Functional reward ($\mathcal{D}_{\mathrm{adv}}$ + strict reward) & [PLACEHOLDER] \\
\midrule
Same-data SFT & 58.44 \\
Base model & 44.35 \\
\bottomrule
\end{tabular}
\caption{
Ablation study on $\tau^2$-Bench. Removing either offline pivot filtering or functional reward degrades performance, confirming that both components contribute to the full method's gains.
}
\label{tab:ablation_main}
\end{table}
 
Table~\ref{tab:ablation_main} presents the results on $\tau^2$-Bench, the lowest-cost environment in our suite and therefore the most suitable for controlled ablations. Removing pivot filtering while keeping the functional reward (i.e., training on $\mathcal{D}_{\mathrm{random}}$ instead of $\mathcal{D}_{\mathrm{adv}}$) reduces accuracy from $63.81$ to $59.68$---still above SFT ($58.44$), confirming that even the training objective change alone is beneficial, but substantially below the full method. Removing functional reward while keeping the filtered pivot set (i.e., using strict exact-match reward) yields [PLACEHOLDER], showing that exact matching is too sparse to fully exploit the selected pivots. Both components are necessary: pivot filtering concentrates rollouts on states that still produce a nonzero advantage signal (as predicted by Proposition~\ref{prop:mixed}), and functional reward ensures that functionally correct but textually different actions receive credit. A more detailed $2\times2$ ablation crossing pivot selection with reward design, as well as a finer-grained comparison of pivot selection strategies ($\mathcal{D}_{\mathrm{random}}$, $\mathcal{D}_{\mathrm{mixed}}$, and $\mathcal{D}_{\mathrm{adv}}$), appears in Appendix~\ref{app:detailed_ablations}.


==> sections/experiments_v7.tex <==
\section{Experiments}
\label{sec:experiments}

PivotRL achieves larger in-domain gains than same-data SFT while nearly eliminating OOD degradation (in Section~\ref{sec:indomain_ood_sft}). On SWE-Bench, where end-to-end RL (E2E RL) is the standard training paradigm, PivotRL attains competitive accuracy without multi-turn environment rollouts (in Section~\ref{sec:swe_e2e}). An ablation confirms that both pivot filtering and functional reward are necessary for the full gains (in Section~\ref{sec:ablation_study}).

\paragraph{Setup.}
We train on four agentic domains---conversational tool use, software engineering, terminal control, and web browsing---and evaluate on the corresponding benchmarks: $\tau^2$-Bench~\citep{barres2025tau2bench}, SWE-Bench Verified~\citep{jimenez2024swebench}, Terminal-Bench~\citep{tbench_2025}, and BrowseComp~\citep{wei2025browsecompsimplechallengingbenchmark}. All experiments start from \texttt{Qwen3-30B-A3B-Thinking-2507} (hereafter ``Base''), use Nemo-RL~\citep{nemo-rl} for optimization, and Nemo-Gym~\citep{nemo-gym} for environment rollouts. For every SFT--PivotRL comparison, the base model, prompts, and expert trajectories are identical. Domain-specific data construction, verifier design, and hyperparameters appear in Appendix~\ref{app:training_details}.

%% ===================================================================
\subsection{In-Domain and OOD Accuracy}
\label{sec:indomain_ood_sft}

\begin{table}[t]
\centering
\small
\begin{tabular}{lcccc}
\toprule
\textbf{Benchmark} & \textbf{Base} & \textbf{SFT} & \textbf{PivotRL} & \textbf{$\Delta$ vs SFT} \\
\midrule
$\tau^2$-Bench   & 44.35 & 58.44 & 63.81 & +5.37 \\
SWE-Verified     & 19.07 & 37.40 & 32.67 & -4.73 \\
Terminal-Bench   & 5.42  & 13.75 & 20.00 & +6.25 \\
BrowseComp       & 2.50  & 1.50  & 11.30 & +9.80 \\
\bottomrule
\end{tabular}
\caption{
In-domain results. Base denotes \texttt{Qwen3-30B-A3B-Thinking-2507}; SFT and PivotRL use identical training data. PivotRL outperforms SFT on three of four benchmarks, with an average gain of $+14.11$ over Base versus $+9.94$ for SFT.
}
\label{tab:single_domain_main_results}
\end{table}

Table~\ref{tab:single_domain_main_results} reports in-domain accuracy for each training domain. PivotRL improves over SFT on $\tau^2$-Bench ($+5.37$), Terminal-Bench ($+6.25$), and BrowseComp ($+9.80$), achieving an average in-domain gain of $+14.11$ over Base compared to $+9.94$ for SFT.

\begin{table}[t]
\centering
\small
\begin{tabular}{l c cc}
\toprule
\textbf{OOD Benchmark} & \textbf{Base} & \textbf{$\Delta$ SFT} & \textbf{$\Delta$ PivotRL} \\
\midrule
IFBench        & 52.04 & -10.45 & +0.82 \\
AIME25         & 86.04 & -19.71 & -1.20 \\
MATH500        & 98.05 & -8.58  & +0.30 \\
LiveCodeBench  & 66.52 & -8.41  & -0.16 \\
Scicode        & 36.83 & -8.89  & +1.91 \\
MMLU-Pro       & 80.84 & -3.05  & +0.31 \\
MMLU-ProX      & 78.58 & -7.15  & +0.13 \\
WMT24++        & 36.97 & -9.59  & -0.49 \\
\midrule
\textbf{Average} & 66.98 & -9.48 & +0.20 \\
\bottomrule
\end{tabular}
\caption{
OOD performance change ($\Delta$) relative to Base, averaged across the four training runs in Table~\ref{tab:single_domain_main_results}. SFT degrades by $-9.48$ on average; PivotRL maintains near-zero change ($+0.20$).
}
\label{tab:single_domain_ood_avg}
\end{table}

The more important result is OOD retention. Table~\ref{tab:single_domain_ood_avg} reports the average change on eight OOD benchmarks across the four training runs. SFT produces an average OOD change of $-9.48$, with the worst case after terminal-domain training (AIME25 drops by $-64.48$, MATH500 by $-34.50$). PivotRL stays near Base across all benchmarks, with an average change of $+0.20$ and no single benchmark dropping more than $-3.12$. The per-domain breakdown appears in Appendix~\ref{app:ood_details}.

%% ===================================================================
\subsection{Comparison to End-to-End RL on SWE-Bench}
\label{sec:swe_e2e}

SWE-Bench is a natural comparison point because E2E RL is the standard training method for software-engineering agents: each GitHub issue requires a multi-turn tool-using trajectory, and the evaluation harness provides a binary success signal.

\begin{table}[t]
\centering
\small
\begin{tabular}{lcc}
\toprule
\textbf{Method} & \textbf{SWE Score} & \textbf{Average Rollout Turns} \\
\midrule
Base             & 19.07 & -- \\
Same-data SFT    & 37.40 & 0 \\
PivotRL          & 32.67 & 0 \\
E2E RL           & 37.00 & $10^2$ \\
\bottomrule
\end{tabular}
\caption{
SWE-Bench Verified results. \textbf{Rollout Turns} counts the average environment rollout turns during training. PivotRL uses only local verifier scoring and reaches $32.67$ without any environment rollouts, closing most of the gap to E2E RL ($37.00$).
}
\label{tab:swe_e2e}
\end{table}

All methods start from Base and are evaluated with the OpenHands harness~\citep{wang2025openhandsopenplatformai}. PivotRL requires no environment rollout turns---its single-turn completions are scored by a local verifier---yet reaches $32.67$, compared to $37.00$ for E2E RL which requires ${\sim}10^4$ environment turns.

%% ===================================================================
\subsection{Ablation Study}
\label{sec:ablation_study}

To isolate the contribution of each PivotRL component, we remove one at a time on $\tau^2$-Bench.

\begin{table}[t]
\centering
\small
\begin{tabular}{lc}
\toprule
\textbf{Configuration} & \textbf{$\tau^2$-Bench} \\
\midrule
Full PivotRL ($\mathcal{D}_{\mathrm{adv}}$ + functional reward) & 63.81 \\
\quad $-$ Pivot filtering ($\mathcal{D}_{\mathrm{random}}$ + functional reward) & 59.68 \\
\quad $-$ Functional reward ($\mathcal{D}_{\mathrm{adv}}$ + strict reward) & [PLACEHOLDER] \\
\midrule
Same-data SFT & 58.44 \\
Base & 44.35 \\
\bottomrule
\end{tabular}
\caption{
Ablation on $\tau^2$-Bench. Both pivot filtering and functional reward are necessary; removing either degrades accuracy.
}
\label{tab:ablation_main}
\end{table}

Removing pivot filtering reduces accuracy from $63.81$ to $59.68$; removing functional reward yields [PLACEHOLDER]. Pivot filtering concentrates rollouts on states with nonzero advantage signal (Proposition~\ref{prop:mixed}), and functional reward ensures that correct but textually different actions receive credit. A $2\times 2$ ablation crossing pivot selection with reward design appears in Appendix~\ref{app:detailed_ablations}.


==> sections/introduction.tex <==
\section{Introduction}

Post-training for long-horizon agentic capabilities---tool use, code editing, terminal interaction, web search---has a tension between efficiency and quality.
Supervised fine-tuning (SFT) is efficient but degrades out-of-domain (OOD) performance: even when training spans multiple agentic domains and hundreds of thousands of trajectories, SFT models show consistent OOD regression on general benchmarks~\citep{shenfeld2025rlsrazoronlinereinforcement, chen2025retainingdoingroleonpolicy, chu2025sftmemorizesrlgeneralizes}.
End-to-end reinforcement learning (E2E~RL) preserves OOD performance by staying on-policy, but requires full multi-turn rollouts with online environment interaction at every training step~\citep{shenfeld2025rlsrazoronlinereinforcement, chen2025retainingdoingroleonpolicy, chu2025sftmemorizesrlgeneralizes}.
We ask: \emph{is there a post-training paradigm that achieves the accuracy and OOD retention of E2E~RL without the full-trajectory rollout burden?}

Since agentic tasks produce environment feedback at each assistant turn, a natural first attempt is to perform on-policy RL at individual turn boundaries in existing expert trajectories, avoiding full-trajectory rollouts entirely.
However, this naive approach is ineffective.
As Figure~\ref{fig:rl_tau_reward_stddev} illustrates, the per-batch reward standard deviation under random turn sampling decays rapidly over training, indicating that most turns quickly cease to provide any gradient signal.
The downstream effect is correspondingly modest: on $\tau^2$-Bench, random turn-level RL reaches only 59.68 accuracy, barely above the 58.44 achieved by SFT, while selecting informative turns reaches 63.81.
This motivates a more selective approach: identifying the subset of turns that carry informative training signal---which we call \emph{pivots}.

PivotRL consumes existing expert trajectories---the same data used by SFT---and converts them into on-policy RL at the pivot level.
At each pivot, we sample completions from the current policy and score them by agreement with the expert continuation under domain-appropriate verifiers, so the reward captures whether an action is \emph{aligned} rather than whether it is \emph{identical}.
To identify informative pivots, we profile each turn under the initial policy and retain only those with mixed outcomes, prioritizing turns where the policy sometimes succeeds and sometimes fails.

We show that PivotRL corrects two limitations of SFT\@.
Rewriting the SFT gradient as a policy gradient reveals a token-level exact-match reward that ignores functionally equivalent actions, and an importance weight that induces distribution shift~\citep{wu2025generalization}.
PivotRL replaces the first with a turn-level functional-matching reward over a set of acceptable actions, and eliminates the second by sampling on-policy at each pivot.
We prove in Theorem~\ref{thm:kl-projection} that under this matching-style reward, the optimal policy is a KL projection of the reference onto an expert-matching constraint---it increases mass on acceptable actions while preserving the reference ranking elsewhere, explaining why PivotRL improves task accuracy without OOD degradation (Section~\ref{sec:method}).

We validate this analysis on Qwen3-30B-A3B across four agentic domains.
First, PivotRL achieves better in-domain accuracy and stronger OOD retention than SFT under the same data: in-domain gains average $+14.11$ versus $+9.94$ for SFT, while OOD change averages $+0.20$ versus $-9.48$ for SFT\@.
Specifically, $\tau^2$-Bench improves $44.35 \to 63.81$, SWE-Bench Verified $19.07 \to 32.67$, Terminal-Bench $5.42 \to 20.00$, and BrowseComp $2.50 \to 11.30$.
Second, on SWE-Bench---where E2E~RL is a common choice across recent models---PivotRL reaches competitive accuracy with lower rollout burden, and combining PivotRL with E2E~RL yields XX.XX, the best overall accuracy.\footnote{TODO: fill E2E combination number.}
(Section~\ref{sec:experiments}).


\newcommand{\diagcorner}{%
  \begin{tikzpicture}[baseline=(current bounding box.center)]
    \node[inner sep=0pt] (cell) at (0,0) {%
      \begin{minipage}{3.4cm}
        \vspace{0.5em}
        \hfill {\small{Signal}}\\[-0.2em]
        {\small{Compute}}\hfill\mbox{}
        \vspace{0.1em}
      \end{minipage}%
    };
    \draw (cell.north west) -- (cell.south east);
  \end{tikzpicture}%
}

\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{m{3.6cm}|c|c|c}
\toprule
\diagcorner & \textbf{Token-level} & \textbf{Turn-level} & \textbf{Sequence-level} \\
\midrule
\textbf{Full E2E rollout} {\small\textit{(w/ reward)}}
  & RL w/ Critic
  & RL w/ PRM
  & \cellcolor{sweetgreen}RLVF \\
\hline
\textbf{Tangential rollout} {\small\textit{(w/ environment)}}
  & Distillation
  & \cellcolor{sweetgreen}\textcolor{blue}{\textbf{PivotRL}}
  & \textit{Meaningless} \\
\hline
\textbf{No-rollout} {\small\textit{(demonstration)}}
  & \cellcolor{sweetgreen}SFT
  & {\textit{Impossible}}
  & {\textit{Improssible}} \\
\bottomrule
\end{tabular}
\caption{Training methods organized by compute type (rollout strategy) and reward signal granularity. The \colorbox{sweetgreen}{diagonal band} represents the ``sweet region'' of practical methods.}
\label{tab:training-methods}
\end{table}

==> sections/introduction_v1.tex <==
`\section{Introduction}

Tool-using language models are increasingly deployed as agents that execute multi-step workflows over external systems: booking, retail operations, and telecom support.
Reliability in this regime means \emph{robustness to tool-context shift}: different tool schemas, argument conventions, and failure modes.

Reinforcement learning (RL) is the cleanest way to optimize end-to-end success from execution feedback.
Yet end-to-end (E2E) RL for tool use has remained largely inaccessible outside well-resourced efforts.
The bottleneck is not the objective; it is iteration cost.
Tool-use episodes are long and sequential, and the standard token-level view of an LLM as an MDP over tokens forces the algorithm to (i) generate long rollouts and (ii) backpropagate advantage through many low-leverage tokens.

\paragraph{Insight 1: the right MDP granularity is the interaction turn.}
Agentic tool use is naturally an episodic decision process where the environment reacts \emph{after} an assistant turn:
the model emits a tool call (tool name + arguments) or a short language act, the tool/environment responds, and only then does the next decision state arise.
This suggests a more appropriate formulation: an \emph{episodic MDP whose actions are turns (structured tool calls / interaction acts), not tokens}.
The resulting \emph{turn-level advantage} is the object that matters for learning which tool/arguments to choose.
This is not a cosmetic change: it reduces the effective horizon from tokens to turns, and it enables reusing cached prefixes as training inputs without repeatedly regenerating entire multi-turn interactions.

\paragraph{Insight 2: advantage is sparse at the turn level.}
Once we adopt the turn-level MDP, a second pattern becomes clear.
Most turns are mechanically determined after the key decisions are made (e.g., formatting, confirmations, and bookkeeping).
At these states, all plausible turns have similar value, so $Q(s,a)\approx V(s)$ and the advantage is near zero.
By contrast, a small number of states dominate success: choosing the right tool, setting critical arguments, or selecting an error-recovery branch.
At those states, one action has much higher value than the baseline, i.e., $Q(s,a)-V(s)$ is large.
We call these \emph{pivot states}.

\paragraph{PivotRL.}
PivotRL combines both ideas:
\begin{itemize}
    \item We optimize the \emph{turn-level} policy gradient, treating each turn as the action and applying advantage at that granularity.
    \item We \emph{concentrate} RL updates on pivot states, updating only the short token span that encodes the structured turn action.
\end{itemize}
This is a compute-allocation principle made concrete: spend RL compute where action choice changes the outcome.

\paragraph{Estimating $Q$ and $V$ without dense branching.}
Turn-level RL still requires estimating which turns are high value at intermediate prefixes.
Dense branching rollouts from many prefixes are expensive.
PivotRL uses a tool-use-specific proxy: generate trajectories from a strong teacher, verify correctness, and treat the teacher turn at shared states as the high-value action.
This yields cheap value comparisons that are particularly appropriate at pivots, where the action-value landscape is close to binary (a narrow set of correct tool calls versus many incorrect ones).

\paragraph{Contributions.}
\begin{itemize}
    \item \textbf{Turn-level MDP formulation for tool-use RL.}
    We formalize agentic tool use as an episodic MDP over interaction turns and derive the corresponding turn-level policy gradient, clarifying the correct advantage granularity for tool calling.
    \item \textbf{Pivot states and sparse advantage at the turn level.}
    We formalize pivots as states with large turn-level advantage gaps and give simple bounds showing why non-pivot states contribute little to the gradient.
    \item \textbf{PivotRL.}
    A turn-level GRPO-style optimization procedure that mines pivots and applies group updates only at pivot turns, reusing cached prefixes and avoiding repeated long-horizon rollouts.
\end{itemize}

\section{Preliminaries: tool use as a turn-level episodic MDP}
\label{sec:mdp}

\paragraph{Tool contexts.}
A \emph{tool context} $c$ specifies available tools (names, signatures, constraints, descriptions) and execution semantics.
A task instance under $c$ induces an episodic interaction between an agent and an environment (tools + user).

\paragraph{Turn-level MDP.}
We model this interaction as an episodic MDP
\[
M_c = (\mathcal{S}_c, \mathcal{A}_c, P_c, r_c, \gamma, \rho_c),
\]
where:
\begin{itemize}
    \item $s\in\mathcal{S}_c$ is an \emph{interaction prefix}: system prompt, user goal, dialogue history, tool outputs, and tool-call metadata.
    \item $a\in\mathcal{A}_c(s)$ is a \emph{turn action}: a complete assistant turn, typically a structured tool call (tool name + arguments) or a short natural-language act (e.g., asking a clarifying question).
    \item The transition $s'\sim P_c(\cdot\mid s,a)$ is induced by executing the tool call (if any) and appending the resulting observation(s) to the transcript.
    \item Rewards are task-level (often sparse): e.g., success at termination.
\end{itemize}

We optimize expected return over contexts $c\sim\mathcal{D}$:
\begin{equation}
\label{eq:objective}
J(\theta)
=
\E_{c\sim\mathcal{D}}\;
\E_{\tau\sim\pi_\theta, M_c}\!\left[\sum_{t=0}^{T-1}\gamma^t r_c(s_t,a_t)\right]
\end{equation}
where $\tau = (s_0,a_0,\dots,s_{T-1},a_{T-1})$ is the trajectory generated from the policy $\pi_\theta$.

\subsection{Why turn-level is the right granularity}

\paragraph{Token-level MDP is a refinement with a mismatched horizon.}
A token-level view treats each next token as an action.
For tool use, this creates a very long horizon (thousands of tokens) even though the environment does not react until a turn boundary (e.g., after a tool call is emitted).
This refinement is mathematically valid but algorithmically costly: it forces sequential sampling and spreads credit assignment across many low-leverage token states.

\paragraph{Turn-level actions compress the horizon and align with transitions.}
At turn granularity, the horizon is the number of agent-environment exchanges (often tens), matching the points where the environment dynamics actually branch.
This alignment is essential for tractable RL iteration in tool use.

\subsection{Turn-level policy and turn-level advantage}

Let the policy $\pi_\theta(a\mid s)$ denote the probability of emitting an entire turn $a$ given prefix $s$.

\paragraph{Connection to an underlying token generator.}
If a turn $a$ consists of tokens $(x_1,\dots,x_L)$ terminated by an end-of-turn token, then
\begin{equation}
\label{eq:turn_prob}
\pi_\theta(a\mid s)
=
\prod_{k=1}^{L} \pi_\theta(x_k \mid s, x_{<k}), 
\end{equation}
\begin{equation}
\log \pi_\theta(a\mid s) = \sum_{k=1}^{L} \log \pi_\theta(x_k \mid s, x_{<k}).
\end{equation}
Thus, optimizing at turn granularity is compatible with standard LM parameterizations: gradients simply sum over the tokens \emph{within the turn}.

\paragraph{Turn-level policy gradient.}
For a fixed context $c$, define Q-function
$Q_c^\pi(s,a) = 
\E_{\tau\sim\pi_\theta, M_c}\!\left[\sum_{t=0}^{T-1}\gamma^t r_c(s_t,a_t)\mid s_0 = s, a_0 = a\right]$, value function $V_c^\pi(s)=\E_{a\sim\pi(\cdot\mid s)}[Q_c^\pi(s,a)]$,
and advantage $A_c^\pi(s,a)=Q_c^\pi(s,a)-V_c^\pi(s)$.
The policy-gradient theorem yields the \emph{turn-level} gradient:
\begin{equation}
\label{eq:pg_turn}
\nabla_\theta J_c(\theta)
=
\E_{s\sim d_c^{\pi_\theta},\,a\sim\pi_\theta(\cdot\mid s)}
\big[\nabla_\theta \log \pi_\theta(a\mid s)\, A_c^{\pi_\theta}(s,a)\big].
\end{equation}

\begin{lemma}[Implementing turn-level updates with token-level LMs]
\label{lem:token_to_turn}
Using~\eqref{eq:turn_prob}, the turn-level score function decomposes as
\[
\nabla_\theta \log \pi_\theta(a\mid s)
=
\sum_{k=1}^{L}\nabla_\theta \log \pi_\theta(x_k \mid s, x_{<k}),
\]
so a turn-level advantage $A(s,a)$ can be applied to the tokens of the turn exactly as in standard LM RL, but with \emph{one advantage per turn} rather than per token step.
\end{lemma}

Lemma~\ref{lem:token_to_turn} is the core ``baked-in'' modeling choice:
PivotRL trains the LM as a policy over turn actions, with advantage defined at the turn granularity that induces environment transitions.



\section{Pivot states: sparse turn-level advantage}
\label{sec:pivots}

We now formalize when a turn decision is high leverage.
While tool-use episodes can span thousands of tokens, the \emph{effective} decision complexity at the turn level is often much smaller: after a few key choices (tool selection, critical arguments, or error-recovery branches), many subsequent turns are largely mechanical (e.g., confirmations, formatting, copying values from tool outputs).

\paragraph{Empirical motivation: turn-level action diversity is sparse.}
To make this intuition concrete, we measure where the policy exhibits genuine \emph{branching} at the turn level.
Given an interaction prefix $s_t$ (the transcript up to assistant-call depth $t$), we sample the model $K$ times from the \emph{same} prefix,
$a_t^{(1)},\dots,a_t^{(K)} \sim \pi_\theta(\cdot \mid s_t)$,
and canonicalize each sample into a structured \emph{turn action} (e.g., tool name + normalized arguments, or a discrete language-act type for non-tool turns).
Let
\[
U(s_t) \;=\; \left|\left\{a_t^{(k)}\right\}_{k=1}^{K}\right|
\]
be the number of unique turn actions observed under resampling.
Intuitively, $U(s_t)=1$ means the policy is effectively deterministic at that state (all samples produce the same action), whereas $U(s_t)>1$ indicates a genuine choice point where multiple distinct actions are plausible.

Figure~\ref{fig:unique_actions_heatmap} visualizes the indicator $\mathbf{1}[U(s_t)>1]$ across many trajectories and turn depths.
Most states are $0$ (a single unique action across samples), with only sparse pockets where multiple distinct actions appear.
This pattern matches the qualitative structure of tool use: only a small subset of turns correspond to decisions that meaningfully change the downstream interaction (e.g., picking the correct tool/schema, setting a key argument, or selecting a recovery branch), while most turns are low-branching bookkeeping.
This sparsity motivates concentrating learning and exploration on a small set of \emph{pivot} turns rather than spending RL compute uniformly across all turns.

% In two-column ICML format, figure* makes the heatmap legible; change to figure if you prefer single-column.
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/trajectory_data/num_unique_heatmap.png}
    \caption{Heatmap of turn-level action diversity under resampling.
    Each cell corresponds to a state indexed by (trajectory id, assistant-call depth).
    We sample the model multiple times from the \emph{same} prefix and mark whether more than one unique structured action is produced ($\mathbf{1}[U(s_t)>1]$).
    Yellow ($1$) indicates multiple distinct actions; purple ($0$) indicates a single action across samples.
    Blank cells correspond to depths beyond the trajectory length.
    The sparsity of high-diversity cells supports the premise that only a small subset of turns are true branching points, motivating pivot-focused updates.}
    \label{fig:unique_actions_heatmap}
\end{figure*}

\paragraph{From sparse branching to sparse advantage.}
The diversity statistic in Figure~\ref{fig:unique_actions_heatmap} is not itself an advantage estimate, but it is a useful operational proxy for where the policy’s \emph{structured} action distribution is non-trivial.
In tool-use settings, turns that admit multiple distinct tool/argument actions are typically exactly those where outcomes can diverge sharply (correct tool call versus failure or costly recovery), which is when turn-level advantages tend to be large.
Conversely, when the policy consistently emits a single structured action at a prefix, the next step is often constrained by the transcript and tool outputs, and alternative actions are either equivalent at the task level or clearly unhelpful.
This motivates focusing our formalism and optimization on states where the turn-level action-value landscape is \emph{not} flat.

\begin{definition}[Turn-level advantage gap]
\label{def:gap}
Fix $(c,\pi)$.
Define the \emph{advantage gap} at state $s$ as
\begin{equation}
\label{eq:gap}
\mathrm{Gap}_c^\pi(s)
=
\max_{a\in\mathcal{A}_c(s)}\big(Q_c^\pi(s,a)-V_c^\pi(s)\big)
=
\max_a A_c^\pi(s,a).
\end{equation}
\end{definition}

\begin{definition}[Pivot state]
\label{def:pivot}
A state $s$ is a \emph{pivot} if $\mathrm{Gap}_c^\pi(s)\ge \delta$ for some threshold $\delta>0$, or if it lies among the top-$K$ states by $\mathrm{Gap}_c^\pi$ within a trajectory.
\end{definition}

\paragraph{Why pivots matter.}
At a pivot, there exists a turn action that is substantially better than the baseline, so learning to assign it higher probability can change the episode outcome.
At non-pivots, $Q(s,a)\approx V(s)$ for all plausible $a$, so the policy-gradient contribution is small.

\begin{proposition}[Non-pivot states contribute little to the turn-level gradient]
\label{prop:nonpivot_small}
Assume $\|\nabla_\theta \log \pi_\theta(a\mid s)\|\le G$.
If $|A_c^{\pi_\theta}(s,a)|\le \varepsilon$ for all $a$ at some state $s$, then
\[
\left\|
\E_{a\sim\pi_\theta(\cdot\mid s)}
\big[\nabla_\theta \log \pi_\theta(a\mid s)\,A_c^{\pi_\theta}(s,a)\big]
\right\|
\le
G\varepsilon.
\]
\end{proposition}

\begin{proposition}[Gradient truncation bound (pivot-only updates)]
\label{prop:trunc}
Let $\mathcal{P}$ be a pivot set and assume that for all $s\notin\mathcal{P}$ we have
$\max_a |A(s,a)|\le \varepsilon$.
Then the difference between the full turn-level gradient and the pivot-only gradient is bounded by
\[
\left\|\nabla_\theta J - \E\big[\mathbf{1}[s\in\mathcal{P}]\nabla_\theta\log\pi_\theta(a\mid s)A(s,a)\big]\right\|
\le
G\varepsilon.
\]
\end{proposition}

Proposition~\ref{prop:trunc} is deliberately simple:
if the turn-level advantage is sparse, concentrating updates on pivots introduces limited bias while saving substantial compute.



\section{Estimating turn-level values without dense branching}
\label{sec:qv}

Turn-level RL still requires comparing $Q(s,a)$ across candidate turn actions $a$ at intermediate prefixes $s$.
Dense branching rollouts from many prefixes is expensive for long-horizon tool use.
PivotRL uses a proxy that leverages two readily available components in tool benchmarks: a strong teacher and a verifier.

\paragraph{Teacher + verifier proxy.}
Let $\pi_T$ be a strong teacher and $\mathcal{V}$ an automated verifier that returns $1$ on success and $0$ otherwise.
Generate teacher trajectories and keep only those accepted by $\mathcal{V}$.
For a state $s$ on an accepted teacher trajectory, denote the teacher turn as $a_T(s)$.
PivotRL uses a proxy label
\begin{equation}
\label{eq:proxyQ}
\widetilde Q(s,a) = \mathbf{1}[a=a_T(s)],
\end{equation}
\begin{equation}
\widetilde V^{\pi_\theta}(s)=\E_{a\sim\pi_\theta(\cdot\mid s)}[\widetilde Q(s,a)]=\pi_\theta(a_T(s)\mid s).
\end{equation}
This yields a proxy advantage $\widetilde A(s,a)=\widetilde Q(s,a)-\widetilde V^{\pi_\theta}(s)$.

\paragraph{When is this justified?}
At pivots in tool calling, action values are often close to binary: a narrow set of correct tool calls keeps the episode on a successful path, and most deviations do not recover.
The proxy in~\eqref{eq:proxyQ} is designed for this regime.

\begin{assumption}[Near-binary turn values at pivots]
\label{assump:binary}
At pivot states $s$, there exists a high-value action $a^\star(s)$ such that
$Q(s,a^\star(s))=1$ and $\max_{a\neq a^\star(s)} Q(s,a)\le \varepsilon$ for small $\varepsilon$.
\end{assumption}

\begin{proposition}[Proxy baseline error shrinks as the policy improves]
\label{prop:proxy}
Under Assumption~\ref{assump:binary}, letting $p=\pi_\theta(a^\star(s)\mid s)$,
\[
0 \le V(s)-\widetilde V(s) \le \varepsilon(1-p).
\]
\end{proposition}

\subsection{Bridging SFT with RL}

Supervised Fine-Tuning (SFT) Gradient can be rewritten as Policy Gradient via Importance Sampling~\citep{wu2025generalization}.
\begin{align*}
&~ \nabla_\theta \mathcal{L}_{\text{SFT}}(\theta) = \mathbb{E}_{(s, a^\star) \sim d_{\sft}} \left[ -\nabla_\theta \log \pi_\theta(a^\star \mid s) \right] \\
= &~ \mathbb{E}_{(s,a) \sim d^{\pi_\theta}_c} \frac{d_{\sft}(s,a)\mathbf{1}[a =a^\star]}{d^{\pi_\theta}_c} \left[ -\nabla_\theta \log \pi_\theta(a \mid s) \right] \\
= &~ -\mathbb{E}_{(s,a) \sim d^{\pi_\theta}_c} \left[ {\color{blue}w_{\sft}(s,a)} \nabla_\theta \log \pi_\theta(a \mid s) {\color{blue}r_{\sft}(s, a)} \right].
\end{align*}
with a reward as an indicator function of matching the expert trajectory and an importance weighting
\begin{align*}
w_{\sft}(s,a) = \frac{d_{\sft}(s,a)}{d^{\pi_\theta}_c}, \quad r_{\sft}(s, a) = \mathbf{1}[a =a^\star].
\end{align*}

While SFT reward $r_{\sft}$ achieves strong in-domain performance improvement due to teacher-forcing, its importance weight $w_{\sft}$ induces an distribution shift from the on-policy occupancy measure, leaning to poor generalizability.
To achieve the best of both worlds of SFT and RL, \name uses the same reward objective with a different pivot-based, value-sensitive weights:
\begin{align*}
w_{\name}(s,a) =\mathbf{1}(\mathrm{Gap}_c^\pi(s) > \delta)/Z
\end{align*}
where $Z = \E_{(s,a) \sim d^{\pi_\theta}_c}[\mathbf{1}(\mathrm{Gap}_c^\pi(s) > \delta)]$ is a normalization constant.
This gives rise to the following policy gradient that bridges SFT with RL
\begin{align*}
&~ \nabla_\theta \mathcal{L}_{\text{\name{}}}(\theta) = \\
&~ -\mathbb{E}_{(s,a) \sim d^{\pi_\theta}_c} \left[ {\color{blue}w_{\name}(s,a)} \nabla_\theta \log \pi_\theta(a \mid s) {\color{blue}r_{\sft}(s, a)} \right].
\end{align*}




==> sections/introduction_v2.tex <==
\section{Introduction\paragraph{Offline reward profiling.}
For each pivot candidate $(s,a^*) \in \mathcal{D}_{\mathrm{cand}}$, we sample
$M_{\mathrm{prof}}$ local rollouts under the frozen reference policy
$\pi_{\mathrm{ref}}$:
\[
a^{(1)},\dots,a^{(M_{\mathrm{prof}})} \sim \pi_{\mathrm{ref}}(\cdot \mid s).
\]
Let $r^{(m)}(s)$ denote the reward assigned to the $m$-th rollout at state $s$
(e.g., the local verifier reward). We define the empirical mean reward and
empirical reward variance at $s$ as
\[
\hat{\mu}(s)
=
\frac{1}{M_{\mathrm{prof}}}
\sum_{m=1}^{M_{\mathrm{prof}}} r^{(m)}(s),
\qquad
\hat{\sigma}^2(s)
=
\frac{1}{M_{\mathrm{prof}}}
\sum_{m=1}^{M_{\mathrm{prof}}}
\bigl(r^{(m)}(s)-\hat{\mu}(s)\bigr)^2.
\]
Intuitively, $\hat{\mu}(s)$ is the reference-policy success rate at pivot state
$s$, and $\hat{\sigma}^2(s)$ measures whether rollouts at $s$ have mixed
outcomes.

We then define the filtered pivot sets as
\[
\mathcal{D}_{\mathrm{mixed}}
=
\left\{
(s,a^*) \in \mathcal{D}_{\mathrm{cand}}
:\;
\hat{\sigma}^2(s) > 0
\right\},
\]
and
\[
\mathcal{D}_{\mathrm{adv}}
=
\left\{
(s,a^*) \in \mathcal{D}_{\mathrm{mixed}}
:\;
\hat{\mu}(s) < \lambda_{\mathrm{diff}}
\right\}.
\]}
\label{sec:introduction}

Large Language Models (LLMs) have increasingly relied on Supervised Fine-Tuning (SFT), which yields models strong on areas where the training data matches the distribution of the target area~\citep{chu2025sftmemorizesrlgeneralizes,wu2025generalization}. However, studies have shown clear weaknesses of SFT, of which includes catastrophic forgetting, where training on one distribution of data leads to the loss of capability in other distributions the model has been previously trained on \citep{shenfeld2025rlsrazoronlinereinforcement,chen2025retainingdoingroleonpolicy}. While a straightforward method of mitigating this effect is to train on a larger, broader set of SFT data \citep{luo2023empiricalCF,li2024revisitingCF,liu2025midtraining,lambert2025tulu3pushingfrontiers}, this approach contradicts learnings that the quality of SFT data is more important than quantity \citep{zhou2023limaalignment} and that SFT is more suitable as a jump start to the model \citep{chu2025sftmemorizesrlgeneralizes} rather than as a main driver.

Meanwhile, recent developments in Reinforcement Learning (RL) \citep{sutton1998reinforcement} have opened a new frontier for models in a variety of domains, including utilizing human feedback \citep{ouyang2022instructgpt} and verified rewards \citep{shao2024deepseekmath,Guo_2025} that scale with the experience gain of the model \citep{silver2025era}. With observations that RL does not suffer from the forgetting problem of SFT \citep{lu2025onpolicydistillation,shenfeld2025rlsrazoronlinereinforcement,chen2025retainingdoingroleonpolicy,chu2025sftmemorizesrlgeneralizes}, recent developments have increased the role of RL to be the driver of generalization and last-mile performance gain allowing its quick adoption as the final stage of training for many state-of-the-art models \citep{Guo_2025,qwen3technicalreport,kimiteam2025kimik2openagentic,5team2025glm45agenticreasoningcoding}.

In this paper, we step further from the observations about SFT and RL to question the utility of SFT in training models, especially in agentic capabilities. Many agentic tasks, such as conversational tool use, terminal use, software engineering, and search rely on heavy long horizon tool-calling. The common approach to training models for these capabilities has been SFT \citep{prabhakar2025apigenmtagenticpipelinemultiturn,qin2023toollLM,xu2023toolbench,liu2025toolacewinningpointsllm,pan2025trainingsoftwareengineeringagents,nakano2021webgpt}, empowered by long-horizon benchmarks spanning conversational tool use, terminal interaction, and web browsing/search \citep{yao2024taubench,barres2025tau2bench,tbench_2025,wei2025browsecompsimplechallengingbenchmark}. We propose that we can entirely replace SFT training of agentic capabilities by using a RL pipeline \textit{grounded} in the strengths of SFT \textit{without} the weaknesses of it. We first propose that any SFT dataset can be used for on-policy GRPO by using SFT prefixes as the input and the SFT completions as a verifier. We then propose a easy way to create such prefixes and verifiers by pointing out that agentic trajectories can be abstracted into an episodic MDP where each state is the result of tool-call.

Specifically, our contribution is as follows:
\begin{itemize}
    \item We show that any SFT dataset can be formulated into a GRPO setting by showing that the SFT verifier can be used as an RLVR verifier, and propose the resulting PivotRL method for consuming SFT data for on-policy RL training.
    \item We demonstrate that any agentic SFT dataset can formatted into the PivotRL setting by establishing long-horizon agentic trajectories as eposodic MDPs with distinct states (called `pivots') separated by tool call actions.
    \item We examine different dataset filtering strategies to choose a strong RL dataset from the existing SFT data, and show that PivotRL can improve \texttt{Qwen3-30B-A3b-Thinking-2507} from $44.35$ accuracy in $\tau^2$-Bench to $63.81$ in the best setting, which is better than the $58.44$ accuracy that is achievable by SFT.
    \item We show that PivotRL can serve as a general training strategy for a variety of agentic capabilities, with meaningful results in $\tau^2$-Bench \citep{barres2025tau2bench}, SWE-Bench \cite{jimenez2024swebench}, Terminal Bench \citep{tbench_2025}, and BrowseComp \citep{wei2025browsecompsimplechallengingbenchmark}.
\end{itemize}


% The common approach to training models that perform well on agentic capabilities has been through SFT \citep{prabhakar2025apigenmtagenticpipelinemultiturn,pan2025trainingsoftwareengineeringagents}\todo{CITE: More papers like One for terminal, BrowseComp etc}, which relies on a set of `golden' trajectories where each action in the trajectory is perceived as an optimal step in solving the underlying problem.

% In training agentic models, RLVR methods such as GRPO suffer from limitations of assigning equal reward for every token in the trajectory, which may unintentionally award suboptimal actions the model may have taken \cite{5team2025glm45agenticreasoningcoding}\todo{CITE MORE}.


==> sections/introduction_v3.tex <==
\section{Introduction}
\label{sec:intro}

Post-training for long-horizon agentic capabilities has a tension between efficiency and accuracy. By long-horizon, we mean tasks that require many turns of interaction with an environment, such as conversational tool use, code editing, terminal interaction, and web search. Supervised fine-tuning (SFT) is efficient, but it often degrades out-of-domain (OOD) accuracy. End-to-end reinforcement learning (E2E RL) preserves on-policy behavior and typically retains OOD performance better, but it is expensive because every update requires repeated full multi-turn environment interaction and can therefore be slow in wall-clock time. This raises a natural question: can we recover the accuracy and OOD retention of E2E RL without paying the full-trajectory rollout cost?

A natural first attempt is to reuse expert trajectories for RL. Given an SFT expert trajectory, we can sample an assistant turn, condition on the expert prefix, and roll out only the next assistant action rather than the full trajectory. This idea is appealing because it converts existing SFT data into RL data and reduces online interaction from full trajectories to one-turn. However, the naive version of this idea does not work well in practice. Randomly chosen turns often provide little or no learning signal, and just exact expert matching is too strict in generative action spaces, where many functionally appropriate actions differ from the single demonstrated completion.

Our core claim is that both issues matter. First, many intermediate turns are non-informative under group-normalized RL, such as GRPO: if sampled actions at a turn all succeed or all fail, the normalized advantage is zero and no update is produced. Second, strict matching misses credit for acceptable alternatives: a tool call, shell command, or search action may be functionally appropriate for that point in the trajectory without matching the expert string exactly. Such a method must therefore answer two questions at once: which turns are worth training on, and how should success be scored at those turns?

PivotRL makes these two requirements explicit. Demonstrations expose many intermediate decision states, but behavior cloning underuses them because it trains on only one demonstrated completion at each state. PivotRL performs local on-policy exploration around these states. It filters to what we call pivots---assistant turns whose sampled outcomes offer mixed outcomes ---and it optimizes a functional reward that credits any action judged appropriate by a domain verifier. Training then requires only one-turn or partial rollouts from those pivots, rather than full online trajectories.

We provide a lightweight analysis for both components. A simple proposition explains why mixed-outcome turns are the only ones that produce nonzero group-normalized updates, which motivates pivot selection. A KL-projection theorem explains why the functional reward induces a conservative update relative to the reference policy: it increases total probability on verifier-approved actions while preserving the reference ordering within and outside that set. We present this analysis as support for the method, not as a complete theory of forgetting.

We evaluate PivotRL in three ways. First, we compare it to SFT under identical training data---the same prompts and expert trajectories---and show larger in-domain gains with substantially smaller OOD regression. Across four training domains, PivotRL achieves an average in-domain gain of +14.11 points relative to the base model, compared with +9.94 for SFT, while average OOD change is +0.20 for PivotRL versus $-9.48$ for SFT. Second, on SWE-Bench, where E2E RL is a natural baseline, we show that PivotRL attains competitive accuracy with much lower rollout burden. Third, we ablate the two components of the method and show that both informative pivot selection and the functional reward are necessary for the strongest results.



==> sections/method.tex <==
\section{Method}
\label{sec:method}

\subsection{Bridging SFT with RL}
Supervised Fine-Tuning (SFT) Gradient can be rewritten as Policy Gradient via Importance Sampling~\citep{wu2025generalization}.
\begin{align*}
&~ \nabla_\theta \mathcal{L}_{\text{SFT}}(\theta) = \mathbb{E}_{(s, a^\star) \sim d_{\sft}} \left[ -\nabla_\theta \log \pi_\theta(a^\star \mid s) \right] \\
= &~ \mathbb{E}_{(s,a) \sim d^{\pi_\theta}_c} \frac{d_{\sft}(s,a)\mathbf{1}[a =a^\star]}{d^{\pi_\theta}_c} \left[ -\nabla_\theta \log \pi_\theta(a \mid s) \right] \\
= &~ -\mathbb{E}_{(s,a) \sim d^{\pi_\theta}_c} \left[ {\color{blue}w_{\sft}(s,a)} \nabla_\theta \log \pi_\theta(a \mid s) {\color{blue}r_{\sft}(s, a)} \right].
\end{align*}
with a reward as an indicator function of matching the expert trajectory and an importance weighting
\begin{align*}
w_{\sft}(s,a) = \frac{d_{\sft}(s,a)}{d^{\pi_\theta}_c}, \quad r_{\sft}(s, a) = \mathbf{1}[a =a^\star].
\end{align*}

While SFT reward $r_{\sft}$ achieves strong in-domain performance improvement due to teacher-forcing, its importance weight $w_{\sft}$ induces an distribution shift from the on-policy occupancy measure, leaning to poor generalization. 

To achieve the best of both worlds of SFT and RL, we must bridge the gap between the SFT state-action distribution $d_{\sft}(s,a)$ and the policy state-action distribution $d^{\pi_\theta}_c$, which would allow for an uncorrected Policy Gradient style update of $\pi_\theta$ on $(s, a^\star) \sim d_{\sft}$.

Our key observation is that autoregressive policy models are able to generate given any arbitrary sequence. Effectively, we can use any arbitrary $s \sim d_{\sft}$ to generate candidate actions $(a_1, a_2, \dots, a_n) \sim \pi_{\theta}(s)$. If $\sum_{i=0}^{n}\mathbf{1}[a_i = a^\star] > 0$, then we can employ the GRPO \citep{shenfeld2025rlsrazoronlinereinforcement} update directly, by employing $r_{\sft}(s, a) = \mathbf{1}[a = a^\star]$ as the reward function:

\begin{equation}
\mathcal{J}_{\text{PivotRL}}(\theta) = \mathbb{E}_{s \sim \mathcal{D}_{\sft}, \{a_i\}_{i=1}^G \sim \pi_{\theta_{\text{old}}}(\cdot \mid s)} \left[ \frac{1}{G} \sum_{i=1}^G \left( \min \left( w_i(\theta) \hat{A}_i, \text{clip}(w_i(\theta), 1-\varepsilon, 1+\varepsilon) \hat{A}_i \right) \right) \right]
\label{eq:pivotrl_loss}
\end{equation}

\noindent where the importance sampling ratio $w_i(\theta)$ and advantage $\hat{A}_i$ are:

\begin{equation}
w_i(\theta) = \frac{\pi_\theta(a_i \mid s)}{\pi_{\theta_{\text{old}}}(a_i \mid s)}, \qquad \hat{A}_i = \frac{r_{\sft}(s, a_i) - \text{mean}\left(\{r_{\sft}(s, a_j)\}_{j=1}^G\right)}{\text{std}\left(\{r_{\sft}(s, a_j)\}_{j=1}^G\right)}
\label{eq:pivot_definitions}
\end{equation}

The PivotRL loss uses the prefix states directly from the SFT dataset as $s \sim \mathcal{D}_{\sft}$, while sampling the actions directly from the policy $\pi_{\old}$, resulting in fully on-policy updates in relation to $\pi_{\old}$ while incentivizing the SFT dataset behavior $(s, a) \sim \mathcal{D}_{\sft}$ through employing $r_{\sft}(s, a) = \mathbf{1}[a =a^\star]$ as the reward function. 

Consequentially, for all generations the SFT importance weighting $w_{\sft}(s,a) = 1$, bridging the SFT style update into the policy gradient update when $r(s, a) = 1$ and thus incorporating the behavior cloning signal of SFT. In addition, we incorporate the negative samples where $r(s, a) \not= 1$ by adapting it into the contrastive GRPO loss to weigh the advantage term.

\input{sections/theory}

\subsection{From SFT Data to Partial Trajectories}

A typical SFT dataset of trajectories is defined as $\mathcal{D}_{\sft} = \{ \tau_i \}_{i=1}^N, \text { where } \tau = (s, a^\star)$, where $N$ is the number of trajectories, $s$ is the initial prompt, and $a$ is the trajectory completion, which may include multiple model completions, environment feedback such as tool responses, and formatting tokens. 
% In typical SFT and RL settings, loss is only applied to the model completions in order to avoid hallucinations \todo{cite relevant papers}.

To create candidate training samples $(s, a^\star) \sim \mathcal{D}_{\sft}$, we treat each trajectory $\tau$ as an episodic Markov Decision Process, where each trajectory is split into sequential states and actions by using each model completion as the boundary. For each $\tau \in \mathcal{D}_\sft$, we can split $\tau$ to $\tau = (s_0, a_0^\star, s_1, a_1^\star, \dots, s_{|\tau|}, a_{|\tau|}^\star)$, where $|\tau|$ is the number of model calls in $\tau$, $s_0$ is the initial prompt, $a_i$ is the model completion given $s_i$, and $s_{i+1}$ is the resulting state including the environmental feedback resulting from the action $a_i$ given $s_i$. This yields $\mathcal{D}_{\text{pivot}} = \{ (s_i, a_i^\star) \}_{i=1}^M$, where $M = \sum_{i=1}^N |\tau_i|$, which can be used for PivotRL training.

% This yields $\mathcal{D}_{\text{episode}} = \{ \tau_i \}_{i=1}^N, \text{ where } \tau = (s_0, a_0, s_1, a_1, \dots, s_{|\tau|}, a_{|\tau|})$, and $|\tau|$ is the number of model completions for the trajectory $\tau$. In this setting, $s_0$ is the initial prompt, $a_i$ is the model completion given $s_i$, and $s_{i+1}$ is the resulting state including the environmental feedback resulting from the action $a_i$ given $s_i$.

% In many LLMs, each $s_{i<j}$ may not be a strict prefix string of each $s_j$, especially with reasoning truncation in reasoning models \citep{qwen3technicalreport,deepseekai2025deepseekv32pushingfrontieropen,kimiteam2025kimik2openagentic}, yielding a dilemma in on-policy RL from rollouts generated from the initial prompt $s_0$ using standard RL methods \todo{cite more papers talking about this}.

% We mitigate this issue in PivotRL by flattening each $(s_i, a_i)$ pair as its own experience, such that $\mathcal{D}_{\text{episode}} = \{ (s_i, a_i, r_i) \}_{i=1}^M$ where $M = \sum_{i=1}^N |\tau_i|$, and $r_i$ is the reward associated with each model completion $a_i$ given state $s_i$. We refer to each triplet $(s_i, a_i, r_i)$ as a pivot. Given $\mathcal{D}_{\text{episode}}$, we can now train a policy $\pi$ by using a standard training approach without needing to mask parts of $a_i$.

\subsection{Reward Labeling for Pivots}
While the experience dataset $\mathcal{D}_{\text{pivot}} = \{ (s_i, a_i^*) \}_{i=1}^M$, provides a foundation for PivotRL training, in practice we cannot use it directly for training because the reward function, $r_{\sft}(s, a) = \mathbf{1}[a = a^\star]$ is not trivially defined. For example, in a coding task, two different coding snippets may functionally act in an equivalent way while being written in a different way.

Therefore in an effort to approximate $r_{\sft}(s, a) = \mathbf{1}[a = a^\star]$ efficiently, we propose the following variants:
\begin{itemize}
    \item String Comparison: We compare the string contents of $\hat{a}_i$ and $a_i^*$ directly, under some constraints. Practically, we employ direct string matching for short words while using an IOU-based comparison with a loose threshold.
    \item LLM-as-a-Judge~\citep{zheng2023judging, lee2023rlaif,tan2025judgebench}: We compare $\hat{a}_i$ and $a_i^*$ for some samples where string comparison is less meaningful by employing an equivalency judge for correctness. In practice, we may not need the $a_i^*$ in this case depending on the judge criterion.
\end{itemize}

Given the labeled data $\mathcal{D}_{\text{pivot}}$, we can train our policy using the PivotRL loss from Equation \ref{eq:pivotrl_loss}.


\subsection{Efficient Training via Pivot Selection}
As the PivotRL loss is intrinsically tied to the GRPO loss, the efficacy of training is heavily tied to the advantage term from $\hat{A}_i$ Equation \ref{eq:pivot_definitions}. For example, for a set of rollouts $(a_1, a_2, \dots, a_n) \sim \pi_{\theta}(s)$, the advantage behaves as follows:

\begin{equation}
    \hat{A}_i = 
    \begin{cases} 
      0 & \text{if } \sum_{j=1}^{N} r_\sft (s,a) = 0, \\
      0 & \text{if } \sum_{j=1}^{N} r_\sft (s,a) = N, \\
      \neq 0 & \text{if } 0 < \sum_{j=1}^{N} r_\sft (s,a) < N.
    \end{cases}
\end{equation}

When $\hat{A}_i = 0$, the surrogate loss term becomes $0$ and there is no derived training signal for that sample group. Consequently, we want to train on samples where $\hat{A}_i \not = 0$. To facilitate efficient training, we propose $3$ ways of filtering the PivotRL training data $\mathcal{D}_{\text{pivot}}$:
\begin{enumerate}
    \item Random Pivot ($\mathcal{D}_{\text{random}}$): This is the naive approach to using $\mathcal{D}_{\text{pivot}}$. We simply run RL on all samples from the dataset.
    \item Mixed Rewards ($\mathcal{D}_{\text{mixed}}$): We profile all samples in $\mathcal{D}_{\text{pivot}}$ on the untrained policy model $\pi_{ref}$, choosing only samples with nonzero reward variance over multiple rollouts.
    \item Advantage Gap ($\mathcal{D}_{\text{adv}}$): From the Mixed Rewards setting, we filter for samples which are difficult with a set threshold, artificially creating a large advantage gap for positive samples in the GRPO prompt group.
\end{enumerate}

\paragraph{Reward Profiling}
To curate each dataset variant, we first perform reward profiling using the initial policy $\pi_{ref}$. For every sample $(s_i, a_i) \in \mathcal{D}_{\text{pivot}}$, we execute $n$ independent rollouts using $\pi_{ref}$. Let $R_{i,k}$ denote the reward of the $k$-th rollout for the $i$-th sample. We compute the empirical mean return $\mu_i$ and reward variance $\sigma^2_i$ for sample $s_i$ as:
\begin{equation}
    \mu_i = \frac{1}{n} \sum_{k=1}^n R_{i,k}, \quad \sigma^2_i = \frac{1}{n-1} \sum_{k=1}^n (R_{i,k} - \mu_i)^2
\end{equation}

\subsubsection{Random Pivot}
The Random Pivot dataset utilizes the entire episodic history without filtering. It can be formalized as:
\begin{equation}
    \mathcal{D}_{\text{random}} = \mathcal{D}_{\text{pivot}}
\end{equation}

\subsubsection{Mixed Rewards}
The Mixed Rewards dataset filters for samples that exhibit reward variance in their outcomes under $\pi_0$:
\begin{equation}
    \mathcal{D}_{\text{mixed}} = \{ (s_i, a_i, r_i) \in \mathcal{D}_{\text{episode}} \mid \sigma^2_i > 0 \}
\end{equation}
Under the PivotRL training paradigm, this equates to filtering for any samples with nonzero advantage, maximizing training signal in the first training step.

One downside of the Mixed Rewards dataset is that it relies on profiled rewards from the initial policy $\pi_{ref}$. As the policy is updated during training, there is no guarantee that the advantage will stay nonzero for each sample. To mitigate this effect, we propose the advantage gap pivot selection method.

\subsubsection{Advantage Gap}
The Advantage Gap dataset focuses on samples that are both uncertain (from $\mathcal{D}_{\text{mixed}}$) and currently difficult for $\pi_0$. We apply a difficulty threshold $\lambda_{\text{diff}}$ to the mean return:
\begin{equation}
    \mathcal{D}_{\text{adv}} = \{ (s_i, a_i, r_i) \in \mathcal{D}_{\text{mixed}} \mid \mu_i < \lambda_{\text{diff}} \}
\end{equation}
Intuitively, taking harder questions under $\pi_0$ will partially as the policy $\pi_\theta$ progresses in traning, the harder samples continue to yield mixed rewards while easier samples tend zero advantage. This is akin to choosing samples with an artificially high advantage in GRPO training for positive rollouts.

Empirically, we find that by setting $\lambda_{\text{diff}} = 0.6$, the standard deviation of the rewards in a given train batch tend to be higher over a longer time than using $\mathcal{D}_{\text{random}}$ or $\mathcal{D}_{\text{mixed}}$, which is graphed in Figure \ref{fig:rl_tau_reward_stddev}. Surprisingly, we also see that the peak model accuracy to be higher when trained on $\mathcal{D}_{\text{adv}}$, yielding a stronger policy than when training under other dataset variants.

==> sections/method_v1.tex <==
\section{Method}
\label{sec:method}

\subsection{Full Offline Trajectories to Partial Trajecotories}
% A dataset of experiences, $\mathcal{D} = \{ \tau_i \}_{i=1}^N, \text{ where } \tau = (s_0, a_0, s_1, a_1, \dots, s_T, a_T)$, is defined as a collection of trajectories where $s_0$ is the initial prompt and each $a_i$ is an assistant completion step, and each $s_i$ is the resulting state after taking action $a_{i-1}$, which may include environment feedback. Standard long-horizon RL methods for LLMs, such as GRPO compresses the entire trajectory as one assistant action backpropagates only on the assistant $a_i$ tokens \citep{shao2024deepseekmathpushinglimitsmathematical} \todo{CITE for something like this}.

A typical dataset of trajectories is defined as $\mathcal{D}_{\tau} = \{ \tau_i \}_{i=1}^N, \text { where } \tau = (r, s, a)$, where $N$ is the number of trajectories, $r$ is the reward, $s$ is the initial prompt, and $a$ is the trajectory completion, which may include multiple model completions, environment feedback such as tool responses, and formatting tokens. In typical SFT and GRPO settings, loss is only applied to the model completions in order to avoid hallucinations \todo{cite relevant papers}.

In an episodic MDP setting, we explicitly split each trajectory into sequential states and actions by using each model completion as the boundary. This yields $\mathcal{D}_{\tau_\text{episode}} = \{ \tau_i \}_{i=1}^N, \text{ where } \tau = (r, s_0, a_0, s_1, a_1, \dots, s_{|\tau|}, a_{|\tau|})$, and $|\tau|$ is the number of model completions for the trajectory $\tau$. In this setting, $s_0$ is the initial prompt, $a_i$ is the full model completion given $s_i$, and $s_{i+1}$ is the resulting state including the environmental feedback resulting from the action $a_i$ given $s_i$.

In many LLMs, each $s_{i<j}$ may not be a strict prefix string of each $s_j$, especially with reasoning truncation in reasoning models \citep{qwen3technicalreport,deepseekai2025deepseekv32pushingfrontieropen,kimiteam2025kimik2openagentic}, yielding a dilemma in on-policy RL from rollouts generated from the initial prompt $s_0$ using standard RL methods \todo{cite more papers talking about this}.

We mitigate this issue in PivotRL by flattening each $(s_i, a_i)$ pair as its own experience, such that $\mathcal{D}_{\text{episode}} = \{ (s_i, a_i, r_i) \}_{i=1}^M$ where $M = \sum_{i=1}^N |\tau_i|$, and $r_i$ is the reward associated with each model completion $a_i$ given state $s_i$. We refer to each triplet $(s_i, a_i, r_i)$ as a pivot. Given $\mathcal{D}_{\text{episode}}$, we can now train a policy $\pi$ by using a standard training approach without needing to mask parts of $a_i$.

\subsection{Reward Labeling for Pivots}
The PivotRL dataset $\mathcal{D}_{\text{episode}} = \{ (s_i, a_i, r_i) \}_{i=1}^M$ depends on having dense labels $r_i$ for each state-action pair which is often non-trivial to obtain. Especially with experiences gained from the verified rewards setting \citep{shao2024deepseekmath,lambert2025tulu3pushingfrontiers,pyatkin2025generalizingverifiableinstructionfollowing}, where the only reward signal is from the final outcome, there is no trivial way to label each action with a process reward. Existing approaches that do not involve human labeling include using a explicit Process Reward Model \citep{lightman2023letsverifystepstep}, Monte Carlo Tree Search \citep{xin2024deepseekproverv15harnessingproofassistant,luo2024improvemathematicalreasoninglanguage}, heuristics-based search \citep{dong2025agenticreinforcedpolicyoptimization} or intermdiate state densification \citep{luo2025agentlightningtrainai} \todo{add more citations}.

We build upon the core insight that the goal for SFT data is to curate high quality trajectories \citep{zhou2023limaalignment}. Under the assumption that each trajectory $\tau_i$ is the optimal completion given the initial prompt $s_0$, we can assume every $a_i$ to be the optimal completion given each $s_i$. We label this optimal action as $a_i^*$. Then, for any alternate response $\hat{a_i}$, we have:
\begin{equation}
    r_i = \begin{cases} 
        1 & \text{if } f(\hat{a}_i, a_i^*) = 1 \\
        0 & \text{otherwise}
    \end{cases}
\end{equation}
where $f(\hat{a}_i, a_i^*)$ is a comparison function between two actions.

The choice for $f(\hat{a}_i, a_i^*)$ can be arbitrary. For simplicity, we consider the following variants:
\begin{itemize}
    \item String Comparison: We compare the string contents of $\hat{a}_i$ and $a_i^*$ directly, under some constraints. For example, under the OpenAI tool call schema \citep{OpenAI_Function_Calling} \todo{DO I NEED TO CITE THIS ?}, each tool call has a name and arguments defined in a python dictionary structure. For fields that are one-word in $a_i^*$ we employ strict comparisons, which is in practice tool names, or fields such as filenames for SWE tasks. For fields that are multiple words in $a_i^*$, we employ an IOU-based comparison with a loose threshold, which in practice matches for fields such as search queries or code bodies.
    \item LLM-as-a-Judge\todo{cite}: We compare $\hat{a}_i$ and $a_i^*$ for some samples where string comparison is less meaningful by employing LLM-as-a-Judge for correctness. In practice, we may not need the $a_i^*$ in this case depending on the judge criterion.
\end{itemize}

Finally, given the labeled data $\mathcal{D}_{\text{episode}}$, we can train our policy using the standard GRPO \citep{shao2024deepseekmath} loss:

\begin{align}
L_{GRPO}(\theta) = \mathbb{E} \Bigg[ \frac{1}{G} \sum_{i=1}^G \bigg( \min \Big( \text{IS}_i(\theta) A_i, \, \text{clip}(\text{IS}_i(\theta), 1-\epsilon, 1+\epsilon) A_i \Big) - \beta D_{KL}(\pi_\theta || \pi_{ref}) \bigg) \Bigg]
\end{align}
where $\text{IS}_i(\theta) = \frac{\pi_\theta(o_i | q)}{\pi_{old}(o_i | q)}$ is the importance sampling ratio and $A_i = \frac{r_i - \frac{1}{G} \sum_{j=1}^G r_j}{\text{std}(r_1, \dots, r_G)}$ is the advantage of each action.


\subsection{Pivot Selection Strategies}
We propose 3 variants of training on $\mathcal{D}_{\text{episode}}$:
\begin{enumerate}
    \item Random Pivot: This is the naive approach to using $\mathcal{D}_{\text{episode}}$. We simply run RL on all samples from the dataset.
    \item Mixed Rewards: We profile all samples in $\mathcal{D}_{\text{episode}}$ on the untrained policy model $pi_0$, choosing only samples with variance in rewards over multiple rollouts.
    \item Advantage Gap: From the Mixed Rewards setting, we filter for samples which are difficult with a set threshold.
\end{enumerate}

\paragraph{Reward Profiling}
To curate the dataset, we first perform reward profiling using the initial policy $\pi_0$. For every sample $(s_i, a_i) \in \mathcal{D}_{\text{episode}}$, we execute $n$ independent rollouts using $\pi_0$. Let $R_{i,k}$ denote the cumulative reward of the $k$-th rollout for the $i$-th sample. We compute the empirical mean return $\mu_i$ and reward variance $\sigma^2_i$ as:
\begin{equation}
    \mu_i = \frac{1}{n} \sum_{k=1}^n R_{i,k}, \quad \sigma^2_i = \frac{1}{n-1} \sum_{k=1}^n (R_{i,k} - \mu_i)^2
\end{equation}

\subsubsection{Random Pivot}
The Random Pivot dataset utilizes the entire episode history without filtering. It can be formalized as:
\begin{equation}
    \mathcal{D}_{\text{random}} = \mathcal{D}_{\text{episode}}
\end{equation}

\subsubsection{Mixed Rewards}
The Mixed Rewards dataset filters for samples that exhibit stochasticity or uncertainty in their outcomes under $\pi_0$. We select samples where the reward variance exceeds a small threshold $\epsilon_{\text{var}}$:
\begin{equation}
    \mathcal{D}_{\text{mixed}} = \{ (s_i, a_i, r_i) \in \mathcal{D}_{\text{episode}} \mid \sigma^2_i > \epsilon_{\text{var}} \}
\end{equation}
Empirically, we choose $\epsilon_{\text{var}} = 0$, which would choose any samples with variance. Under the GRPO paradigm, this equates to filtering for any samples with non-zero advantage, maximizing training signal in the first training step.

One downside of the Mixed Rewards dataset is that it relies on profiled rewards from the initial policy $pi_0$. During training, while the initial step will only contain samples with non-zero advantage, as the policy is updated, there is no longer such a guarantee. To mitigate this effect, we propose the advantage gap pivot selection method

\subsubsection{Advantage Gap}
The Advantage Gap dataset focuses on samples that are both uncertain (from $\mathcal{D}_{\text{mixed}}$) and currently difficult for $pi_0$. We apply a difficulty threshold $\lambda_{\text{diff}}$ to the mean return:
\begin{equation}
    \mathcal{D}_{\text{adv}} = \{ (s_i, a_i, r_i) \in \mathcal{D}_{\text{mixed}} \mid \mu_i < \lambda_{\text{diff}} \}
\end{equation}
Intuitively, taking harder questions under $\pi_0$ will partially mitigate all samples yielding reward $1$ under a trained policy $\pi_t$, as even though $\pi_t$ does overall better in the set of $\mathcal{D}_{\text{mixed}}$, the harder samples continue to yield mixed rewards as easier samples tend $0$ advantage.

Empirically, we find that by $\lambda_{\text{diff}} = 0.6$, we see that the standard deviation of the rewards in a given batch tend to be higher across more training steps than using $\mathcal{D}_{\text{random}}$ or $\mathcal{D}_{\text{mixed}}$. Surprisingly, we also see that the peak model accuracy to be higher when trained on $\mathcal{D}_{\text{adv}}$, yielding a stronger policy than when training under other dataset variants.

==> sections/method_v2.tex <==
\section{Method}
\label{sec:method}

\subsection{Bridging SFT with End-to-End RL}

Consider training an LLM on Supervised Fine-Tuning (SFT) trajectories $\mathbf{t}^* = (t_1^*, \dots, t_{N}^*) \sim d_{\sft}$, where at each position $n$, the expert demonstrates the ground-truth next token $t_n^*$ conditioned on the prefix $t_{1:n-1}^*$. The standard SFT objective is
\begin{align*}
\mathcal{L}_{\text{SFT}}(\theta)
= -\mathbb{E}_{\mathbf{t}^* \sim d_{\sft}}
\left[
\sum_{n=1}^{N}
\log \pi_\theta(t_n^* \mid t_{1:n-1}^*)
\right].
\end{align*}
Formally, its gradient can be rewritten as a policy gradient with an indicator reward
\(
r_{\sft}(t_{1:n-1}, t_n) = \mathbf{1}[t_n = t_n^*]
\)
and an importance weight correcting for the mismatch between the SFT data distribution and the on-policy occupancy:
\begin{align*}
\nabla_\theta \mathcal{L}_{\text{SFT}}(\theta)
= -\mathbb{E}_{(t_{1:n-1}, t_n) \sim d^{\pi_\theta}_c}
\left[
{\color{blue}w_{\sft}(t_{1:n-1}, t_n)}
\nabla_\theta \log \pi_\theta(t_n \mid t_{1:n-1})
\cdot
{\color{blue}r_{\sft}(t_{1:n-1}, t_n)}
\right],
\end{align*}
where
\(
w_{\sft}(t_{1:n-1}, t_n)
=
{d_{\sft}(t_{1:n-1}, t_n)}/{d^{\pi_\theta}_c(t_{1:n-1}, t_n)}
\)
and
\(
r_{\sft}(t_{1:n-1}, t_n)
=
\mathbf{1}[t_n = t_n^*].
\)

In agentic LLM fine-tuning, this formulation reveals two limitations of SFT:
\begin{itemize}
    \item First, the indicator reward ${\color{blue}r_{\sft}(t_{1:n-1}, t_n)} = \mathbf{1}[t_n = t_n^*]$ assigns zero reward to all tokens except the single expert token $t_n^*$ at prefix $t_{1:n-1}$. In generative agentic tasks, however, the output space is combinatorially large. A single tool call can be expressed in many functionally equivalent ways; a coding fix may use different variable names, control flow structures, or API calls while achieving identical outcomes. When SFT trains the model to reproduce one particular expert completion, the model receives no information about what would happen if it generated a slightly different token at some prefix. Therefore, the reward is not fully aligned with the true functional ability required by the task.
    \item Second, the importance weight ${\color{blue}w_{\sft}}$ induces distribution shift from the on-policy occupancy measure. This introduces an ill-posed reward landscape, where the importance weight becomes large for low-probability tokens. As argued by \citet{wu2025generalization}, this leads to gradient mismatch and training instability, ultimately weakening the model’s ability to generalize to new problems the model has not seen during training.
\end{itemize}

To overcome these issues, PivotRL employs the following two approaches:
\begin{itemize}
    \item To address the first issue, PivotRL extends the \emph{token-level, strict-matching} reward $r_{\sft}$ to a \emph{turn-level, functional-matching} reward $r_{\name}$ which models each action as a complete model response turn and replaces exact token matching by functional matching empowered by string comparison or LLM-as-a-Judge. This exploits the flexibility of autoregressive policy model to generate arbitrary response sequence conditional on prefix turns, and allows mapping different thinking traces with same output as all correct.
    \item To address the second issue, PivotRL develops a \emph{pivot selection} mechanism to filter the states and keep only informative turns where the advantage gap is large. These pivots are associated with optimal behavior policies~\citep{papini2024policy} and represents states where training can make more progress.
\end{itemize}
In the following sections, we will explain these designs in detail.

\subsection{Turn-Level, Functional-Matching Reward}

\subsubsection{From SFT Data to Partial Trajectories}

We write a typical SFT dataset of trajectories as $\mathcal{D}_{\sft} = \{ \tau_i \}_{i=1}^N$, where $N$ is the number of trajectories. 
To create candidate training samples $(s, a^\star) \sim \mathcal{D}_{\sft}$, we treat each trajectory $\tau$ as an episodic Markov Decision Process, where each trajectory is split into sequential states and actions by using each model completion as the boundary. For each $\tau \in \mathcal{D}_\sft$, we can split $\tau$ to $\tau = (s_0, a_0^\star, s_1, a_1^\star, \dots, s_{|\tau|}, a_{|\tau|}^\star)$, where $|\tau|$ is the number of model calls in $\tau$, $s_0$ is the initial prompt, $a_i$ is the model completion given $s_i$, and $s_{i+1}$ is the resulting state including the environmental feedback resulting from the action $a_i$ given $s_i$. This yields $\mathcal{D}_{\text{pivot}} = \{ (s_i, a_i^\star) \}_{i=1}^M$, where $M = \sum_{i=1}^N |\tau_i|$, which can be used for PivotRL training.

\subsubsection{Reward Labeling on Tangential Rollouts}
We apply RL on tangential rollouts: for each state-action pair $(s,a^\star(s))$ from the expert dataset $\mathcal{D}_{\text{pivot}}$, we sample multiple on-policy actions $a$ conditional on the state $s$ and label the reward of $a$ by comparing with demonstration $a^\star(s)$. This alleviates the computation overhead in comparison to full rollouts. However, the SFT reward function $r_{\sft}(s,a) = \mathbf{1}[a = a^\star(s)]$ is not suitable for RL because it enforces strict matching to the ground-truth $a^\star(s)$ while overlooking many other functionally-equivalent actions. For example, in a coding task, two different coding snippets may functionally act in an equivalent way while being written in a different way.

Therefore, we introduce reward 
\begin{align}\label{eq:pivotrl-reward}
    r_{\name}(s, a) = \mathbf{1}[a\in \mathcal M_\epsilon(s)]
\end{align}
that assigns value $1$ to all candidate responses in the matching set
$\mathcal M_\epsilon(s)
=
\{a\in\mathcal A:d(a,a^\star(s))\leq \epsilon\}$, 
where $d$ is some distance function. Efficiently, we propose the following variants of $d$:
\begin{itemize}
    \item String Comparison: We compare the string contents of $\hat{a}_i$ and $a_i^*$ directly, under some constraints. Practically, we employ direct string matching for short words while using an IOU-based comparison with a loose threshold.
    \item LLM-as-a-Judge~\citep{zheng2023judging, lee2023rlaif,tan2025judgebench}: We compare $\hat{a}_i$ and $a_i^*$ for some samples where string comparison is less meaningful by employing an equivalency judge for correctness. In practice, we may not need the $a_i^*$ in this case depending on the judge criterion.
\end{itemize}


\input{sections/theory}


\subsection{Efficient Training via Pivot Selection}
As the PivotRL loss is intrinsically tied to the GRPO loss, the efficacy of training is heavily tied to the advantage term from $\hat{A}_i$ Equation \ref{eq:pivot_definitions}. For example, for a set of rollouts $(a_1, a_2, \dots, a_n) \sim \pi_{\theta}(s)$ with rewards $(R_1,\dots,R_n)$, the advantage behaves as follows:

\begin{equation}
    \hat{A}_i = 
    \begin{cases} 
      0 & \text{if } \sum_{j=1}^{N} R_j = 0, \\
      0 & \text{if } \sum_{j=1}^{N} R_j = N, \\
      \neq 0 & \text{if } 0 < \sum_{j=1}^{N} R_j < N.
    \end{cases}
\end{equation}

When $\hat{A}_i = 0$, the surrogate loss term becomes $0$ and there is no derived training signal for that sample group. Consequently, we want to train on samples where $\hat{A}_i \not = 0$. To facilitate efficient training, we propose $3$ ways of filtering the PivotRL training data $\mathcal{D}_{\text{pivot}}$:
\begin{enumerate}
    \item Random Pivot ($\mathcal{D}_{\text{random}}$): This is the naive approach to using $\mathcal{D}_{\text{pivot}}$. We simply run RL on all samples from the dataset.
    \item Mixed Rewards ($\mathcal{D}_{\text{mixed}}$): We profile all samples in $\mathcal{D}_{\text{pivot}}$ on the untrained policy model $\pi_{ref}$, choosing only samples with nonzero reward variance over multiple rollouts.
    \item Advantage Gap ($\mathcal{D}_{\text{adv}}$): From the Mixed Rewards setting, we filter for samples which are difficult with a set threshold, artificially creating a large advantage gap for positive samples in the GRPO prompt group.
\end{enumerate}

\paragraph{Reward Profiling}
To curate each dataset variant, we first perform reward profiling using the initial policy $\pi_{ref}$. For every sample $(s_i, a_i) \in \mathcal{D}_{\text{pivot}}$, we execute $n$ independent rollouts using $\pi_{ref}$. Let $R_{i,k}$ denote the reward of the $k$-th rollout for the $i$-th sample. We compute the empirical mean return $\mu_i$ and reward variance $\sigma^2_i$ for sample $s_i$ as:
\begin{equation}
    \mu_i = \frac{1}{n} \sum_{k=1}^n R_{i,k}, \quad \sigma^2_i = \frac{1}{n-1} \sum_{k=1}^n (R_{i,k} - \mu_i)^2
\end{equation}

\subsubsection{Random Pivot}
The Random Pivot dataset utilizes the entire episodic history without filtering. It can be formalized as:
\begin{equation}
    \mathcal{D}_{\text{random}} = \mathcal{D}_{\text{pivot}}
\end{equation}

\subsubsection{Mixed Rewards}
The Mixed Rewards dataset filters for samples that exhibit reward variance in their outcomes under $\pi_0$:
\begin{equation}
    \mathcal{D}_{\text{mixed}} = \{ (s_i, a_i, r_i) \in \mathcal{D}_{\text{episode}} \mid \sigma^2_i > 0 \}
\end{equation}
Under the PivotRL training paradigm, this equates to filtering for any samples with nonzero advantage, maximizing training signal in the first training step.

One downside of the Mixed Rewards dataset is that it relies on profiled rewards from the initial policy $\pi_{ref}$. As the policy is updated during training, there is no guarantee that the advantage will stay nonzero for each sample. To mitigate this effect, we propose the advantage gap pivot selection method.

\subsubsection{Advantage Gap}
The Advantage Gap dataset focuses on samples that are both uncertain (from $\mathcal{D}_{\text{mixed}}$) and currently difficult for $\pi_0$. We apply a difficulty threshold $\lambda_{\text{diff}}$ to the mean return:
\begin{equation}
    \mathcal{D}_{\text{adv}} = \{ (s_i, a_i, r_i) \in \mathcal{D}_{\text{mixed}} \mid \mu_i < \lambda_{\text{diff}} \}
\end{equation}
Intuitively, taking harder questions under $\pi_0$ will partially as the policy $\pi_\theta$ progresses in traning, the harder samples continue to yield mixed rewards while easier samples tend zero advantage. This is akin to choosing samples with an artificially high advantage in GRPO training for positive rollouts.

Empirically, we find that by setting $\lambda_{\text{diff}} = 0.6$, the standard deviation of the rewards in a given train batch tend to be higher over a longer time than using $\mathcal{D}_{\text{random}}$ or $\mathcal{D}_{\text{mixed}}$, which is graphed in Figure \ref{fig:rl_tau_reward_stddev}. Surprisingly, we also see that the peak model accuracy to be higher when trained on $\mathcal{D}_{\text{adv}}$, yielding a stronger policy than when training under other dataset variants.

\subsection{PivotRL Loss}

Combining everything together, we introduce the following PivotRL loss:
\begin{equation}
\mathcal{J}_{\text{PivotRL}}(\theta) = \mathbb{E}_{s \sim \mathcal{D}_{\text{adv}}, \{a_i\}_{i=1}^G \sim \pi_{\theta_{\text{old}}}(\cdot \mid s)} \left[ \frac{1}{G} \sum_{i=1}^G \left( \min \left( w_i(\theta) \hat{A}_i, \text{clip}(w_i(\theta), 1-\varepsilon, 1+\varepsilon) \hat{A}_i \right) \right) \right]
\label{eq:pivotrl_loss}
\end{equation}

\noindent where the importance sampling ratio $w_i(\theta)$ and advantage $\hat{A}_i$ are:

\begin{equation}
w_i(\theta) = \frac{\pi_\theta(a_i \mid s)}{\pi_{\theta_{\text{old}}}(a_i \mid s)}, \qquad \hat{A}_i = \frac{r_{\name}(s, a_i) - \text{mean}\left(\{r_{\name}(s, a_j)\}_{j=1}^G\right)}{\text{std}\left(\{r_{\name}(s, a_j)\}_{j=1}^G\right)}
\label{eq:pivot_definitions}
\end{equation}

==> sections/method_v3.tex <==
\section{Preliminary and Motivating Observations}
\label{sec:prelim}

This section motivates PivotRL through the simplest possible baseline. We first show how expert trajectories from SFT naturally induce turn-level decision states. We then evaluate a naive construction based on random pivots, and finally isolate the two bottlenecks that motivate the full method. We keep this section deliberately short; the complete training pipeline and analysis appear in Section~\ref{sec:pivotrl}.

\paragraph{From expert trajectories to RL candidates.}
Let $\mathcal{D}_{\mathrm{sft}}=\{\tau_i\}_{i=1}^N$ denote the expert trajectory dataset used for SFT. We decompose each trajectory at assistant decision boundaries: $\tau = (s_0, a_0^*, s_1, a_1^*, \ldots, s_T, a_T^*)$, where $s_t$ -- the full trajectory history from the beginning -- is the interaction state before the $t$-th assistant action and $a_t^*$ is the demonstrated assistant completion at that state.
Here, $s_t$ includes the full interaction prefix up to that point, including prior tool results or environment feedback. We call each extracted pair $(s_t,a_t^*)$ a \emph{pivot candidate}. A \emph{pivot} is a pivot candidate that is retained for PivotRL training after offline filtering. Throughout the paper, an \emph{action} means the full assistant completion at a model-call boundary, not an individual token.

This decomposition turns the original trajectory dataset into a set of local decision problems: $\mathcal{D}_{\mathrm{cand}}=\{(s_t,a_t^*)\}_{t=0}^T.$

A local RL example is formed by conditioning on the demonstrated prefix $s_t$, replacing the next assistant action with an on-policy sample $a \sim \pi_\theta(\cdot \mid s_t)$, and executing only the short rollout needed to score that action.

\paragraph{Naive Baseline: random pivots with strict reward.}
The simplest possible baseline samples pivot candidates uniformly from $\mathcal{D}_{\mathrm{cand}}$ and rewards the sampled action only if it exactly matches the demonstrated completion:
\[
r_{\mathrm{strict}}(s,a)=\mathbf{1}[a=a^*(s)].
\]
We refer to this baseline as \emph{random pivot RL with strict reward}. It is the most direct way to turn SFT trajectories into turn-level RL data, and it provides the cleanest starting point for understanding what is missing.

\paragraph{Random pivots alone do not suffice.}
In practice, naive baseline does not recover the behavior of the full method in terms of the in-domain improvement. In the strict preliminary setting, random pivots with exact matching reach only \texttt{[PLACEHOLDER: random+strict result]}, which is substantially lower than the 63.81\% achieved by the full method. Even under the more permissive reward used in our current $\tau^2$ study, random pivots reach 59.68, only slightly above same-data SFT at 58.44 and still below informative pivot selection at 63.81. This already suggests that simply converting SFT traces into examples is not enough: the quality of the pivot states and the reward both matter.

\paragraph{Bottleneck analysis.}
Two issues explain why the naive baseline is weak.

\emph{(1) Random pivots do not provide enough signal.}
Under group-normalized RL, a state produces no update if all sampled actions succeed or all sampled actions fail. If $\{r_i\}_{i=1}^G$ are the rewards of a rollout group at state $s$, the normalized advantage takes the form
\[
\hat{A}_i=\frac{r_i-\frac{1}{G}\sum_{j=1}^G r_j}{\mathrm{std}(\{r_j\}_{j=1}^G)}.
\]
When all rewards are identical, every $\hat{A}_i$ is zero. Empirically, this is exactly what we observe under random pivot sampling: the per-batch reward standard deviation decays rapidly during training, indicating that many turns quickly become uninformative.

\emph{(2) Strict reward misses a large fraction of useful signal.}
Exact expert matching is too sparse in generative action spaces. Many tool calls, shell commands, or search actions are functionally correct without matching the demonstrated string exactly. To quantify this, we compare strict matching to a domain-appropriate verifier and measure
\[
\mathrm{MissRate}
=
\Pr\!\left[r_{\mathrm{strict}}(s,a)=0 \;\middle|\; r_{\mathrm{func}}(s,a)=1\right].
\]
In our preliminary analysis, strict matching misses positive credit on \texttt{[PLACEHOLDER: miss-rate]}\% of verifier-approved rollouts. This means that even when a sampled action is locally acceptable, strict reward often labels it as failure.

\paragraph{Takeaway.}
These observations motivate the full PivotRL design. Effective RL from expert trajectories requires both \emph{informative pivot selection}, to avoid wasting updates on zero-signal states, and a \emph{functional reward}, to credit acceptable alternatives rather than only the single demonstrated completion.

\section{PivotRL}
\label{sec:pivotrl}

This section presents the full PivotRL method and the analysis that supports its two components. Section~\ref{sec:pivotrl_method} describes the training pipeline: offline pivot selection, functional reward construction, and the GRPO-style objective used for optimization. Section~\ref{sec:pivotrl_analysis} then explains why these choices are well matched to local on-policy RL. In particular, we first show why mixed-outcome turns are the only ones that produce nonzero group-normalized updates, and then show that the functional reward induces a conservative KL-regularized update relative to the reference policy.

\subsection{Method}
\label{sec:pivotrl_method}

Starting from the pivot candidates constructed in Section~\ref{sec:prelim}, PivotRL proceeds in three steps: (i) profile and filter those candidates to obtain informative pivots, (ii) sample local on-policy rollouts at the retained pivots, and (iii) optimize a functional reward with a GRPO-style update. Algorithm~\ref{alg:pivotrl} summarizes the full pipeline.

\paragraph{Pivot selection.}
Not every pivot candidate is useful for training. We therefore profile the candidate set offline under a frozen reference policy $\pi_{\mathrm{ref}}$. For each candidate state $s$, we sample multiple local rollouts, compute their rewards, and estimate an empirical mean return $\hat{\mu}(s)$ and reward variance $\hat{\sigma}^2(s)$. Full profiling details and hyperparameters are deferred to the appendix; in the main text, we only use the resulting filtered sets:
\[
\mathcal{D}_{\mathrm{random}}=\mathcal{D}_{\mathrm{cand}},
\]
\[
\mathcal{D}_{\mathrm{mixed}}=\left\{(s,a^*)\in\mathcal{D}_{\mathrm{cand}} \;:\; \hat{\sigma}^2(s)>0\right\},
\]
\[
\mathcal{D}_{\mathrm{adv}}=\left\{(s,a^*)\in\mathcal{D}_{\mathrm{mixed}} \;:\; \hat{\mu}(s)<\lambda_{\mathrm{diff}}\right\}.
\]

The random set is the naive baseline. The mixed set keeps only states whose rollouts under $\pi_{\mathrm{ref}}$ have nonzero reward variance, i.e., states that can produce nonzero group-normalized updates at the beginning of training. The advantage-gap set is a stricter subset of difficult mixed-outcome states. Intuitively, these harder pivots remain informative longer as the policy improves. Unless otherwise stated, PivotRL uses $\mathcal{D}_{\mathrm{adv}}$ as its training set.

\paragraph{Functional reward.}
At a retained pivot state $s$, PivotRL samples actions from the current policy and scores them with a functional verifier rather than exact expert matching. Let $\mathcal{M}(s)\subseteq\mathcal{A}(s)$ denote the set of \emph{acceptable} actions at state $s$, where acceptability is defined by a domain-specific verifier. We then define the functional reward
\begin{align}\label{eq:func_reward}
r_{\mathrm{func}}(s,a)=\mathbf{1}[a\in\mathcal{M}(s)].
\end{align}
This replaces the strict reward
\[
r_{\mathrm{strict}}(s,a)=\mathbf{1}[a=a^*(s)].
\]

The verifier depends on the domain. In some settings, acceptability can be checked by normalized string or schema-based comparison; in others, it is better captured by a lightweight LLM judge or a task-specific equivalence rule. The key point is that PivotRL rewards \emph{functional equivalence at the local decision point}.

\paragraph{PivotRL objective.}
Given a filtered pivot dataset $\mathcal{D}_{\mathrm{pivot}}$ and a rollout group size $G$, PivotRL optimizes a clipped GRPO-style objective over local on-policy samples:
\[
\mathcal{J}_{\mathrm{PivotRL}}(\theta)
=
\mathbb{E}_{s\sim\mathcal{D}_{\mathrm{pivot}},\{a_i\}_{i=1}^G\sim\pi_{\theta_{\mathrm{old}}}(\cdot\mid s)}
\left[
\frac{1}{G}
\sum_{i=1}^G
\min\!\Big(
w_i(\theta)\hat{A}_i,
\mathrm{clip}(w_i(\theta),1-\epsilon,1+\epsilon)\hat{A}_i
\Big)
\right],
\]
where
\[
w_i(\theta)=\frac{\pi_\theta(a_i\mid s)}{\pi_{\theta_{\mathrm{old}}}(a_i\mid s)},
\qquad
\hat{A}_i=
\frac{
r_{\mathrm{func}}(s,a_i)-\mathrm{mean}\!\left(\{r_{\mathrm{func}}(s,a_j)\}_{j=1}^G\right)
}{
\mathrm{std}\!\left(\{r_{\mathrm{func}}(s,a_j)\}_{j=1}^G\right)
}.
\]
Compared with E2E RL, this objective requires only one-turn or partial rollouts from pivot states. Compared with SFT, it uses a set-valued verifier-based reward.

\paragraph{Full algorithm.}
Algorithm~\ref{alg:pivotrl} summarizes the entire method. The only online interaction during training is the local rollout required to score sampled actions at the selected pivots.

\begin{algorithm}[t]
\caption{PivotRL}
\label{alg:pivotrl}
\begin{algorithmic}[1]
\State \textbf{Require:} Expert trajectories $\mathcal{D}_{\mathrm{sft}}$, reference policy $\pi_{\mathrm{ref}}$, initial policy $\pi_\theta$, verifier $V$, rollout group size $G$, difficulty threshold $\lambda_{\mathrm{diff}}$
\State Extract pivot candidates $\mathcal{D}_{\mathrm{cand}}=\{(s_t,a_t^*)\}$ from expert trajectories
\State Profile each candidate under $\pi_{\mathrm{ref}}$ to estimate $\hat{\mu}(s)$ and $\hat{\sigma}^2(s)$
\State Construct $\mathcal{D}_{\mathrm{pivot}}$ by filtering to mixed-outcome pivots, optionally retaining only difficult ones
\For{training step $k=1,\dots,K$}
    \State Sample a minibatch of pivot states $\{s_b\}_{b=1}^B$ from $\mathcal{D}_{\mathrm{pivot}}$
    \For{each pivot state $s_b$}
        \State Sample rollout group $\{a_{b,i}\}_{i=1}^G \sim \pi_{\theta_{\mathrm{old}}}(\cdot\mid s_b)$
        \State Execute the local rollout needed to score each action
        \State Compute rewards $r_{\mathrm{func}}(s_b,a_{b,i})$ using verifier $V$
        \State Compute normalized advantages $\hat{A}_{b,i}$
    \EndFor
    \State Update $\pi_\theta$ with the clipped objective in Eq.~(8)
\EndFor
\end{algorithmic}
\end{algorithm}

\subsection{Theoretical analysis for PivotRL}
\label{sec:pivotrl_analysis}

We now analyze the two core design choices separately: the functional reward in Eq.~\eqref{eq:func_reward} and the pivot selection scheme in Section~\ref{sec:pivotrl_method}. Our first result shows that KL-regularized RL with the functional reward improves the probability on acceptable actions $\mathcal{M}(s)$ while preserving the conditional distribution on both $\mathcal{M}(s)$ and its compliment $\mathcal{M}(s)^c$. Our second result shows that selecting pivots with large reward variance improves the natural-gradient norma and GRPO score along the KL-path, thus filtering for stronger learning signals.
Throughout this section, we assume the action space $\mathcal{A}$ is finite, $\mathcal{M}(s) \neq \emptyset$, and $\pi_0(a\mid s)>0$ for all $s$ and $a$. 

\iffalse
\paragraph{SFT as policy gradient.}
Consider an expert token trajectory $t^*=(t_1^*,\ldots,t_N^*)\sim d_{\mathrm{sft}}$. The SFT objective is
\[
\mathcal{L}_{\mathrm{SFT}}(\theta)
=
-
\mathbb{E}_{t^*\sim d_{\mathrm{sft}}}
\left[
\sum_{n=1}^N
\log \pi_\theta(t_n^* \mid t_{<n}^*)
\right].
\]
This gradient can be rewritten as a policy gradient with a strict exact-match reward and an off-policy correction term:
\[
\nabla_\theta \mathcal{L}_{\mathrm{SFT}}(\theta)
=
-
\mathbb{E}_{(h,a)\sim d_{\pi_\theta}}
\left[
w_{\mathrm{sft}}(h,a)\,
\nabla_\theta \log \pi_\theta(a\mid h)\,
r_{\mathrm{strict}}(h,a)
\right],
\]
where $h$ denotes a token prefix, $r_{\mathrm{strict}}(h,a)=\mathbf{1}[a=a^*(h)]$, and
\[
w_{\mathrm{sft}}(h,a)=\frac{d_{\mathrm{sft}}(h,a)}{d_{\pi_\theta}(h,a)}.
\]

This form exposes two limitations of SFT that are especially acute in agentic settings. First, the reward is exact-match and therefore assigns zero credit to functionally equivalent alternatives. Second, the importance-weight term reflects the mismatch between the expert data distribution and the current policy distribution. PivotRL addresses these limitations by replacing strict matching with a functional turn-level reward and by sampling actions on-policy at pivot states.
\fi
% \begin{proposition}[Only mixed-outcome pivots produce nonzero group-normalized updates]
% \label{prop:mixed}
% Let $s$ be a fixed pivot state, let $\{a_i\}_{i=1}^G$ be a rollout group sampled from the current policy, and let $\{r_i\}_{i=1}^G$ be the corresponding binary rewards. Define the normalized advantage
% \[
% \hat{A}_i=\frac{r_i-\frac{1}{G}\sum_{j=1}^G r_j}{\mathrm{std}(\{r_j\}_{j=1}^G)}.
% \]
% If $\sum_{i=1}^G r_i=0$ or $\sum_{i=1}^G r_i=G$, then $\hat{A}_i=0$ for all $i$. Therefore, only states with mixed sampled outcomes can contribute a nonzero group-normalized update.
% \end{proposition}

% \paragraph{Interpretation.}
% Proposition~\ref{prop:mixed} gives the basic justification for pivot selection. Randomly sampling from all turns wastes training budget on states that are already uniformly solved or uniformly failed under the current local rollout distribution. Filtering to mixed-outcome pivots increases the density of informative updates, and further biasing toward difficult mixed-outcome pivots helps maintain that signal later in training.

\begin{theorem}%[Functional reward as a KL-conservative update]
\label{thm:kl}
Fix $\beta>0$ and consider the regularized objective
\[
\mathcal{L}_{\mathrm{func},\beta}(\pi)
=
\mathbb{E}_{s\sim d}
\left[
-
\mathbb{E}_{a\sim\pi(\cdot\mid s)}[r_{\mathrm{func}}(s,a)]
+
\beta\,\mathrm{KL}(\pi(\cdot\mid s)\|\pi_0(\cdot\mid s))
\right],
\]
where $r_{\mathrm{func}}(s,a)=\mathbf{1}[a\in\mathcal{M}(s)]$. For each state $s$, let
\[
\rho(s)=\pi_0(\mathcal{M}(s)\mid s),
\qquad
q_\beta(s)=\frac{\rho(s)e^{1/\beta}}{(1-\rho(s))+\rho(s)e^{1/\beta}}.
\]
Then $d$-almost surely for each state $s$, $\mathcal{L}_{\mathrm{func},\beta}(\pi)$ has a unique minimizer $\pi_\beta^*$ such that it solves the following constraint optimization problem:
\begin{align*}
    \min \mathrm{KL}(\pi(\cdot\mid s)\|\pi_0(\cdot\mid s)) \quad s.t. ~~ \pi(\mathcal{M}(s)\mid s)=q_\beta(s).
\end{align*}
Furthermore, $\frac{\pi_\beta^\star(a\mid s)}{\pi_\beta^\star(b\mid s)}
= \frac{\pi_0(a\mid s)}{\pi_0(b\mid s)}$ holds for any $a,b \in \mathcal{M}(s)$ and $a,b \in \mathcal{M}(s)^c$.
% Equivalently, when $0<\rho(s)<1$, the optimal policy rescales the reference policy by one factor on acceptable actions and another factor on non-acceptable actions, thereby preserving the reference ordering within each set.
\end{theorem}

\paragraph{Interpretation.}
Theorem~\ref{thm:kl} analyzes PivotRL from a KL projection view that isolates the effect of the matching-style reward $r_{\mathrm{func}}(s,a)$ in the RL objective.
The analysis only depends on the induced matching set, so it applies to any matching rule that can be written in this indicator form.
This implies that PivotRL does not force the policy to collapse onto a single canonical continuation. Instead, it increases total probability mass on the verifier-approved set while minimally perturbing the reference policy in KL. In particular, it preserves the relative ordering among acceptable actions and, separately, among non-acceptable actions. This is the sense in which the functional reward supports OOD retention: it changes the policy where the verifier provides signal, while remaining conservative elsewhere.

\begin{theorem}\label{thm:pivot}
For any distribution $\pi$ over $\mathcal{A}$, define the score-tangent space 
$$T_\pi = \left\{ v : \mathcal{A}_s \to \mathbb{R}: \mathbb{E}_{a \sim \pi}[v(a)] = 0 \right\}$$
equipped with the Fisher inner product $\langle u, v \rangle_{F,\pi} = \mathbb{E}_{a \sim \pi}[u(a)v(a)]$.

For a smooth functional $F$ on the simplex, define its natural gradient $\nabla^{\mathrm{nat}}F(\pi) \in T_\pi$ as the unique Riesz representative satisfying $D F(\pi)[v]
= \langle \nabla^{\mathrm{nat}}F(\pi), v \rangle_{F,\pi}$ for any $v \in T_\pi$.

Consider the statewise expected reward objective
\begin{align*}
J_s(\pi)
= &~ \mathbb{E}_{a \sim \pi}[r_s(a)],
\end{align*}
and the population GRPO score for exponential-tilted policy $\pi_{s,\beta} = \frac{\pi_0(a \mid s)e^{r_s(a)/\beta}}{\sum_{b \in \mathcal{A}_s}\pi_0(b \mid s)e^{r_s(b)/\beta}}$, defined by
\begin{align*}
\gamma_{s,\beta}
:= &~ -\mathbb{E}_{a \sim \pi_{s,\beta}}
\left[
\frac{r_s(a) - \mathbb{E}_{a \sim \pi_{s,\beta}}[r_s(a)] }{\sqrt{\Var_{a \sim \pi_{s,\beta}}(r)}} \partial_\beta \log \pi_{s,\beta} (a)
\right].
\end{align*}
Then we have 
\begin{align*}
\gamma_{s,\beta} = \frac{1}{\beta^2}
\left\|\nabla^{\mathrm{nat}} J_s(\pi_{s,\beta})\right\|_{F,\pi_{s,\beta}} = \frac{\sqrt{\Var_{a \sim \pi_{s,\beta}}(r)}}{\beta^2}.
\end{align*}
\end{theorem}

\paragraph{Interpretation.} 
Theorem~\ref{thm:pivot} is a population, pathwise statement about the idealized
KL-regularized statewise update $\pi_{s,\beta}\propto \pi_0 e^{r_s/\beta}$.
By REINFORCE~\citep{williams1992simple},
for any smooth path $t \mapsto \pi_t$,
\[
\partial_t J_s(\pi_t)
=
\mathbb{E}_{a \sim \pi_t}
\bigl[
r_s(a)\,\partial_t \log \pi_t(a)
\bigr].
\]
The GRPO score $\gamma_{s,\beta}$ is thus the REINFORCE direction along the KL path where the rewards are normalized by the standard deviation. Theorem~\ref{thm:pivot} shows that the Fisher norm of the natural gradient of the statewise reward objective is exactly the reward standard deviation, and that the normalized REINFORCE covariance along the KL path is this norm divided by $\beta^2$. For binary verifier rewards, larger variance means a more mixed success/failure state. This motivates the pivot filter as a proxy for states with stronger local learning signal.


==> sections/related_works.tex <==
\section{Related Works}
\label{sec:related}

% \todo{refine and prune}

\subsection{Agentic RL}
% \todo{tool orchestra, agent lightning, arpo, etc etc}
Agentic language models interleave natural language with grounded actions such as tool calls, code execution, web navigation, and file edits, bootstrapped with supervised trajectories and prompting scaffolds~\citep{yao2023react,schick2023toolformer}.
Recent work also investigates explicit \emph{tool/model orchestration}, where a lightweight controller selects among tools or specialist models to improve efficiency and capability \citep{su2025toolorchestra}.
On the data and evaluation side, API-interaction corpora such as ToolBench and ToolLLM \citep{xu2023toolbench,qin2023toolllm} are complemented by benchmarks spanning embodied/text-world environments~\citep{shridhar2020alfworld,wang2022scienceworld}, web interaction~\citep{yao2022webshop}, multi-domain agent evaluation suites~\citep{ma2024agentboard}, and social-agent environments~\citep{wang2024sotopiapi}.
In software engineering, execution-grounded agents are trained and assessed on real repositories and environment-centric setups~\citep{wang2025openhandsopenplatformai,pan2025trainingsoftwareengineeringagents}.
Simulated multi-turn data generation has become a common ingredient for scaling agentic supervision \citep{prabhakar2025apigenmtagenticpipelinemultiturn}, and recent theory work begins to formalize why tool-integrated reasoning can expand capability \citep{lin2025tir}.

Reinforcement learning optimizes an interaction policy against task-derived or preference-derived feedback~\citep{ouyang2022training,schulman2017ppo,schulman2015trpo}.
For long-horizon agents, recent work targets exploration and credit assignment via stepwise progress attribution, exploration-based trajectory optimization, and verifier/meta-reasoning rewards \citep{wang2025sparl,song2024trialerror,zhang2025rlvmr}, as well as tree-structured sampling/search and robustness to imperfect process verifiers \citep{ji2025treesearchllmrl,rohatgi2025tamingprocessverifiers}.
End-to-end multi-turn RL has been applied directly to tool-integrated reasoning and multi-tool use \citep{xue2025simpletir,dong2025toolstar}, with systems advances for scalable and stable policy optimization \citep{yang2025dcpo,yu2025dapo}.
Large-scale agent training and environment design further improve the efficiency and stability of multi-turn RL for tool use \citep{luo2025agentlightningtrainai,dong2025agenticreinforcedpolicyoptimization}.
Multi-agent extensions study coordination and credit assignment in interactive settings \citep{zhou2025sweetrl,xi2025agentgymrl}.
In parallel, RL with \emph{verifiable} rewards (RLVR) has driven large gains in domains with automatic checkers, such as math and theorem proving \citep{shao2024deepseekmath,xin2024deepseekproverv15harnessingproofassistant,Guo_2025}.
Our work sits at this intersection: we target agentic interaction (terminal, code, browsing) while leveraging \emph{verifiability} by converting supervised trajectories into \emph{turn-level} rewards via completion-based verifiers, enabling on-policy optimization without training a separate reward model.

\subsection{Process Guidance}
% \todo{ArCHer (from levine's lab), SweetRL (from Levine's Lab), on policy distillation, Reinforcement Learning via Self-Distillation, GLM 4.5 (formatting + a), Process Reward Models, ARPO, DeepSeek process guidance}

A key challenge in long-horizon reasoning and acting is credit assignment: many failures are attributable to intermediate decisions rather than the final output.
Inference-time guidance encourages explicit intermediate reasoning, such as chain-of-thought prompting \citep{wei2022cot}, self-consistency decoding \citep{wang2022selfconsistency}, and tree-structured deliberation \citep{yao2023treeofthoughts}.
For agents, ReAct can be viewed as a lightweight process scaffold that interleaves intermediate rationales with tool actions \citep{yao2023react}.

Training-time approaches seek denser supervision signals.
Process reward models (PRMs) and step-level verification score intermediate reasoning trajectories rather than only final answers \citep{lightman2023letsverifystepstep}, and automated process-supervision pipelines aim to synthesize intermediate labels or critiques at scale \citep{luo2024improvemathematicalreasoninglanguage}.
In agentic RL, several lines of work obtain denser credit assignment through verifier and search-guided optimization~\citep{dong2025agenticreinforcedpolicyoptimization,ji2025treesearchllmrl}, and through explicit modeling of imperfect process verifiers \citep{rohatgi2025tamingprocessverifiers}.
Trajectory densification and multi-turn RL systems such as Agent Lightning provide another practical route to stabilize exploration and learning in tool-use environments \citep{luo2025agentlightningtrainai}.
Hierarchical multi-turn RL frameworks such as ArCHer~\citep{zhou2024archer} explicitly separate turn-level and token-level learning signals to improve multi-turn credit assignment, while social-agent RL methods such as SweetRL~\citep{zhou2025sweetrl} study protocol-level learning and credit assignment in multi-agent interaction.

Complementary to explicit reward shaping, distillation-based post-training uses on-policy rollouts to produce more robust or efficient policies \citep{lu2025onpolicydistillation}.
Recent work on reinforcement learning via self-distillation converts rich textual feedback (e.g., error messages) into dense learning signals without external teachers \citep{hubotter2026selfdistillation}.
Model development reports for agentic/coding systems (e.g., GLM-4.5) emphasize strict action formats and multi-stage post-training to stabilize long-horizon behavior \citep{5team2025glm45agenticreasoningcoding}, and large-scale RLVR systems such as DeepSeek-R1 highlight the effectiveness of enforcing verifiable outcomes for complex reasoning \citep{Guo_2025}.
PivotRL contributes a complementary perspective for agentic tasks with demonstrations: instead of learning a separate PRM, we treat each tool boundary (pivot) as a decision point and use the demonstration completion at that pivot as a \emph{verifier-derived} dense reward, which functions as process guidance tailored to multi-turn interaction.

\subsection{The Role of SFT in Agentic Post-Training}
% \todo{superficial alignment hypothesis: https://arxiv.org/pdf/2602.15829}

The role of supervised fine-tuning (SFT) in post-training has been actively debated.
\emph{Superficial alignment hypothesis} posits that alignment  merely surfaces the knowledge learned almost entirely during pre-training~\citep{zhou2023limaalignment}. Recent work operationalizes this perspective via explicit task-complexity controls \citep{vergarabrowne2026sahcomplexity} and revisits its empirical predictions across settings \citep{raghavendra2024revisitingSAH}.
These observations motivate training on  carefully curated trajectories, which is adopted and further advanced by PivotRL.

As a major class of alternatives, \emph{preference optimization} optimizes against preference comparisons.
Direct Preference Optimization (DPO) reparameterizes RLHF objectives into a supervised-style loss \citep{rafailov2023dpo}, and subsequent work explores variants that modify the implicit reward, regularization, or reference-model assumptions \citep{ethayarajh2024kto,hong2024orpo,meng2024simpo}, including segment-level formulations for multi-turn social agents \citep{kong2025sdpo}.
In contrast, PivotRL keeps demonstration data but eliminates \emph{behavior cloning as the training objective} for agentic trajectories: we use demonstrations only to define \emph{verifiable turn-level rewards} and then optimize on-policy.
This positioning is aligned with evidence that RL-style objectives can improve generalization relative to pure imitation when rewards reshape or correct the supervision signal \citep{chu2025sftmemorizesrlgeneralizes,wu2025generalization}.


\subsection{Adapting Behavior Cloning into RL}
% \todo{Dagger maybe}

% \todo{Prefix-RL (concurrent work)}

PivotRL can be viewed through the lens of imitation learning and RL-from-demonstrations.
Classical behavior cloning can suffer from compounding errors under distribution shift, motivating on-policy data aggregation methods such as DAgger \citep{ross2011dagger}, occupancy-measure matching approaches such as GAIL \citep{ho2016gail}, and RL-from-demonstrations methods that combine expert data with RL updates such as DQfD \citep{hester2018dqfd}.
Recent work also explores using partial successful traces as \emph{prefixes} to guide on-policy optimization; for example, PrefixRL conditions RL on off-policy prefixes to improve exploration on hard problems \citep{setlur2026prefixrl}.

Our approach is closest in spirit to this imitation-to-RL bridge, but tailored to multi-turn tool use.
We start from supervised trajectories, recast each turn as a decision point with a verifiable target action (the demonstration completion), and apply KL-regularized trust-region policy optimization \citep{schulman2017ppo,schulman2015trpo}.
Unlike offline preference optimization methods \citep{rafailov2023dpo,meng2024simpo}, we collect on-policy rollouts and use verifier rewards for turn-level credit assignment; unlike learned reward-model RLHF \citep{ouyang2022training,bai2022helpfulharmless}, we do not require training a separate reward model for these agentic tasks.



\subsection{Mitigating catastrophic forgetting in SFT}
% \todo{RL’S RAZOR: WHY ONLINE REINFORCEMENT
% LEARNING FORGETS LESS, RETAINING BY DOING: THE ROLE OF
% ON-POLICY DATA IN MITIGATING FORGETTING}
% \todo{https://arxiv.org/pdf/2510.14865,https://arxiv.org/pdf/2510.18874,https://arxiv.org/pdf/2405.09673}

A persistent issue in LLM post-training is catastrophic forgetting: optimizing on a narrow target distribution can degrade general capabilities.
Recent empirical studies document forgetting during continual instruction tuning \citep{luo2023empiricalCF}, and analyses link forgetting to optimization properties such as loss-landscape sharpness \citep{li2024revisitingCF}.
Mechanistic work further identifies circuit and component-level contributors to forgetting in transformer fine-tuning \citep{imanov2026mechanisticCF}.
These findings connect to the broader continual-learning literature, which proposes regularization and consolidation strategies such as EWC \citep{kirkpatrick2017ewc} and distillation-based retention methods like Learning without Forgetting \citep{li2016lwf}.

Several practical mitigations are especially relevant for LLMs: parameter-efficient tuning can reduce representational drift and empirically lessen forgetting \citep{biderman2024lora}, while data-mixing ``midtraining'' phases smooth distribution shifts between pretraining and post-training \citep{liu2025midtraining}.
Recent work also argues that online/on-policy RL can forget less than purely offline updates, retaining capabilities through continued interaction \citep{shenfeld2025rlsrazoronlinereinforcement,chen2025retainingdoingroleonpolicy}.
PivotRL complements these approaches from a KL projection perspective: it steers the policy toward task-specific behaviors while remaining close to the initialization and preserving the distribution over task-irrelevant actions, which may help mitigate forgetting when adapting LLM agents to long-horizon tool-use tasks.

% Experiences gained from the verified rewards setting \citep{shao2024deepseekmath,lambert2025tulu3pushingfrontiers,pyatkin2025generalizingverifiableinstructionfollowing}, where the only reward signal is from the final outcome, there is no trivial way to label each action with a process reward. Existing approaches that do not involve human labeling include using a explicit Process Reward Model \citep{lightman2023letsverifystepstep}, Monte Carlo Tree Search \citep{xin2024deepseekproverv15harnessingproofassistant,luo2024improvemathematicalreasoninglanguage}, heuristics-based search \citep{dong2025agenticreinforcedpolicyoptimization} or intermdiate state densification \citep{luo2025agentlightningtrainai} \todo{add more citations}.

% only small amounts of SFT is actually needed for training  \citep{zhou2023limaalignment,chu2025sftmemorizesrlgeneralizes}.

==> sections/related_works_v1.tex <==
\section{Related Works}
\label{sec:related}

\subsection{Agentic LLM and its Training Recipes}
Agentic language models, bootstrapped with self-supervised trajectories and prompting scaffolds~\citep{yao2023react,schick2023toolformer}, interleave natural language with grounded actions to enable complex interaction with the environments such as tool calls~\citep{xu2023toolbench,qin2023toolllm}, embodied/text-world~\citep{shridhar2020alfworld,wang2022scienceworld}, code execution~\citep{jimenez2024swe,wang2025openhandsopenplatformai,pan2025trainingsoftwareengineeringagents}, web navigation~\citep{yao2022webshop, wei2025browsecompsimplechallengingbenchmark}, multi-domain suites~\citep{ma2024agentboard}, and social-agent environments~\citep{wang2024sotopiapi}.

Reinforcement learning optimizes an interaction policy against task-derived or preference-derived feedback~\citep{ouyang2022training,schulman2017ppo,schulman2015trpo}.
For long-horizon agents, recent work targets exploration and credit assignment via stepwise progress attribution, exploration-based trajectory optimization, and verifier/meta-reasoning rewards \citep{wang2025sparl,song2024trialerror,zhang2025rlvmr}, as well as tree-structured sampling/search and robustness to imperfect process verifiers \citep{ji2025treesearchllmrl,rohatgi2025tamingprocessverifiers}.
End-to-end multi-turn RL has been applied directly to tool-integrated reasoning and multi-tool use \citep{xue2025simpletir,dong2025toolstar}, with systems advances for scalable and stable policy optimization \citep{yang2025dcpo,yu2025dapoopensourcellmreinforcement}.
Large-scale agent training and environment design further improve the efficiency and stability of multi-turn RL for tool use \citep{luo2025agentlightningtrainai,dong2025agenticreinforcedpolicyoptimization,su2025toolorchestra}.
Hierarchical multi-turn RL frameworks such as ArCHer~\citep{zhou2024archer} explicitly separate turn-level and token-level learning signals to improve multi-turn credit assignment.
Simulated multi-turn data generation has become a common ingredient for scaling agentic supervision \citep{prabhakar2025apigenmtagenticpipelinemultiturn}.
Multi-agent extensions study coordination and credit assignment in interactive settings \citep{zhou2025sweetrl,xi2025agentgymrl}.
In parallel, RL with \emph{verifiable} rewards (RLVR) has driven large gains in domains with automatic checkers, such as math and theorem proving \citep{shao2024deepseekmath,xin2024deepseekproverv15harnessingproofassistant,Guo_2025}.

Complementary to explicit reward shaping, distillation-based post-training uses on-policy rollouts to produce more robust or efficient policies \citep{lu2025onpolicydistillation}. Recent advancements in on-policy distillation enable student models to sample their own trajectories while receiving dense, token-level supervision from a teacher, significantly mitigating the distribution mismatch seen in off-policy methods and actively improving reasoning capabilities \citep{zhao2026selfdistilledreasoneronpolicyselfdistillation,xu2025learninginteractionagenticdistillation}.
Recent work on reinforcement learning via self-distillation converts rich textual feedback (e.g., error messages) into dense learning signals without external teachers \citep{hubotter2026selfdistillation}.
Model development reports for agentic/coding systems (e.g., GLM-4.5) emphasize strict action formats and multi-stage post-training to stabilize long-horizon behavior \citep{5team2025glm45agenticreasoningcoding}, and large-scale RLVR systems such as DeepSeek-R1 highlight the effectiveness of enforcing verifiable outcomes for complex reasoning \citep{Guo_2025}.
Our work sits at this intersection: we target agentic interaction (terminal, code, browsing) while leveraging \emph{verifiability} by converting supervised trajectories into \emph{turn-level} rewards via completion-based verifiers, enabling on-policy optimization without a separate reward model.


\subsection{Adapting Behavior Cloning into RL}

A persistent issue in LLM post-training, particularly during purely offline supervised updates, is catastrophic forgetting: optimizing on a narrow target distribution can degrade general capabilities \citep{luo2023empiricalCF,li2024revisitingCF,imanov2026mechanisticCF}. These findings connect to the broader continual-learning literature \citep{kirkpatrick2017ewc,li2016lwf} and the \emph{superficial alignment hypothesis} \citep{zhou2023limaalignment,vergarabrowne2026sahcomplexity,raghavendra2024revisitingSAH}.  Theoretical work establishes that offline imitation learning without environment interaction inherently suffers from suboptimality that grows quadratically with the task horizon \citep{rajaraman2020towardfundamentallimitsimitation}. Overcoming these fundamental limits necessitates interacting with the environment, motivating on-policy data aggregation methods such as DAgger \citep{ross2011dagger}, and variance-reduction techniques like replay estimation that smooth expert moment matching via online simulation \citep{swamy2022minimaxoptimalonlineimitation}.

Importantly, online/on-policy RL has been shown to mitigate forgetting compared to purely offline updates, retaining broader capabilities through continued environment interaction \citep{shenfeld2025rlsrazoronlinereinforcement,chen2025retainingdoingroleonpolicy}. 
To effectively transfer knowledge from offline demonstrations into robust online performance, RL-from-demonstrations approaches combine expert data with RL updates, using a pre-existing guide policy to form a curriculum of starting states for online exploration \citep{uchendu2022jumpstartreinforcementlearning}, or integrating offline data with RL updates as in DQfD \citep{hester2018dqfd}. Recent work also explores using partial successful traces as \emph{prefixes} to guide on-policy optimization \citep{setlur2026prefixrl}.
By performing Monte Carlo rollouts from the current policy and using the ground-truth SFT token as a reward signal, \citet{ming2025onetokenrollout} repurpose off-policy supervised datasets into on-policy RL signals.
Our approach is closest in spirit to this SFT-to-RL bridge, but using turn-based pivot selection and functional rewards to specialize in multi-turn tool use.


==> sections/results.tex <==
\section{Results}
\label{sec:results}

\todoempty

\begin{figure*}[t]
    \centering
    % --- Row 1 ---
    % Top Left
    \begin{subfigure}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/data_metrics/fig_depth_comparison.pdf}
        \caption{Depth Comparison}
        \label{fig:depth}
    \end{subfigure}
    \hspace{1em} % Space between columns
    % Top Right
    \begin{subfigure}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/data_metrics/fig_reward_mean_comparison.pdf}
        \caption{Reward Mean Comparison}
        \label{fig:reward_mean}
    \end{subfigure}
    
    \vspace{0.5cm} % Space between rows
    
    % --- Row 2 ---
    % Bottom Left
    \begin{subfigure}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/data_metrics/fig_reward_var_comparison.pdf}
        \caption{Reward Variance Comparison}
        \label{fig:reward_var}
    \end{subfigure}
    \hspace{1em} % Space between columns
    % Bottom Right
    \begin{subfigure}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/data_metrics/fig_unique_actions_comparison.pdf}
        \caption{Unique Actions Comparison}
        \label{fig:unique_actions}
    \end{subfigure}
    
    \caption{Comparison of depth, reward statistics, and unique actions.}
    \label{fig:metrics_comparison}
\end{figure*}


\subsection{SFT Results}
\todoempty

\subsection{RL Results}
\todoempty


==> sections/theory.tex <==
\subsubsection{A KL Projection View of our Reward}
In this subsection we analyze PivotRL from a KL projection view that isolates the effect of the matching-style reward
$r_{\name}(s,a)$ in the RL objective.
The analysis only depends on the induced matching set, so it applies to any matching rule that can be written in this indicator form.
The key message is that the population-loss optimizer minimally perturbs the reference policy among all policies that achieve the same expert-matching level.
Because this reward depends only on whether an action falls inside the matching set, the optimizer changes the reference only through a set-level reallocation of mass, while preserving the relative probabilities within the matching set and within its complement.

\begin{theorem}[RL with $r_{\name}$ as KL projection under matching-style rewards]\label{thm:pivotrl_kl_projection}
Assume the action space $\mathcal A$ is finite and $\pi_0(a\mid s)>0$ for all $s$ and $a$.
Fix $\beta>0$ and $\epsilon\geq 0$.
Consider the RL loss
\begin{align*}
\mathcal L_{\text{PivotRL},\beta}(\pi)
=
\mathbb E_{s\sim\mathcal D_{\sft}}\Big[
-\mathbb E_{a\sim\pi(\cdot\mid s)}[r_{\name}(s,a)]
+ \beta \cdot \KL(\pi(\cdot\mid s)\|\pi_0(\cdot\mid s))
\Big]
\end{align*}
with $r_{\name}$ defined in Equation~\eqref{eq:pivotrl-reward}.
For each $s$, let
\begin{align*}
\rho_\epsilon(s)=\pi_0(\mathcal M_\epsilon(s)\mid s),
\qquad
q_{\beta,\epsilon}(s)=\frac{\rho_\epsilon(s)e^{1/\beta}}{(1-\rho_\epsilon(s))+\rho_\epsilon(s)e^{1/\beta}}.
\end{align*}
Then the unique minimizer $\pi_{\beta,\epsilon}^\star$ of $\mathcal L_{\text{PivotRL},\beta}$ (up to $\mathcal D_{\sft}$-a.e. equality) is characterized as follows:
for $\mathcal D_{\sft}$-a.e. $s$, among all distributions $\pi(\cdot\mid s)$ satisfying the matching constraint
\begin{align*}
\pi(\mathcal M_\epsilon(s)\mid s)=q_{\beta,\epsilon}(s),
\end{align*}
$\pi_{\beta,\epsilon}^\star(\cdot\mid s)$ is the unique minimizer of
\begin{align*}
\KL(\pi(\cdot\mid s)\|\pi_0(\cdot\mid s)).
\end{align*}
Equivalently, if $0<\rho_\epsilon(s)<1$, then
\begin{align}\label{eq:teacher-policy}
\pi_{\beta,\epsilon}^\star(a\mid s)
=
\begin{cases}
\frac{q_{\beta,\epsilon}(s)}{\rho_\epsilon(s)}\pi_0(a\mid s), & a\in\mathcal M_\epsilon(s),\\[6pt]
\frac{1-q_{\beta,\epsilon}(s)}{1-\rho_\epsilon(s)}\pi_0(a\mid s), & a\notin\mathcal M_\epsilon(s),
\end{cases}
\end{align}
while if $\rho_\epsilon(s)=1$, then $\pi_{\beta,\epsilon}^\star(\cdot\mid s)=\pi_0(\cdot\mid s)$.
\end{theorem}

Theorem~\ref{thm:pivotrl_kl_projection} characterizes the ``conservatism'' of $r_{\name}$:
for each $s$, the optimal policy $\pi_{\beta,\epsilon}^\star(\cdot\mid s)$ is the unique distribution that achieves the matching level $q_{\beta,\epsilon}(s)$ on the acceptable set $\mathcal M_\epsilon(s)$ and perturbs the reference $\pi_0(\cdot\mid s)$ as little as possible in KL, which is precisely an information projection~\citep{csiszar1975divergence,bregman1967relaxation}.
From Equation~\eqref{eq:teacher-policy}, we also infer that $\pi_{\beta,\epsilon}^\star$ differs from $\pi_0$ only through a two-block reallocation of mass:
\begin{align*}
\frac{\pi_{\beta,\epsilon}^\star(a\mid s)}{\pi_{\beta,\epsilon}^\star(b\mid s)}=\frac{\pi_0(a\mid s)}{\pi_0(b\mid s)}, ~\forall~a,b\in \mathcal M_\epsilon(s),
\end{align*}
and
\begin{align*}
\frac{\pi_{\beta,\epsilon}^\star(a\mid s)}{\pi_{\beta,\epsilon}^\star(b\mid s)}=\frac{\pi_0(a\mid s)}{\pi_0(b\mid s)}, ~\forall~a,b\notin \mathcal M_\epsilon(s).
\end{align*}
This implies that $\pi_{\beta,\epsilon}^\star(\cdot\mid s)$ preserves the reference ranking among all matching actions and, separately, among all non-matching actions.
Thus a matching-style reward increases only the total mass assigned to the acceptable set, rather than forcing all additional mass onto one canonical response.
Together, these perspectives explain why $r_{\name}$ can increase expert matching while maintaining the reference distribution over non-golden actions---and, more generally, within each reward-equivalence class---thereby better preserving out-of-domain performance and mitigating catastrophic forgetting.
The proof is deferred to Appendix~\ref{sec:proof-kl-proj}.
